Minimax optimal approaches to the label shift problem in non-parametric settings

We study the minimax rates of the label shift problem in non-parametric classification. In addition to the unsupervised setting in which the learner only has access to unlabeled examples from the target domain, we also consider the setting in which a small number of labeled examples from the target domain is available to the learner. Our study reveals a difference in the difficulty of the label shift problem in the two settings, and we attribute this difference to the availability of data from the target domain to estimate the class conditional distributions in the latter setting. We also show that a class proportion estimation approach is minimax rate-optimal in the unsupervised setting.

==> YK-macros.tex <==

\def\Avar{{\sf Avar}}
\def\abs#1{\left|#1\right|}
\def\aff{{\sf aff}}
\def\argmin{{\arg\min}}
\def\argmax{{\arg\max}}
\def\avar{{\sf avar}}

\def\bA{\mathbf{A}}
\def\bB{\mathbf{B}}
\def\bC{\mathbf{C}}
\def\bD{\mathbf{D}}
\def\bE{\mathbf{E}}
\def\bF{\mathbf{F}}
\def\bff{\mathbf{f}}
\def\bG{\mathbf{G}}
\def\bH{\mathbf{H}}
\def\bI{\mathbf{I}}
\def\bJ{\mathbf{J}}
\def\bK{\mathbf{K}}
\def\bL{\mathbf{L}}
\def\bM{\mathbf{M}}
\def\bN{\mathbf{N}}
\def\bO{\mathbf{O}}
\def\bP{\mathbf{P}}
\def\bQ{\mathbf{Q}}
\def\bR{\mathbf{R}}
\def\bS{\mathbf{S}}
\def\bT{\mathbf{T}}
\def\bU{\mathbf{U}}
\def\bV{\mathbf{V}}
\def\bW{\mathbf{W}}
\def\bX{\mathbf{X}}
\def\bY{\mathbf{Y}}
\def\bZ{\mathbf{Z}}

\def\bGamma{{\boldsymbol\Gamma}}
\def\bDelta{{\boldsymbol\Delta}}
\def\bTheta{{\boldsymbol\Theta}}
\def\bLambda{{\boldsymbol\Lambda}}
\def\bXi{{\boldsymbol\Xi}}
\def\bPi{{\boldsymbol\Pi}}
\def\bSigma{{\boldsymbol\Sigma}}
\def\bUps{{\boldsymbol\Upsilon}}
\def\bPhi{{\boldsymbol\Phi}}
\def\bPsi{{\boldsymbol\Psi}}
\def\bOmega{{\boldsymbol\Omega}}

\def\ba{\mathbf{a}}
\def\bb{\mathbf{b}}
\def\bc{\mathbf{c}}
\def\bbd{\mathbf{d}}
\def\bd{{\sf bd}}
\def\be{\mathbf{e}}
\def\bbf{\mathbf{f}}
\def\bg{\mathbf{g}}
\def\bh{\mathbf{h}}
\def\bi{\mathbf{i}}
\def\bj{\mathbf{j}}
\def\bk{\mathbf{k}}
\def\bl{\mathbf{l}}
% \def\bm{\mathbf{m}}
\def\bn{\mathbf{n}}
\def\bo{\mathbf{o}}
\def\bp{\mathbf{p}}
\def\bq{\mathbf{q}}
\def\br{\mathbf{r}}
\def\bs{\mathbf{s}}
\def\bt{\mathbf{t}}
\def\bu{\mathbf{u}}
\def\bv{\mathbf{v}}
\def\bw{\mathbf{w}}
\def\bx{\mathbf{x}}
\def\by{\mathbf{y}}
\def\bz{\mathbf{z}}

\def\balpha{{\boldsymbol\alpha}}
\def\bbeta{{\boldsymbol\beta}}
\def\bgamma{{\boldsymbol\gamma}}
\def\bdelta{{\boldsymbol\delta}}
\def\beps{{\boldsymbol\epsilon}}
\def\bveps{{\boldsymbol\varepsilon}}
\def\bzeta{{\boldsymbol\zeta}}
\def\bfeta{{\boldsymbol\eta}}
\def\btheta{{\boldsymbol\theta}}
\def\bvtheta{{\boldsymbol\vartheta}}
\def\biota{{\boldsymbol\iota}}
\def\bkappa{{\boldsymbol\kappa}}
\def\blambda{{\boldsymbol\lambda}}
\def\bmu{{\boldsymbol\mu}}
\def\bnu{{\boldsymbol\nu}}
\def\bxi{{\boldsymbol\xi}}
\def\bpi{{\boldsymbol\pi}}
\def\brho{{\boldsymbol\rho}}
\def\bvrho{{\boldsymbol\varrho}}
\def\bsigma{{\boldsymbol\sigma}}
\def\btau{{\boldsymbol\tau}}
\def\bups{{\boldsymbol\upsilon}}
\def\bphi{{\boldsymbol\phi}}
\def\bvphi{{\boldsymbol\varphi}}
\def\bpsi{{\boldsymbol\psi}}
\def\bomega{{\boldsymbol\omega}}

\def\bbA{\mathbb{A}}
\def\bbB{\mathbb{B}}
\def\bbC{\mathbb{C}}
\def\bbD{\mathbb{D}}
\def\bbE{\mathbb{E}}
\def\bbF{\mathbb{F}}
\def\bbG{\mathbb{G}}
\def\bbH{\mathbb{H}}
\def\bbI{\mathbb{I}}
\def\bbJ{\mathbb{J}}
\def\bbK{\mathbb{K}}
\def\bbL{\mathbb{L}}
\def\bbM{\mathbb{M}}
\def\bbN{\mathbb{N}}
\def\bbO{\mathbb{O}}
\def\bbP{\mathbb{P}}
\def\bbQ{\mathbb{Q}}
\def\bbR{\mathbb{R}}
\def\bbS{\mathbb{S}}
\def\bbT{\mathbb{T}}
\def\bbU{\mathbb{U}}
\def\bbV{\mathbb{V}}
\def\bbW{\mathbb{W}}
\def\bbX{\mathbb{X}}
\def\bbY{\mathbb{Y}}
\def\bbZ{\mathbb{Z}}

\def\Ber{{\sf Ber}}
\def\bin{{\sf bin}}

\def\cA{\mathcal{A}}
\def\cB{\mathcal{B}}
\def\cC{\mathcal{C}}
\def\cD{\mathcal{D}}
\def\cE{\mathcal{E}}
\def\cF{\mathcal{F}}
\def\cG{\mathcal{G}}
\def\cH{\mathcal{H}}
\def\cI{\mathcal{I}}
\def\cJ{\mathcal{J}}
\def\cK{\mathcal{K}}
\def\cL{\mathcal{L}}
\def\cM{\mathcal{M}}
\def\cN{\mathcal{N}}
\def\cO{\mathcal{O}}
\def\cP{\mathcal{P}}
\def\cQ{\mathcal{Q}}
\def\cR{\mathcal{R}}
\def\cS{\mathcal{S}}
\def\cT{\mathcal{T}}
\def\cU{\mathcal{U}}
\def\cV{\mathcal{V}}
\def\cW{\mathcal{W}}
\def\cX{\mathcal{X}}
\def\cY{\mathcal{Y}}
\def\cZ{\mathcal{Z}}

\def\cat{{\sf cat}}
\def\Cov{{\sf Cov}}
\def\cov{{\sf cov}}
\def\card{{\bf card}}
\def\cf{{\it cf.}}
\def\cl{{\sf cl}}
\def\complex{{\bbC}}
\def\cone{{\sf cone}}
\def\conv{{\sf conv}}
\def\deq{\overset{d}{=}}
\def\det{{\sf det}}
\def\diag{{\sf diag}}
\def\diam{{\sf diam}}
\def\dist{{\sf dist}}
\def\dom{{\sf dom}}
\def\doop{{\sf do}}
\def\dto{\overset{\sf d}{\to}}
\def\Ex{{\bbE}}
\def\Exp{{\sf Exp}}
\def\exp{{\sf exp}}
\def\eg{{\it e.g.}}
\def\epi{{\sf epi}}
\def\eps{{\epsilon}}
\def\etc{{\it etc.}}
\def\ie{{\it i.e.}}
\def\iid{{\sf iid}}
\def\ind{{\sf ind}}
\def\intr{{\sf int}}
\def\integers{{\bbZ}}

\def\halpha{\widehat{\balpha}}
\def\hbeta{\widehat{\bbeta}}
\def\hdelta{\widehat{\bdelta}}
\def\hGamma{\widehat{\bGamma}}
\def\hgamma{\widehat{\bgamma}}
\def\hmu{\widehat{\bmu}}
\def\hSigma{\widehat{\bSigma}}
\def\hsigma{\widehat{\bsigma}}
\def\hTheta{\widehat{\bTheta}}
\def\htheta{\widehat{\btheta}}
\def\hw{\widehat{\bw}}

\def\KL{{\sf KL}}
\def\ker{{\sf ker}}
\def\lspan{{\sf span}}
\def\maximize{{\sf maximize}}
\def\med{{\sf med}}
\def\minimize{{\sf minimize}}
\def\norm#1{\left\|#1\right\|}
\def\ones{\mathbf{1}}
\def\Poi{{\sf Poi}}
\def\Pr{{\bbP}}
\def\peq{\overset{\sf p}{=}}
\def\plim{{\sf plim}}
\def\proj{{\sf proj}}
\def\prox{{\sf prox}}
\def\pto{\overset{\sf p}{\to}}
\def\ran{{\sf ran}}
\def\rank{{\sf rank}}
\def\reals{{\bbR}}
\def\relint{{\sf relint}}
\def\sign{{\sf sign}}
\def\supp{{\sf supp}}
\def\symm{{\bbS}}

\def\st{\textrm{subject to}}
\def\tr{{\sf tr}}
\def\tube{{\sf tube}}
\def\TV{{\sf TV}}
\def\unif{{\sf unif}}
\def\Var{{\sf Var}}
\def\var{{\sf var}}
\def\vct{{\sf vec}}
\def\veps{\varepsilon}
\def\vol{{\sf vol}}
\def\zeros{\mathbf{0}}


==> YK-thm-macros.tex <==

\newtheorem{theorem}{Theorem}[section]
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{model}[theorem]{Model}
% \newenvironment{proof}{\noindent {\sc Proof:}}{$\Box$ \medskip} 
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{remark}[theorem]{Remark}


==> estimator.tex <==
\begin{theorem}[\textbf{Lower-bound}]
	Let $ (\cX,\rho) = ([0,1]^d, \|\cdot\|_2) $ for some $ d\in \mathbb{N}. $ Assume further that $ \alpha \beta \le d. $ Let $ \cT $ be the class of probability distributions $ (P,Q) $ such that $ \eta_Q $ is $ \alpha $ smooth, $ P_0 $ and $ P_1 $ have strong densities, and $ Q $ has noise parameter $ \beta. $ For any classifier $  \hat h  $ learned on $ (\bX,\bY), $ we have:
\[ \sup_{(P,Q)\in \cT} \Ex_{(\bX,\bY) \sim (P,Q)} \left[\cE_Q(\hat h)  \right] \ge c(n_P+n_Q)^{-(\beta+1)/d_0} ,\] where, $ d_0= 2+\frac d\alpha. $
\end{theorem}
\begin{proof}
	Let $ r = c_r N^{-\frac1{\alpha d_0}} ,\ m = \lfloor c_m r^{\alpha\beta -d} \rfloor,\ w = c_w r^d ,$ where, $ N = n_P+n_Q,\ c_r = \frac19, \ c_m = 8\times 9^{\alpha\beta - d},\ 0<c_w \le 1 $ to be chosen later. 
	
	For such a choice we have $ 8\le m < \lfloor r^{-1} \rfloor ^d. $ As, $ \alpha\beta \le d, $ we have $ r \le \frac19. $ This implies $ c_m r^{\alpha\beta -d} \ge 8. $  Since $ r^{-1} \ge 8 $ which gives us $ r^{-1} \le \frac{9\lfloor r^{-1}\rfloor}{8}. $ Therefore, $ c_mr^{\alpha\beta -d} = 8 (9r)^{\alpha\beta}\left( \frac{r^{-1}}{9}\right) < 8^{1-d } \lfloor r^{-1} \rfloor ^d  \le \lfloor r^{-1} \rfloor ^d.$ 
	
	$ mw = mc_w r^d <1. $
	
	\textbf{Construction of $ p_0 $ and $ p_1: $}
	Divide $ \cX = [0,1]^d $ into $ \lfloor r^{-1} \rfloor ^d $ hypercubes of length $ r. $ Let $ \cZ $ be the set of their centers. Let $ \cZ_1 \subset \cZ $ such that $ \left|\cZ_1 \right| = m. $ Let $ \cZ_0 = \cZ \backslash \cZ_1,\ \cX_1 = \cup_{z\in\cZ_1} B\left( z,\frac r6  \right), \text{and } \cX_0 = \cup_{z\in\cZ_0} B\left( z,\frac r2  \right). $ Let $ q_1 = \frac w{\text{Vol}\left( B\left(z,\frac r6\right)  \right)}, \text{ and } q_0 = \frac{1-mw}{\text{Vol}\left(\cX_0\right)}.$  For $ \sigma \in \{-1,1\}^m, $ define \[ p_1^\sigma (x) = \begin{cases}
	a^\sigma q_1 \left(1+\sigma(z)\eta_z (x) \right) & x \in B\left(z,\frac r6  \right), \ z \in \cZ_1,\\
	a^\sigma q_0 & x \in B\left(z,\frac r2  \right), \ z \in \cZ_0,\\
	0 & \text{otherwise},
	\end{cases} \] and, \[ p_0^\sigma (x) = \begin{cases}
	b^\sigma q_1 \left(1-\sigma(z)\eta_z (x) \right) & x \in B\left(z,\frac r6  \right), \ z \in \cZ_1,\\
	b^\sigma q_0 & x \in B\left(z,\frac r2  \right), \ z \in \cZ_0,\\
	0 & \text{otherwise},
	\end{cases} \] where, $ \eta_z (x) = C_\alpha' r^\alpha u^\alpha \left( \frac{\|x-z\|_2}{r}  \right) ,$ \[ u(x) = \begin{cases}
	1 & \text{if } x \le \frac16,\\
	1 - 6\left(x -\frac16  \right) & \text{if } \frac16 < x \le \frac13,\\
	0 & \text{if } x> \frac13,
	
	\end{cases} \] and $ C_\alpha' = \min \left\{ C_\alpha 6^{-\alpha}, \frac12  \right\}. $
	
	We want $ \int p_1^\sigma (x) dx = a^\sigma \left[ mw + (1-mw) + w\sum_{z\in\cZ_1} \sigma(z) C_\alpha'r^\alpha \right] = 1. $ Hence, $ a^\sigma = \frac1 {1+ w\sum_{z\in\cZ_1} \sigma(z)C_\alpha'r^\alpha}. $ Also, $ b^\sigma = \frac1 {1- w\sum_{z\in\cZ_1} \sigma(z)C_\alpha'r^\alpha}. $ Also, we want $ \frac{a^\sigma q_0 \pi_Q ^\sigma   }{b^\sigma q_0 \left(1-\pi_Q ^\sigma  \right)} = 1, $ which implies $ \pi_Q ^\sigma = \frac{1/a^\sigma}{1/a^\sigma + 1/b^\sigma} = \frac 12 \left( 1+ w  \sum_{z\in\cZ_1} \sigma(z) \right)  . $ We have freedom to set $ \pi_P^\sigma>0. $ Set $ \pi_P^\sigma = \frac 12 \left( 1+ w  \sum_{z\in\cZ_1} \sigma(z) \right)  . $
	
	Then \[ \frac{1-\pi_Q^\sigma}{\pi_Q^\sigma} \frac{p_0^\sigma(x)}{p_1^\sigma(x)} = \begin{cases}
	\frac{1- \sigma(z)\eta_z(x)}{1+ \sigma(z)\eta_z(x)} & \text{if } x\in \cX_1,\\
	1 & \text{if } x\in \cX_0.
	\end{cases} \] 
	Then $ \eta_Q^\sigma(x) = \begin{cases}
	\frac{1+ \sigma(z)\eta_z(x)}{2} & \text{if } x\in \cX_1,\\
	\frac12 & \text{if } x\in \cX_0.
	\end{cases} $ 
	
	So, $ \eta_Q^\sigma $ simplifies to \[ \eta_Q^\sigma(x) = \begin{cases}
	\frac{1+ \sigma(z)C_\alpha'r^\alpha}{2} & \text{if } x\in B\left( z,\frac r6 \right),\ z\in\cZ_1\\
	\frac12 & \text{if } x\in\cX_0.
	\end{cases}. \] 
	Extend it to \[ \eta_Q^\sigma(x) = \begin{cases}
	\frac{1+ \sigma(z)C_\alpha'r^\alpha}{2} & \text{if } x\in B\left( z,\frac r6 \right),\ z\in\cZ_1\\
	\frac12 & \text{otherwise.}
	\end{cases}. \] 
	The marginal density of $ X $ under the distribution $ Q $ is \[q_X = \pi_Q^\sigma p_1 + (1-\pi_Q^\sigma) p_0 = \begin{cases}
	q_1 & \text{for } x\in \cX_1,\\
	q_0 & \text{for } x \in \cX_0.
	\end{cases}\] 
	
	
	For $ x\in B\left(z,\frac r6 \right), \ z\in \cZ_1, $ \begin{align*}
		q_X(x) & = \pi_Q^\sigma p_1(x) + (1-\pi_Q^\sigma) p_0(x)\\
		& = a^\sigma q_1 \left(1+\sigma(z)\eta_z (x) \right) \frac1{2a^\sigma}  + b^\sigma q_1 \left(1-\sigma(z)\eta_z (x) \right) \frac1{2b^\sigma}\\
		& = q_1.
	\end{align*}
	
	For $ x\in B\left(z,\frac r2 \right), \ z\in \cZ_0, $ \begin{align*}
	q_X(x) & = \pi_Q^\sigma p_1(x) + (1-\pi_Q^\sigma) p_0(x)\\
	& = a^\sigma q_0  \frac1{2a^\sigma}  + b^\sigma q_0  \frac1{2b^\sigma}\\
	& = q_0.
	\end{align*}
	
	
	  \textbf{Checking H\"older condition of $ \eta_Q: $}
	 For $ 0\le x\le y, $ $ y  = x + (x-y) \le \left( x^\alpha + (y-x)^\alpha \right)^{1/\alpha}. $ This implies $ y^\alpha - x^\alpha \le (y-x)^\alpha. $  Hence, \begin{align*}
	 	\left|\eta_Q(x) - \eta_Q(x') \right| & = C_\alpha' r^\alpha \left|  u^\alpha \left(\frac{\|x-z\|_2 }{r} \right) - u^\alpha \left(\frac{\|x'-z\|_2 }{r} \right)\right|\\
	 	& \le C_\alpha \|x-x'\|_2^\alpha.
	 \end{align*}
	 
	 \textbf{Checking Tsybakov's noise condition:} For $ t < C_\alpha' r^\alpha/2, \ Q_X \left( 0< \left| \eta_Q(X) -\frac12 \right| \le t \right) =0. $ 
	 For $ t\ge C_\alpha' r^\alpha/2, $ \begin{align*}
	 	Q_X \left( 0< \left| \eta_Q(X) -\frac12 \right| \le t \right) &  = mw\\
	 	& \le c_mc_w r^{\alpha \beta}\\
	 	& \le C_\beta \left( \frac{C_\alpha' r^\alpha}{2}  \right)^\beta.
	 \end{align*}
	 
	 \begin{align*}
	 \cE_{Q^\sigma}(h) & = 2\Ex _{Q_X} \left[\left | \eta_Q^\sigma(X) - \frac12 \right | \mathbf{1}\left( h(X) \neq h^*_\sigma(X)  \right)\right]\\
	 & = C_\alpha' r^\alpha Q_X\left( \{h(X) \ne h_\sigma^*(X)  \} \cap \cX_1 \right).
	 \end{align*}
	 
	 At this point it is a good time to mention that choosing different value of $ \pi_P^\sigma $ than $ \pi_Q $ would not have any effect on $ \cE_{Q^\sigma}(h), $ rather than making the proof more lengthy. We can set it to be $ \pi_Q = \pi_P. $  
	 
	 Let $ \cF $ be the set of all classifier relevant to this classification problem. For $ h,h'\in\cF $ define $ \bar\rho (h,h') \coloneqq C_\alpha' r^\alpha Q_X \left( \{h(X)\neq h'(X)\} \cap \cX_1 \right). $ For $ \sigma\in\{-1,1\}^m, $ let $ h_\sigma^* $ be the Bayes classifier defined as $ h_\sigma^* (x) = \mathbf{1}\{\eta_Q^\sigma(x) \ge 1/2\}. $ Then, for $ \sigma, \sigma'\in\{-1,1\}^m, $  $ \bar\rho (h_\sigma^*, h_{\sigma'}^*) = C_\alpha' r^\alpha w \rho_H(\sigma, \sigma'), $ where, $ \rho_H(\sigma,\sigma') $ is the Hamming distance defined as $ \rho_H(\sigma,\sigma') \coloneqq \text{card} \{z\in\cZ_1 :\sigma(z) \neq \sigma'(z) \}. $
	 
	  
	 \begin{lemma}[Varshamov-Gilbert bound]
	 	Let $ m\ge 8. $ Then there exists a subset $ \{ \sigma_0,\ldots , \sigma_M \} \subset \{-1,1\}^m $ such that $ \sigma_0 = (0,\ldots,0), $ \[ \rho_H(\sigma_i , \sigma_j ) \ge \frac m 8, \ \text{for all } 0\le i<j\le M,\ \text{and } M \ge 2^{m/8}, \] where, $ \rho_H $ is the hamming distance. 
	 \end{lemma}
 
 Let $\{ \sigma_0,\ldots , \sigma_M \} \subset \{-1,1\}^m  $ be the choice obtained from the above lemma. For each $ i \in \{0,\ldots,M\} $ let us set the distributions of two populations to be $ (P^i, Q^i) = (P^{\sigma_i}, Q^{\sigma_i}). $ The joint distribution of $ (\bX,\bY) $ is set at $ \Pi_i = {P^i}^{\otimes n_p} \otimes {Q^i}^{\otimes n_Q} = {Q^i}^{\otimes (n_P+n_Q)}.$
 
 Denote $ h_{\sigma_i}^* $ by $ h_i^* .$ For $ 0\le i<j\le M, $ \begin{align*}
 	\bar\rho (h_i^*,h_j^*) &\ge C_\alpha' \frac{wmr^\alpha }{8}\\ 
 	&\ge \frac12 C_\alpha' c_r^\alpha (n_P+n_Q)^{-\frac1{d_0}} c_mr^{\alpha\beta -d} c_w r^d \\
 	& \ge C (n_P+n_Q)^{-\left(\frac{1}{d_0} +\frac{\alpha\beta}{\alpha d_0} \right)}\\
 	& = C (n_p+n_Q)^{-\frac{1+\beta}{d_0}}\\
 	& =: s.
 \end{align*}
 
 Let $ D(P|Q) $ be the KL-Divergence between the distributions $ P $ and $ Q. $ Then $ D(\Pi_i| \Pi_0) = n_P D(P^i|P^0) + n_Q D(Q^i|Q^0) = (n_P+n_Q) D(Q^i|Q^0). $ Now, \begin{align*}
 	D(Q^i|Q^0) & = \int \log\left( \frac{dQ^i}{dQ^0}  \right) dQ^i\\
 	& = \int \left[ \log \left( \frac{\eta_Q^i (x)}{\eta_Q^0(x)}  \right) \eta_Q^i(x) + \log \left( \frac{1-\eta_Q^i (x)}{1-\eta_Q^0(x)}  \right) (1-\eta_Q^i(x))  \right] dQ_X\\
 	& = \sum_{z: \sigma_i(z) \neq \sigma_0(z)} Q_X \left(B\left( z,\frac r6  \right)  \right) \left[ \log \left( \frac{1+ C_\alpha'r^\alpha}{1- C_\alpha'r^\alpha}  \right) \frac{1+ C_\alpha'r^\alpha}{2} +  \log\left( \frac{1- C_\alpha'r^\alpha}{1+ C_\alpha'r^\alpha}  \right) \frac{1- C_\alpha'r^\alpha}{2} \right] \\
 	& = w \rho_H(\sigma_i , \sigma_0) \log \left( \frac{1+ C_\alpha'r^\alpha}{1- C_\alpha'r^\alpha}  \right) C_\alpha'r^\alpha\\
 	& \le 2mw\frac{C_\alpha'^2 r^{2\alpha}}{1-C_\alpha'r^\alpha}\\
 	& \le 4mw C_\alpha'^2 r^{2\alpha}.
 \end{align*}  Hence, 
 \begin{align*}
 	D(\Pi_i|\Pi_0) &\le  4mw C_\alpha'^2 r^{2\alpha} (n_P+n_Q)\\
 	 &= 4m c_w r^d C_\alpha'^2 r^{2\alpha} (n_P+n_Q)\\
 	 & = 4m c_w C_\alpha'^2 r^{2\alpha+d} (n_P+n_Q)\\
 	 & = 4m c_w C_\alpha'^2 c_r^{2\alpha+d} (n_P+n_Q)^{-\frac{2\alpha +d}{\alpha d_0}} (n_P+n_Q)\\
 	 & = 4m c_w C_\alpha'^2 c_r^{2\alpha+d} \text{ since } \alpha d_0 = 2\alpha + d\\
 	 & = 2^5 (\log 2)^{-1} c_w C_\alpha'^2 c_r^{2\alpha+d} \log (M)\\
 	 &\le \frac 18\log (M),  
 \end{align*} for $ c_w $ small enough. 
 \begin{proposition}[Thm 2.5 of Tsybakov (2009)] 
 	Let $ \{ \Pi_h\}_{h\in \cH} $ be a family of distributions indexed over a subset $ \cH $ of a semi-metric $ (\cF,\bar \rho). $ Suppose $\exists h_0, \ldots h_M\in \cH , $ for $ M\ge 2, $ such that:
 	\begin{enumerate}
 		\item $ \bar\rho (h_i , h_j) \ge 2s>0, \forall \ 0 \le i<j \le M, $
 		\item $ \Pi_{h_i} \ll \Pi_{h_0} $ for all $ i\in [M,] $ and the average KL-divergence to $ \Pi_{h_0} $ satisfies \[ \frac1M \sum_{i=1}^M D(\Pi_{h_i}|\Pi_{h_0}) \le \kappa \log M, \ \text{where } 0<\kappa < \frac18. \]
 	\end{enumerate}
 Let $ Z\sim \Pi_h, $ and let $ \hat h : Z \to \cF $ denote any improper learner of $ h \in \cH. $ We have for any $ \hat h : $ \[ \sup_{h\in\cH}  \Pi_h\left( \bar\rho (\hat h (Z),h)  \ge s \right)  \ge \frac {3-2\sqrt{2}}{8}.  \]
\end{proposition}
 
 Hence, \begin{align*}
 	\sup_{(P,Q)\in \cT} \Ex_{(P,Q)} \cE_Q (\hat h)& \ge \sup_{(P,Q)\in \cT} s \Pr_\Pi \left ( \cE_Q (\hat h)\ge s \right)\\
 	& \ge s \sup_{\sigma\in \{-1,1\}^m} \Pi_\sigma \left(\cE_{Q^\sigma} (\hat h)\ge s \right) \\
 	& \ge s \frac {3-2\sqrt{2}}{8}\\
 	& \ge C'(n_p+n_Q)^{-\frac{1+\beta}{d_0}}
 \end{align*}
 
 
 Now we have to deal with the error of estimation for the parameter $ \pi_Q. $ We shall see that, it is enough to construct two distributions for this purpose. Consider $ \cX = B(x_0,r_0)\subset [0,1]^d $ where $ x_0  $ is the mid-point for $ [0,1]^d $ and $ 0< r_0 < \frac12. $
 
 For $ x \in \cX $ let us define the densities of two distributions:
 
 \[ p_0(x) =  \frac1{a(d) r_0^d} \] and \[ p_1(x) = \frac{1}{a(d) r_0^d} \left[\frac12 + \frac{d/\beta + d}{2r_0^{d/\beta}} \|x-x_0\|_2^{d/\beta}  \right] \] Notice that the ratio $ \frac{p_0}{p_1}(x) $ is $ d/\beta $-smooth and hence $ \alpha  $-smooth. For $ k \in \{0,1\}, $ let us define $ \pi_k = \frac 12 \left( 1+ (-1)^k \frac1{\sqrt{n}} \right) = \frac12 + \frac12\delta_k. $ Then $ \frac{\pi_k}{1-\pi_k} = \frac{1+\delta_k}{1-\delta_k}. $ Define $ r(x) = \frac{p_0}{p_1}(x),\ o_k = \frac{\pi_k}{1-\pi_k}, \ po_k(x) = o_kr(x). $ Then $ \eta_Q(x) = \frac{po_k(x)}{1+po_k(x)} .$
 
 To check for Tsybakov's condition we notice that \begin{align*}
 	&\left| \eta_Q(x) - \frac12 \right| \le z\\
 	\implies & \frac{|po_k(x) -1| }{po_k(x)+1} \le 2z \\
 	\implies & \frac{1-2z}{1+2z} \le po_k(x) \le \frac{1+2z}{1-2z} \\
 	\implies & 1 - 6z \le po_k(x) \le 1+ 6 z \ \text{for } z < \frac13\\
 	\implies & o_k (1-6z) - \frac12 \le \frac{{d/\beta} + d}{2r_0^{d/\beta}} \|x-x_0\|_2^{d/\beta} \le o_k (1+6z) - \frac12  \\
 	\implies & \left[\frac{2r_0^{d/\beta}}{{d/\beta} + d}\left(o_k (1-6z) - \frac12\right)\right]^{\frac{1}{{d/\beta}}} \le \|x-x_0\|_2 \le \left[\frac{2r_0^{d/\beta}}{{d/\beta} + d}\left(o_k (1+6z) - \frac12\right)\right]^{\frac{1}{{d/\beta}}}
  \end{align*}
 The Lebesgue of measure of this region is \[ a(d)\left[\frac{2r_0^{d/\beta}}{{d/\beta} + d}\left(o_k (1+6z) - \frac12\right)\right]^{\frac{d}{{d/\beta}}} - a(d) \left[\frac{2r_0^{d/\beta}}{{d/\beta} + d}\left(o_k (1-6z) - \frac12\right)\right]^{\frac{d}{{d/\beta}}} \le C z^\beta , \] using $ x^a - y^a \le (x-y)^a  $ for $ 0 \le y \le x. $  Now, the density $ q_x = \pi_k p_1 + (1-\pi_k) p_0 $ is bounded above by $ \frac{1+{d/\beta} + d}{2}. $ Hence, \[ Q_X \left( \left| \eta_Q(x) - \frac12 \right| \le z    \right) \le C_\beta z^\beta. \] 
 
 Now  \[ D(Q_0|| Q_1) = \log \left( \frac{\pi_0}{\pi_1}  \right) \pi_0 + \log \left( \frac{1-\pi_0}{1-\pi_1}  \right) (1-\pi_0)  \le \frac c {\sqrt{n}}. \] and $ D(P_0|| P_1)  = 0.$ Hence, \[  D(\Pi_0||\Pi_1) = n_Q D(Q_0|| Q_1)  + n_p D(P_0|| P_1)  = c <1. \]


Also  \[ E_{Q_0} \left|  \eta_0(x) - \frac12 \right| \bbI_{\{f_0^* \neq f_1^*\}} \ge c \left( \frac1{\sqrt{n}}  \right) ^{1+\frac{d}{{d/\beta}}} \ge c \left( \frac1n  \right)^{\frac{1+\beta}{2}}.  \]

Hence, the lower bound is of the form \begin{align*}
	\inf_{\hat f}\sup_{(P,Q)\in \cT} \Ex \left|\eta_Q(x) - \frac12 \right| \bbI_{\{\hat f(X)\neq f^*(X)\}} & \ge c\left( \frac1n  \right)^{\frac{1+\beta}{2}} \left( 1- \left\|\Pi_0 - \Pi_1\right\|_{\text{TV}} \right)\\
	& \ge c'\left( \frac1n  \right)^{\frac{1+\beta}{2}}.
\end{align*}

Combining these two lower bounds, we get the result.
 
\end{proof}


\section{Estimator}
We consider the following notations: $m = (\# \cX_0) \wedge (\# \cX_1)$ and $ \alpha_n = \frac{v\log (2n)+\log (8/\delta)}{n}. $ Here, $ v  $ is the VC dimension of the set $ \{ B(x,r): x \in \reals^d , r>0  \}. $ It can be shown $ v \le d+2. $
 We summarize the classifier below:
\begin{itemize}
	\item[Step 1:]  Define  $ \hat\pi_Q =\frac1{n_Q}\sum_{i=1}^{n_Q}Y_i^Q. $ For $ \phi(x) = \frac{p_0}{p_1}(x) $ we consider the estimator $ \widehat\phi (x) = \frac{\widehat P_0(B(x,r))}{\widehat P_1(B(x,r))}\bbI_{\cE_r(x)}, $ where $\widehat P_i(B(x,r)) = \frac{\#\cX_i \cap  B(x,r)}{\#\cX_i},   $ for $ i = 0,1, $ and the event $ \cE_r(x) $ is defined as $ \cE_r(x) = \left\{ \widehat P_1 (B(x,r)) \ge 72 \alpha_m  \right\}. $ The choice of $ r >0 $ will be specified later.
 
	\item[Step 2:] The class label for $ x $ is estimated by:
	\begin{equation}
		\hat f(x) = \mathbb{I}{\left\{\left(\frac{1-\hat \pi_Q}{\hat \pi_Q}\right) \hat \phi(x)\le  1\right\}}.
		\label{eq:two-sample-classifier}
	\end{equation}

\end{itemize} 

\begin{assumption}
	\begin{enumerate}
		\item $ P_0 $ and $ P_1 $ have same support $ \Omega. $ Furthermore, for any $ x\in [0,1]^d $ and $ r>0, $ $ \lambda \left( B(x,r) \cap \Omega  \right) \ge \lambda   c_\mu\left( B(x,r) \right) .$
		
		\item  There exists some $ \lambda_- >0$ and $ \lambda_+>0, $ such that for any $ x \in \Omega, \ \lambda_- \le \frac{p_0}{p_1}(x) \le \lambda_+. $
		\item There exists some $ \alpha, C_\alpha >0 $ such that the following holds:
		\[ \text{for any }x,x'\in \Omega, \ \left| \frac{p_0}{p_1}(x) - \frac{p_0}{p_1}(x')  \right| \le C_\alpha |x-x'|^\alpha \]
	\end{enumerate}
\end{assumption}


\begin{theorem}[Upper bound]
	Let $ \hat f $ be the classifier defined as above with   $ r  =   (n_P+n_Q)^{-\frac{1}{2\alpha + d}}  .$  Then \[ \sup_{(P,Q)\in \cT} \cE(\hat f) \le C\left( (n_P+n_Q)^{-\frac{2\alpha}{2\alpha+d}} \vee \frac{1}{n_Q} \right)^{\frac{1+\beta}{2}} \] for some constant $ C>0 $ not depending on $ n_P $ or $ n_Q. $
\end{theorem}

\begin{lemma}
	Let  $ X_1, \dots, X_n  $ are independent random variables distributed as $ X_i \sim \text{Ber}(p_i). $ Then for any $ t>0 $ following holds: \[ \Pr \left(\left|\sum X_i - \sum p_i \right| > t \right) \le 2 \exp\left(- \frac{t^2}{4\sum p_i(1-p_i)}  \right). \]
	\label{lemma:bernoulli}
\end{lemma}





\begin{proof}
Consider the following notations: $ \zeta(x) = \left|\left(\frac{1-\pi_Q}{\pi_Q}\right)\phi(x)-1\right|,\ n_k^P = \# \{y_i^{(P)}=k\},$ $ n_k^Q = \# \{y_i^{(Q)}=k\}  $,  $n_k = \# \{y_i = k\} $ for $k=0,1.$
 Then by lemma \ref{lemma:bernoulli} \begin{equation}
 	\Pr \left(|\hat\pi_Q - \pi_Q|  > t \right) \le \exp\left(  - \frac{n_Qt^2}{4 \pi_Q (1- \pi_Q)}  \right),
 	\label{eq:y-target}
 \end{equation}
 Letting $ t^2 = 4\eta^2 \pi_Q (1-\pi_Q), $ we get \[ |\hat\pi_Q - \pi_Q| \le 2\eta\sqrt{\pi_Q (1-\pi_Q)} \] with probability at least $ 1-\exp \left( - \eta^2 n_Q  \right). $
  and \begin{equation}
  	\Pr \left( |n_1 - n_P\pi_P - n_Q\pi_Q | >t   \right)\le 2\exp \left(  - \frac{t^2}{n_P + n_Q}  \right).
  	\label{eq:y-total}
  \end{equation}
  
  Letting $ t = \delta N^{\frac{2\alpha + d/2}{2\alpha + d}},  $ we get \[ \Pr \left( |n_1 - n_P\pi_P - n_Q\pi_Q | >\delta N^{\frac{2\alpha + d/2}{2\alpha + d}}   \right)\le 2\exp \left(  - \delta^2 N^{\frac{2\alpha}{2\alpha + d}}  \right). \]
  
  Hence, with probability $ \ge 1- 2\exp \left(  - \delta^2 N^{\frac{2\alpha}{2\alpha + d}}  \right) $ we have \[ |n_1 - n_P\pi_P - n_Q\pi_Q | \le \delta N^{\frac{2\alpha + d/2}{2\alpha + d}}. \]
  
  Since, we assume that $ n_Q\ge n_Q, $ we see that $ c_kN \le n_k  \le C_k N, $ for $ k =0,1. $
  
  
  Consider the following notations: $ \phi = \frac{p_0}{p_1}, \  m = n_0 \wedge n_1,  $ $ \varepsilon_\phi (x) = \sup_{x' \in B(x,r)} |\phi(x)-\phi(x')|,  $ $ c_n = v\log (2n) + \log (8/\delta) $ and $ e_{n,r}(x) = \sqrt{\frac{24c_{n}}{nP_1 (B(x,r))}}. $
  
  Using Lemma 1 and 2 in [Kpotufe] we get that with probability at least $ 1-2\delta $, the following holds for all $ x \in \Omega $ satisfying $ \cE_r(x): $
  \[ \left| \hat \phi (x) - \phi(x) \right| \le e_{n_1,r}(x) \phi(x) + 2 \left(  e_{n_0,r}(x) \sqrt{\phi (x) + \varepsilon_\phi(x,r)} + e^2_{n_0,r}(x) + \varepsilon_\phi(x,r)  \right) \]
  
  Here, $ \varepsilon_\phi(x,r) \le C_\alpha r^\alpha $  and $ e_{n,r} (x) \le \sqrt{\frac{24 (v\log (2n)+ \log(8/\delta))}{n\mu c_d r^d}} .$ Hence, the above inequality can be simplified as: \[ \left| \hat \phi (x) - \phi(x) \right| \le   C_1\sqrt{\frac{24 (v\log (2m)+ \log(8/\delta))}{m\mu c_d r^d}} + C_2 r^\alpha  \]
  Letting $ \delta = 8\times (2m)^{d+1} \exp\left(-\eta^2 \mu c_d m^{\frac{2\alpha}{2\alpha+d}} \right)  $ we get \[ \left| \hat \phi (x) - \phi(x) \right| \le   C_1\eta + C_2 r^\alpha. \]
    Now, \begin{align*}
  	\left|  \frac{1- \hat \pi_Q}{\hat\pi_Q} \hat \phi (x) - \frac{1- \pi_Q}{\pi_Q} \phi(x) \right| \le & \left|  \frac{1- \hat \pi_Q}{\hat\pi_Q}  - \frac{1- \pi_Q}{\pi_Q}  \right|\hat \phi (x) + \frac{1- \pi_Q}{\pi_Q}  \left| \hat \phi (x) - \phi(x) \right| \\
  	 \le & \left|  \frac{1- \hat \pi_Q}{\hat\pi_Q}  - \frac{1- \pi_Q}{\pi_Q}  \right| \left(\phi (x) + C_1 \eta + C_2 r^\alpha\right)+ \frac{1- \pi_Q}{\pi_Q}   \left( C_1 \eta +C_2 r^{\alpha}\right) \\
  	  \le & \frac{|\hat \pi_Q - \pi_Q|}{\hat \pi_Q \pi_Q} \left(\phi (x) + C_1 \eta + C_2 r^\alpha\right)+ \frac{1- \pi_Q}{\pi_Q}   \left( C_1 \eta +C_2 r^{\alpha}\right)
  \end{align*}
  
 
  
  Using $ \left| \frac{1}{1+x'} - \frac1{1+x} \right| = \frac{|x'-x|}{(1+x)(1+x')} $ we get \begin{align*}
  	\left| \frac1{1+\frac{1- \hat \pi_Q}{\hat\pi_Q} \hat \phi (x)}  - \frac1{1+\frac{1- \pi_Q}{\pi_Q} \phi(x)} \right| & \le \frac{\frac{|\hat \pi_Q - \pi_Q|}{\hat \pi_Q \pi_Q} \left(\phi (x) + C_1 \eta + C_2 r^\alpha\right)+ \frac{1- \pi_Q}{\pi_Q}   \left( C_1 \eta +C_2 r^{\alpha}\right)}{\left(1+\frac{1- \hat \pi_Q}{\hat\pi_Q} \hat \phi (x)\right)\left(1+\frac{1- \pi_Q}{\pi_Q} \phi(x)\right)} \\
  	& \le \frac{\left(\phi (x) + C_1 \eta + C_2 r^\alpha\right)|\hat \pi_Q - \pi_Q|}{\left(\hat \pi_Q+ (1-\hat\pi_Q)\hat\phi(x)\right)\left( \pi_Q+ (1-\pi_Q)\phi(x)\right)} + \frac{C_1\eta + C_2 r^\alpha}{\lambda_-} \\
  	& \le \frac{\left(\lambda_+ + C_1 \eta + C_2 r^\alpha\right)\eta'}{\left(\lambda_- -C_1 \eta - C_2 r^\alpha \right)\lambda_-} + \frac{C_1\eta + C_2 r^\alpha}{\lambda_-} \\
  	& \le C_4 \eta' + C_5 \eta + C_6 r^\alpha\le \xi/2
  \end{align*} with probability at least $ 1 - \exp\left(-C_6\xi^2N^{\frac{2\alpha}{2\alpha + d}} \right) - \exp\left(-C_7\xi^2 n_Q\right)\ge 1 - \exp\left(-\xi^2\left(C_6N^{\frac{2\alpha}{2\alpha + d}} \wedge C_7 n_Q\right)\right). $
  Hence, \[ \sup_{\Pr \in \cP}\Pr\left( \left| \hat \eta_Q(X) - \eta_Q(X) \right| > \xi   \right) \le  \exp\left(-\xi^2\left(C_6N^{\frac{2\alpha}{2\alpha + d}} \wedge C_7 n_Q\right)\right). \]
  
  To get a bound for the generalization error we define the following events: $$ A_0 = \left\{ x\in \reals^d: 0< \left| \eta_Q(x) - \frac12\right| < \xi        \right\}  \text{ and for }j \ge 1, \ A_j = \left\{ x\in \reals^d: 2^{j-1}< \left| \eta_Q(x) - \frac12\right| < 2^j\xi        \right\}  $$ Now, \begin{align*}
  	\cE(\hat f)  = & 2 \Ex \left(\left| \eta_Q(X) -\frac12 \right|\bbI_{\{\hat f(X)\neq f^*(X)\}}  \right) \\
  	 = & 2\sum_{j=0}^\infty \Ex\left(\left| \eta_Q(X) -\frac12 \right|\bbI_{\{\hat f(X)\neq f^*(X)\}} \bbI_{\{X\in A_j\}} \right) \\
  	 \le & 2 \xi \Ex\left( 0< \left| \eta_Q(X) -\frac12 \right|< \xi  \right) \\
  	 & + 2\sum_{j=1}^\infty \Pr\left(\left| \eta_Q(X) -\frac12 \right|\bbI_{\{\hat f(X)\neq f^*(X)\}} \bbI_{\{X\in A_j\}} \right)
  \end{align*}
  On the event $ \{ \hat f\neq f^*  \} $ we have $ \left| \eta_Q - \frac12 \right| \le \left| \hat \eta - \eta \right|. $ So, for any $ j \ge 1 $ we get \begin{align*}
  	\Ex &\left(\left| \eta_Q(X) -\frac12 \right|\bbI_{\{\hat f(X)\neq f^*(X)\}} \bbI_{\{X\in A_j\}} \right) \\
  	& \le 2^{j+1}\xi \Ex \left(\bbI_{\{|\hat \eta_Q(X)- \eta_Q(X)| \ge2^{j-1}\xi \}} \bbI_{\{0< |\eta_Q(X)-1/2|<2^{j}\xi\}} \right) \\
  	& = 2^{j+1}\xi \Ex_X \left[\Pr\left(\bbI_{\{|\hat \eta_Q(X)- \eta_Q(X)| \ge2^{j-1}\xi \}}\right) \bbI_{\{0< |\eta_Q(X)-1/2|<2^{j}\xi\}} \right] n\\
  	& \le 2^{j+1}\xi \exp\left(-a(2^{j-1}\xi)^2\right)\Pr_X (0< |\eta_Q(X)-1/2|<2^{j}\xi)\\
  	& \le 2C_\beta 2^{j(1+\beta)}\xi ^{1+\beta} \exp\left(-a(2^{j-1}\xi)^2\right).
  \end{align*} where $ a = C_6N^{\frac{2\alpha}{2\alpha + d}} \wedge C_7 n_Q. $
  Letting $ \xi = \left(C_6N^{\frac{2\alpha}{2\alpha + d}} \wedge C_7 n_Q\right)^{-\frac12} $ we get \begin{align*}
  	\sup_{\Pr \in \cP}\cE(\hat f) & \le 2C_\beta \left( \xi^{1+\beta} + \sum_{j\ge 1}  2^{j(1+\beta)} \xi^{1+\beta}\exp\left(-a(2^{j-1}\xi)^2\right)   \right) \\
  	& \le C \left(N^{\frac{2\alpha}{2\alpha + d}} \wedge n_Q\right)^{-\frac{1+\beta}{2}}.
  \end{align*}
\end{proof}


\section{Adaptive choice of $r$: A Lepski type method}

Consider a noise surrogate for $ \frac{1-\pi_Q}{\pi_Q} \phi(x) $ as  \[ \hat v(x,r) =  \begin{cases}
\frac{1-\hat\pi_Q}{\hat\pi_Q} \sqrt{\frac{24 \alpha_m}{\hat P_1 (B(x,r))}} & \text{if } \cE_r(x) \\
\frac{1-\hat\pi_Q}{\hat\pi_Q} \frac1{\sqrt 3} & \text{otherwise}
\end{cases} \] and signal surrogate as \[ \hat s(x,r) = \left| \frac{1-\hat\pi_Q}{\hat\pi_Q} \hat \phi(x) - 1 \right|. \]
\begin{algorithm}[H]
	\SetAlgoLined
	\textbf{Input: } $ x, \{(X_i^P,Y_i^P)\}_{i=1}^{n_P},  \{(X_i^Q,Y_i^Q)\}_{i=1}^{n_Q}$ \;
	$ r = 2  $ \;
	\Do{$ \text{SNR} > (d+3) \log(n_P+n_Q)  $}{
		$ r \gets \frac r2 $ \;
		$ \text{SNR} = \frac{\hat s(x,r)}{\hat v(x,r)} $\;
	}
	\textbf{Output: } $ \hat f (x) = \bbI{\left\{  \frac{1-\hat \pi_Q}{\hat \pi_Q} \hat \phi(x)  < 1  \right\}} $
	\caption{Data driven choice of $ r $ (Lepski type algorithm)}
\end{algorithm}


==> macros.tex <==
\usepackage{amsmath}
\newcommand{\BALD}{\begin{aligned}}
\newcommand{\EALD}{\end{aligned}}
\newcommand{\BALDS}{\begin{aligned*}}
\newcommand{\EALDS}{\end{aligned*}}
\newcommand{\BCAS}{\begin{cases}}
\newcommand{\ECAS}{\end{cases}}
\newcommand{\BEAS}{\begin{eqnarray*}}
\newcommand{\EEAS}{\end{eqnarray*}}
\newcommand{\BEQ}{\begin{equation}}
\newcommand{\EEQ}{\end{equation}}
\newcommand{\BIT}{\begin{itemize}}
\newcommand{\EIT}{\end{itemize}}
\newcommand{\BMAT}{\begin{bmatrix}}
\newcommand{\EMAT}{\end{bmatrix}}
\newcommand{\BNUM}{\begin{enumerate}}
\newcommand{\ENUM}{\end{enumerate}}
\newcommand{\eg}{e.g.}
\newcommand{\Eg}{E.g.}
\newcommand{\ie}{i.e.}
\newcommand{\cf}{cf.}
\newcommand{\etc}{etc.}
\newcommand{\BA}{\begin{array}}
\newcommand{\EA}{\end{array}}

\newcommand{\ones}{\mathbf 1}
\newcommand{\zeros}{\mathbf 0}

% std math stuff
\newcommand{\reals}{\mathbf{R}}
\newcommand{\complex}{\mathbf{C}}
\newcommand{\integers}{\mathbf{Z}}
\newcommand{\symm}{\mathbf{S}}  % symmetric matrices


\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
\newcommand{\diag}{\mathop{\mathbf{diag}}}
\DeclareMathOperator{\Expect}{\mathbf{E}}
\DeclareMathOperator*{\maximize}{maximize}
\DeclareMathOperator*{\minimize}{minimize}
\newcommand{\nullspace}{\mathcal{N}}
% \newcommand{\Prob}{\mathop{\mathbf{Pr}}}
\renewcommand{\Pr}{\mathbf{Pr}}
\DeclareMathOperator{\rank}{rank}
\newcommand{\range}{\mathcal{R}}
\DeclareMathOperator{\sign}{sign}
\newcommand{\subjectto}{\textrm{subject to}}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\var}{\mathbf{var}}

\newcommand{\pc}{\hspace{1pc}}

\newcommand{\abs}[1]{\left| #1 \right|}

\DeclareMathOperator{\linspan}{span}
\newcommand{\norm}[1]{\left\| #1 \right\|}

\newcommand{\iid}{\emph{i.i.d.}}
\newcommand{\whp}{\emph{w.h.p.}}
\DeclareMathOperator{\cov}{\mathbf{cov}}
\newcommand{\erfc}{\mathop{\textrm{erfc}}}
\DeclareMathOperator{\logdet}{\log\det}

\DeclareMathOperator{\cone}{cone}
\DeclareMathOperator{\conv}{conv}
\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\ext}{ext}
\DeclareMathOperator{\prox}{prox}
\DeclareMathOperator{\relint}{relint}

==> more-proofs.tex <==
%\appendix
	
%	\section{Extension: multiple source distributions}
%	\label{appendix:extension-ts}
%	In this section we extend the theory of transfer learning under target shift setup, when multiple source distributions are present. Let's assume the presence of $ m $ many source distributions denoted as $ P_k, \ k = 1,\dots , m. $ As before, we denote the target distribution as $ Q. $ We make that following structural assumptions for the tuples of distributions $ (P_1, \dots P_m, Q) $: 
%	
%	\begin{definition}[Distribution class]
%		$ \Pi $ is defined as the class of all tuples of distributions $ (P_1, \dots P_m, Q) $ which satisfies the followings:
%		\begin{enumerate}
%			\item $ P_1, \dots P_m, Q $ are distributions defined on $ [0,1]^d \times \{0,1\}. $
%			\item For some probability distributions $ G_0, G_1 $ defined on $ [0,1]^d $ we assume  $ G_i=  P_k(\cdot | Y=i) = Q(\cdot | Y=i) $ for $ i = 0,1 $ and any $ k = 1, \dots, m $.
%			\item $  Q_X $ satisfies strong density assumption as in definition \ref{def:strong-density} with parameters $ \mu = (\mu_-, \mu_+), c_\mu>0, r_\mu>0 $,
%			\item $ G_0 $ and $ G_1 $ have common support $ \Omega, $
%			\item Let $ \pi_{P_k} = P_k(Y = 1) $. For some $ \epsilon>0,$ and any $ k, $ $ \ \epsilon \le \pi_{P_k} \le 1-\epsilon,  $ 
%			\item The density ratio $ \ratio $ is  $ (C_\alpha, \alpha) $-H\"older smooth (see definition \ref{def:holder-smooth}),
%			\item $ \eta_Q $ satisfies margin condition with parameter $ \beta $ (see definition \ref{def:margin-condition}),
%			\item $ \alpha\beta \le d. $
%		\end{enumerate}
%	\end{definition}
%
%
%For a tuple $ (P_1, \dots P_m, Q) \in \Pi  $ let \begin{align*}
%	 \left(X_1^{P_1},Y_1^{P_1} \right), \dots , \left(X_{n_{P_1}}^{P_1},Y_{n_{P_1}}^{P_1} \right) & \stackrel{\iid}{\sim } P_1\\
%	 \left(X_1^{P_2},Y_1^{P_2} \right), \dots , \left(X_{n_{P_2}}^{P_2},Y_{n_{P_2}}^{P_2} \right) & \stackrel{\iid}{\sim } P_2\\
%	 \dots \hspace{2cm} &\\
%	 \left(X_1^{P_m},Y_1^{P_m} \right), \dots , \left(X_{n_{P_m}}^{P_m},Y_{n_{P_m}}^{P_m} \right) & \stackrel{\iid}{\sim } P_m\\
%	 \left(X_1^{Q},Y_1^{Q} \right), \dots , \left(X_{n_{Q}}^{Q},Y_{n_{Q}}^{Q} \right) & \stackrel{\iid}{\sim } Q
%\end{align*}
%
%Let us denote $ Z $ to be the set of all sample points, \ie, \[ Z = \left\{ \left(X_1^{P_1},Y_1^{P_1} \right), \dots , \left(X_{n_{P_1}}^{P_1},Y_{n_{P_1}}^{P_1} \right);\dots ; \left(X_1^{P_m},Y_1^{P_m} \right), \dots , \left(X_{n_{P_m}}^{P_m},Y_{n_{P_m}}^{P_m} \right); \left(X_1^{Q},Y_1^{Q} \right), \dots , \left(X_{n_{Q}}^{Q},Y_{n_{Q}}^{Q} \right)    \right\}. \] The classifier $ \hat f $ constructed from $ Z $ is similar as in \ref{sec:classifier}. The following theorem gives the upper bound for excess risk: 
%\begin{theorem}[Upper bound]
%	\label{th:upper-bound-ex}
%	Let $ \hat f $ be the classifier defined as above with   $ r  =   m^{-\frac{1}{2\alpha + d}}  .$  Then \[ \sup_{(P,Q)\in \Pi} \Ex \cE_Q(\hat f) \le C\left( \left(\sum_{ k =1}^m n_{P_k}+n_Q\right)^{-\frac{2\alpha}{2\alpha+d}} \vee \frac{1}{n_Q} \right)^{\frac{1+\beta}{2}} \] for some constant $ C>0 $ independent of $ n_P $ and $ n_Q. $
%\end{theorem} 
%
%\begin{remark}
%	As before, choice of the bandwidth parameter $ r $ depends on the unknown smoothness parameter $ \alpha. $ One way to get a data-driven choice of $ r $ is to use Lepski type algorithm (see \citet{lepski1997optimal}). 
%\end{remark}
%The following lower bound shows that the classifier $ \hat f $ is rate optimal in terms of excess risk. 
%
%\begin{theorem}[{Lower bound}]
%	\label{th:lower-bound-ex}
%	There exists a constant $ c>0 $ independent of  $ n_P $ and $ n_Q $ such that 
%	\[ \inf_{\hat f} \sup_{(P,Q)\in \Pi} \Ex \cE_Q(\hat f)   \ge c\left( \left(\sum_{ k =1}^m n_{P_k}+n_Q\right)^{-\frac{2\alpha}{2\alpha+d}} \vee \frac{1}{n_Q} \right)^{\frac{1+\beta}{2}}. \]
%\end{theorem}
%
%The proofs of Theorems \ref{th:upper-bound-ex} and \ref{th:lower-bound-ex} are similar the proofs of Theorems \ref{th:upper-bound} and \ref{th:lower-bound}. Theorems \ref{th:upper-bound} and \ref{th:lower-bound} together establish the minimax rate for transfer learning under target shift is: 
%\begin{equation}
%\inf_{\hat f} \sup_{(P,Q)\in \Pi} \Ex \cE_Q(\hat f)  \asymp\left( \left(\sum_{ k =1}^m n_{P_k}+n_Q\right)^{-\frac{2\alpha}{2\alpha+d}} \vee \frac{1}{n_Q} \right)^{\frac{1+\beta}{2}}.
%\label{eq:minimax-rate-ex}
%\end{equation} 
%
%	
	
\newpage	
\section{Supplementary Results and Proofs}
\label{sec:supp-results}

\subsection{Preliminaries}

In this section, we collect the basic results that we repeatedly appeal to in our proofs.

% \begin{lemma}
% 	Let  $ X_1, \dots, X_n  $ are independent random variables distributed as $ X_i \sim \text{Ber}(p). $ Then for any $ t>0 $ the following holds: \[ \Pr \left(\left|\bar X - p \right| > t \right) \le 2 \exp\left(- \frac{nt^2}{4}  \right). \]
% 	\label{lemma:bernoulli}
% \end{lemma}


% \begin{proof}
% 	From Bernstein's inequality:
% 	\[ \text{for any }\lambda>0, \ P\left( |\sum X_i - np|>\lambda   \right) \le 2 \exp \left( - \frac{\lambda^2/2}{np + \lambda/3 }  \right). \] Letting $ \lambda = nt $ we see \begin{align*}
% 		P\left( |\sum X_i - np|>nt   \right) &\le 2 \exp \left( - \frac{n^2t^2/2}{np + nt/3 }  \right)\\
% 		&\le 2 \exp \left( - \frac{nt^2/2}{p + t/3 }  \right)\\
% 		& \le 2 \exp \left( - \frac{nt^2/2}{2 }  \right) \text{ for } t \le 3\\
% 	\end{align*}
% 	Note that $ |\bar X-p| \le 2. $ Hence, we have the inequality for all $ t>0. $
% \end{proof}


% \begin{lemma}
% 	\label{lemma:kl-ineq}
%  Let $ (\Omega, \cA, P) $ be a probability space. 	For a random vector $ X $ on this probability space  let us define $ \mu_X $ to be the measure induced by it. Let $ X $ and $ Y $ are two random vectors, which take values in the same space $ \Omega' $ and $ f $ is a function defined on the domain $ \Omega' $ such that $ f(X) $ and $ f(Y) $ are measurable. Then \[ D\left(\mu_{f(X)} |\mu_{f(Y)}\right) \le D(\mu_X|\mu_Y), \] where $ D(\mu|\nu) $ is the Kulback-Leibler divergence between two distribution $ \mu $ and $ \nu. $
% \end{lemma}

\begin{lemma}[Varshamov-Gilbert bound]
	\label{lemma:varshamov-gilbert}
	Let $ m\ge 8. $ Then there exists a subset $ \{ \sigma_0,\ldots , \sigma_M \} \subset \{-1,1\}^m $ such that $ \sigma_0 = (1 ,\ldots, 1), $ \[ \rho_H(\sigma_i , \sigma_j ) \ge \frac m 8, \ \text{for all } 0\le i<j\le M,\ \text{and } M \ge 2^{m/8}, \] where, $ \rho_H $ is the hamming distance. 
\end{lemma}



% 	\begin{lemma}[\citet{bousquet2003introduction}]
% 		\label{lemma:convergence-vc-bound}
% 	Let $ X_1, \dots, X_n \sim \nu $ for some probability measure $ \nu  $ defined on $ \cX. $	Let $ \cF $ be some collection of measurable functions defined on $ \cX $ with VC dimension $ d_\cF. $ Let $ 0< \delta <1. $ Define $ \alpha_n = \frac{d_\cF\log (2n)+ \log(1/\delta)}{n} $ and $ \nu_n $ to be  the empirical distribution. For a measure $ \mu  $ on $ \cX $ and a measurable function $ f: \cX\to R $  define $ \mu(f) = \int fd\mu. $  Then with probability at least $ 1-\delta $ over the sampling, all $ f \in \cF $ satisfy \begin{align*}
% 	\nu( f) &\le \nu_n (f) + \sqrt{\nu_n (f) \alpha_n} + \alpha_n, \text{ and,}\\
% 	\nu_n (f) & \le 	\nu (f) + \sqrt{\nu (f)\alpha_n} + \alpha_n.
% 	\end{align*}
% \end{lemma}

% \begin{corollary}
% 	Consider the setup in lemma \ref{lemma:convergence-vc-bound}. Then with  probability at least $  1-\delta  $ for all $ f \in \cF $ the following holds  \[ |\nu_n(f) - \nu(f)| \le \sqrt{(3\nu(f)+2\alpha_n)\alpha_n} + \alpha_n. \]
% 	\label{cor:empirical-convergence}
% \end{corollary}



\subsection{Proof of results in section \ref{sec:labeled-target}}

% \begin{proof}[\bf{Proof of theorem \ref{th:lower-bound}}]
% 	\label{pr:lower-bound}
% 	The first part of the proof deals with $ (n_P+n_Q)^{- \frac{\alpha(1+\beta)}{2\alpha + d}} $ rate. The construction of distribution class is adapted from  \cite{kpotufe2018Marginal}. The second part deals with rate $ n_Q^{- \frac{1+\beta}{2}}. $
	
% \noindent	\textbf{Part I:} 
	
% 	Let $  d_0 = 2 + \frac d \alpha,  $ $ r = c_r N^{-\frac1{\alpha d_0}} ,\ m = \lfloor c_m r^{\alpha\beta -d} \rfloor,\ w = c_w r^d ,$ where, $ N = n_P+n_Q,\ c_r = \frac19, \ c_m = 8\times 9^{\alpha\beta - d},\ 0<c_w \le 1 $ to be chosen later. 
	
% 	For such a choice we have $ 8\le m < \lfloor r^{-1} \rfloor ^d. $ As, $ \alpha\beta \le d, $ we have $ r \le \frac19. $ This implies $ c_m r^{\alpha\beta -d} \ge 8. $  Since $ r^{-1} \ge 8 $ which gives us $ r^{-1} \le \frac{9\lfloor r^{-1}\rfloor}{8}. $ Therefore, $ c_mr^{\alpha\beta -d} = 8 (9r)^{\alpha\beta}\left( \frac{r^{-1}}{9}\right) < 8^{1-d } \lfloor r^{-1} \rfloor ^d  \le \lfloor r^{-1} \rfloor ^d.$ 
	
% 	$ mw = mc_w r^d <1. $
	
% 	\textbf{Construction of $ g_0 $ and $ g_1: $}
% 	Divide $ \cX = [0,1]^d $ into $ \lfloor r^{-1} \rfloor ^d $ hypercubes of length $ r. $ Let $ \cZ $ be the set of their centers. Let $ \cZ_1 \subset \cZ $ such that $ \left|\cZ_1 \right| = m. $ Let $ \cZ_0 = \cZ \backslash \cZ_1,\ \cX_1 = \cup_{z\in\cZ_1} B\left( z,\frac r6  \right), \text{and } \cX_0 = \cup_{z\in\cZ_0} B\left( z,\frac r2  \right). $ Let $ q_1 = \frac w{\text{Vol}\left( B\left(z,\frac r6\right)  \right)}, \text{ and } q_0 = \frac{1-mw}{\text{Vol}\left(\cX_0\right)}.$  For $ \sigma \in \{-1,1\}^{\cZ_1}, $ define \[ g_1^\sigma (x) = \begin{cases}
% 	a^\sigma q_1 \left(1+\sigma(z)C_\alpha'r^\alpha\right) & x \in B\left(z,\frac r6  \right), \ z \in \cZ_1,\\
% 	a^\sigma q_0 & x \in B\left(z,\frac r2  \right), \ z \in \cZ_0,\\
% 	0 & \text{otherwise},
% 	\end{cases} \] and, \[ g_0^\sigma (x) = \begin{cases}
% 	b^\sigma q_1 \left(1-\sigma(z)C_\alpha'r^\alpha \right) & x \in B\left(z,\frac r6  \right), \ z \in \cZ_1,\\
% 	b^\sigma q_0 & x \in B\left(z,\frac r2  \right), \ z \in \cZ_0,\\
% 	0 & \text{otherwise},
% 	\end{cases} \] where, $ C_\alpha' = \min \left\{ C_\alpha 6^{-\alpha}, 1-2\epsilon, \frac12  \right\}. $ The constant $  \epsilon $ comes from the assumption that $ \epsilon \le \pi_P \le 1- \epsilon. $
	
% 	We want $ \int g_1^\sigma (x) dx = a^\sigma \left[ mw + (1-mw) + w\sum_{z\in\cZ_1} \sigma(z) C_\alpha'r^\alpha \right] = 1. $ Hence, $ a^\sigma = \frac1 {1+ w\sum_{z\in\cZ_1} \sigma(z)C_\alpha'r^\alpha}. $ Also, $ b^\sigma = \frac1 {1- w\sum_{z\in\cZ_1} \sigma(z)C_\alpha'r^\alpha}. $ Also, we want $ \frac{a^\sigma q_0 \pi_Q ^\sigma   }{b^\sigma q_0 \left(1-\pi_Q ^\sigma  \right)} = 1, $ which implies $ \pi_Q ^\sigma = \frac{1/a^\sigma}{1/a^\sigma + 1/b^\sigma} = \frac 12 \left( 1+ w  \sum_{z\in\cZ_1} \sigma(z) C_\alpha' r^\alpha \right)  . $ We have freedom to choose $ \pi_P^\sigma>0. $ Set $ \pi_P^\sigma = \frac 12 \left( 1+ w  \sum_{z\in\cZ_1} \sigma(z) C_\alpha' r^\alpha \right)  . $ 
	
% 	Then \[ \frac{1-\pi_Q^\sigma}{\pi_Q^\sigma} \frac{g_0^\sigma(x)}{g_1^\sigma(x)} = \begin{cases}
% 	\frac{1- \sigma(z)C_\alpha' r^\alpha}{1+ \sigma(z)C_\alpha' r^\alpha} & \text{if } x\in \cX_1,\\
% 	1 & \text{if } x\in \cX_0.
% 	\end{cases} \] 
% 	Then $ \eta_Q^\sigma(x) = \begin{cases}
% 	\frac{1+ \sigma(z)C_\alpha' r^\alpha}{2} & \text{if } x\in \cX_1,\\
% 	\frac12 & \text{if } x\in \cX_0.
% 	\end{cases} $ 
	
% 	So, $ \eta_Q^\sigma $ simplifies to \[ \eta_Q^\sigma(x) = \begin{cases}
% 	\frac{1+ \sigma(z)C_\alpha'r^\alpha}{2} & \text{if } x\in B\left( z,\frac r6 \right),\ z\in\cZ_1\\
% 	\frac12 & \text{if } x\in\cX_0.
% 	\end{cases}. \] 
% 	Extend it to \[ \eta_Q^\sigma(x) = \begin{cases}
% 	\frac{1+ \sigma(z)C_\alpha'r^\alpha}{2} & \text{if } x\in B\left( z,\frac r6 \right),\ z\in\cZ_1\\
% 	\frac12 & \text{otherwise.}
% 	\end{cases}. \] 
% 	The marginal density of $ X $ under the distribution $ Q $ is \[q_X = \pi_Q^\sigma g_1^\sigma + (1-\pi_Q^\sigma) g_0^\sigma= \begin{cases}
% 	q_1 & \text{for } x\in \cX_1,\\
% 	q_0 & \text{for } x \in \cX_0.
% 	\end{cases}\] 
	
	
% 	For $ x\in B\left(z,\frac r6 \right), \ z\in \cZ_1, $ \begin{align*}
% 	q_X(x) & = \pi_Q^\sigma g_1^\sigma(x) + (1-\pi_Q^\sigma) g_0^\sigma(x)\\
% 	& = a^\sigma q_1 \left(1+\sigma(z)C_\alpha'r^\alpha \right) \frac1{2a^\sigma}  + b^\sigma q_1 \left(1-\sigma(z)C_\alpha'r^\alpha \right) \frac1{2b^\sigma}\\
% 	& = q_1.
% 	\end{align*}
	
% 	For $ x\in B\left(z,\frac r2 \right), \ z\in \cZ_0, $ \begin{align*}
% 	q_X(x) & = \pi_Q^\sigma g_1^\sigma(x) + (1-\pi_Q^\sigma) g_0^\sigma(x)\\
% 	& = a^\sigma q_0  \frac1{2a^\sigma}  + b^\sigma q_0  \frac1{2b^\sigma}\\
% 	& = q_0.
% 	\end{align*}
	
% 	\textbf{Checking for $ \epsilon \le \pi_P^\sigma \le 1- \epsilon  $:}\\
% 	In the expression $ \pi_P^\sigma = \frac 12 \left( 1+ w  \sum_{z\in\cZ_1} \sigma(z) C_\alpha' r^\alpha \right)  $ first we try to get a bound for $ w  \sum_{z\in\cZ_1} \sigma(z) C_\alpha' r^\alpha.  $ Note that \begin{align*}
% 		\left| w  \sum_{z\in\cZ_1} \sigma(z) C_\alpha' r^\alpha  \right|  & \le  w  \sum_{z\in\cZ_1}  C_\alpha' r^\alpha\\& \le mw C_\alpha' r^\alpha \\
% 		 & \le C_\alpha'r^{\alpha} \le 1-2\epsilon.
% 	\end{align*} Hence, $ \pi_P^\sigma \ge \frac12 (1 - (1-2\epsilon)) = \epsilon $ and  $ \pi_P^\sigma \le \frac12 (1 + (1-2\epsilon)) = 1- \epsilon. $
	
% 	\textbf{Checking local $ \alpha $-H\"older condition for  $ g_0 $ and $ g_1 $:} Note that 
% 	We shall verify the local smoothness condition for  $ g_1. $ Exact same steps can be followed  to verify smoothness for $ g_0. $ 
	
% 	Since we are interested in limiting smoothness (see definition \ref{def:holder-smooth}) we set our biggest radius of interest to be $ \frac r6. $ We shall show that for any $ x, x' \in \Omega $ with $ \|x-x'\| \le \frac r6 $ \[ \frac{|g_1(x)-g_1(x')|}{\|x-x'\|^\alpha} \le C_\alpha. \] Note that, $ x, x' \in \Omega $ with $ \|x-x'\| \le \frac r6 $ implies the following possible cases:
% 	\begin{enumerate}
% 		\item $ x, x' \in B(z, r/2) $ for some $ z \in \cZ_0. $ In that case, \[ |g_1(x) - g_1(x')| = |a^\sigma q_0 - a^\sigma q_0| = 0 \] and the inequality  holds trivially. 
% 		 \item $ x, x' \in B(z, r/6) $ for some $ z \in \cZ_1. $ In that case,  \[ |g_1(x) - g_1(x')| = |a^\sigma q_1 (1+ \sigma(z) C_\alpha' r^\alpha ) - a^\sigma q_1(1+ \sigma(z) C_\alpha' r^\alpha )| = 0 \] and the inequality  holds trivially again.
% 		 \item $ x \in B(z, r/2) $ and $ x' \in B(z', r/2) $ for some $ z, z' \in \cZ. $ In that case  \[ \|x-x'\| \ge \|z-z'\| - \|x-z\|-\|x'-z'\| \ge r > \frac r 6. \] So, this an invalid case.
% 	\end{enumerate}
	
% 	\textbf{Checking Tsybakov's noise condition:} \\
% 	For $ t < C_\alpha' r^\alpha/2,$ \[  Q_X^\sigma \left( 0< \left| \eta_Q^\sigma(X) -\frac12 \right| \le t \right) =0. \] 
% 	For $ t\ge C_\alpha' r^\alpha/2, $ \begin{align*}
% 	Q_X \left( 0< \left| \eta_Q(X) -\frac12 \right| \le t \right) &  = mw\\
% 	& \le c_mc_w r^{\alpha \beta}\\
% 	& \le C_\beta \left( \frac{C_\alpha' r^\alpha}{2}  \right)^\beta.
% 	\end{align*}
	
% 	\begin{align*}
% 	\cE_{Q^\sigma}(h) & = 2\Ex _{Q_X} \left[\left | \eta_Q^\sigma(X) - \frac12 \right | \mathbf{1}\left( h(X) \neq h^*_\sigma(X)  \right)\right]\\
% 	& = C_\alpha' r^\alpha Q_X\left( \{h(X) \ne h_\sigma^*(X)  \} \cap \cX_1 \right).
% 	\end{align*}
%  We set $ \pi_Q^\sigma = \pi_P^\sigma. $  
	
% 	Let $ \cF $ be the set of all classifier relevant to this classification problem. For $ h,h'\in\cF $ define $ \bar\rho (h,h') \coloneqq C_\alpha' r^\alpha Q_X \left( \{h(X)\neq h'(X)\} \cap \cX_1 \right). $ For $ \sigma\in\{-1,1\}^m, $ let $ h_\sigma^* $ be the Bayes classifier defined as $ h_\sigma^* (x) = \mathbf{1}\{\eta_Q^\sigma(x) \ge 1/2\}. $ Then, for $ \sigma, \sigma'\in\{-1,1\}^m, $  $ \bar\rho (h_\sigma^*, h_{\sigma'}^*) = C_\alpha' r^\alpha w \rho_H(\sigma, \sigma'), $ where, $ \rho_H(\sigma,\sigma') $ is the Hamming distance defined as $ \rho_H(\sigma,\sigma') \coloneqq \text{card} \{z\in\cZ_1 :\sigma(z) \neq \sigma'(z) \}. $
	
	
	
% 	Let $\{ \sigma_0,\ldots , \sigma_M \} \subset \{-1,1\}^m  $ be the choice obtained from the  lemma \ref{lemma:varshamov-gilbert}. For each $ i \in \{0,\ldots,M\} $ let us set the distributions of two populations to be $ (P^i, Q^i) = (P^{\sigma_i}, Q^{\sigma_i}). $ The joint distribution of $ (\bX,\bY) $ is set at $ \Pi_i = {P^i}^{\otimes n_p} \otimes {Q^i}^{\otimes n_Q} = {Q^i}^{\otimes (n_P+n_Q)}.$
	
% 	Denote $ h_{\sigma_i}^* $ by $ h_i^* .$ For $ 0\le i<j\le M, $ \begin{align*}
% 	\bar\rho (h_i^*,h_j^*) &\ge C_\alpha' \frac{wmr^\alpha }{8}\\ 
% 	&\ge \frac12 C_\alpha' c_r^\alpha (n_P+n_Q)^{-\frac1{d_0}} c_mr^{\alpha\beta -d} c_w r^d \\
% 	& \ge C (n_P+n_Q)^{-\left(\frac{1}{d_0} +\frac{\alpha\beta}{\alpha d_0} \right)}\\
% 	& = C (n_p+n_Q)^{-\frac{1+\beta}{d_0}}\\
% 	& \triangleq 2s.
% 	\end{align*}
	
% 	Let $ D(P|Q) $ be the KL-Divergence between the distributions $ P $ and $ Q. $ Then $ D(\Pi_i| \Pi_0) = n_P D(P^i|P^0) + n_Q D(Q^i|Q^0) = (n_P+n_Q) D(Q^i|Q^0). $ Now, \begin{align*}
% 	D(Q^i|Q^0) & = \int \log\left( \frac{dQ^i}{dQ^0}  \right) dQ^i\\
% 	 = & \int \left[ \log \left( \frac{\eta_Q^i (x)}{\eta_Q^0(x)}  \right) \eta_Q^i(x) + \log \left( \frac{1-\eta_Q^i (x)}{1-\eta_Q^0(x)}  \right) (1-\eta_Q^i(x))  \right] dQ_X\\
% 	 = & \sum_{z: \sigma_i(z) \neq \sigma_0(z)} Q_X \left(B\left( z,\frac r6  \right)  \right) \Bigg[ \log \left( \frac{1+ C_\alpha'r^\alpha}{1- C_\alpha'r^\alpha}  \right) \frac{1+ C_\alpha'r^\alpha}{2} \\
% 	 & +   \log\left( \frac{1- C_\alpha'r^\alpha}{1+ C_\alpha'r^\alpha}  \right) \frac{1- C_\alpha'r^\alpha}{2} \Bigg] \\
% 	 = & w \rho_H(\sigma_i , \sigma_0) \log \left( \frac{1+ C_\alpha'r^\alpha}{1- C_\alpha'r^\alpha}  \right) C_\alpha'r^\alpha\\
% 	 \le & 2mw\frac{C_\alpha'^2 r^{2\alpha}}{1-C_\alpha'r^\alpha}\\
% 	 \le & 4mw C_\alpha'^2 r^{2\alpha}.
% 	\end{align*}  
% 	Hence, 
% 	\begin{align*}
% 	D(\Pi_i|\Pi_0) &\le  4mw C_\alpha'^2 r^{2\alpha} (n_P+n_Q)\\
% 	&= 4m c_w r^d C_\alpha'^2 r^{2\alpha} (n_P+n_Q)\\
% 	& = 4m c_w C_\alpha'^2 r^{2\alpha+d} (n_P+n_Q)\\
% 	& = 4m c_w C_\alpha'^2 c_r^{2\alpha+d} (n_P+n_Q)^{-\frac{2\alpha +d}{\alpha d_0}} (n_P+n_Q)\\
% 	& = 4m c_w C_\alpha'^2 c_r^{2\alpha+d} \text{ since } \alpha d_0 = 2\alpha + d\\
% 	& = 2^5 (\log 2)^{-1} c_w C_\alpha'^2 c_r^{2\alpha+d} \log (M)\\
% 	&\le \frac 18\log (M),  
% 	\end{align*} for $ c_w $ small enough. 

	
% 	By proposition \ref{prop:tsybakov}, \begin{align*}
% 	\sup_{(P,Q)\in \Pi} \Ex \cE_Q (\hat f)& \ge \sup_{(P,Q)\in \Pi} s \Pr_\Pi \left ( \cE_Q (\hat f)\ge s \right)\\
% 	& \ge s \sup_{\sigma\in \{-1,1\}^m} \Pi_\sigma \left(\cE_{Q^\sigma} (\hat f)\ge s \right) \\
% 	& \ge s \frac {3-2\sqrt{2}}{8}\\
% 	& \ge C'(n_p+n_Q)^{-\frac{1+\beta}{d_0}}
% 	\end{align*}
	
% \noindent \textbf{Part II:}	

% 	Now we  deal with the error of estimation for the parameter $ \pi_Q. $ We shall see that, it is enough to construct two distributions for this purpose.


% For some $ w = \frac 1{16} $ (to be chosen later) let us define the following class conditional densities: 

% \[ g_1(x) = \begin{cases}
% 4w (1-\delta) & \text{if } 0 \le  x_1 \le \frac 14,\\
% 4\delta & \text{if } \frac 38 \le x_1 \le \frac 58, \\
% 4(1-\delta)(1-w) & \text{if } \frac 34 \le x_1 \le 1\\
% 0 & \text{elsewhere}.
% \end{cases} \] and \[ g_0(x) = \begin{cases}
% 4(1-w) (1-\delta) & \text{if } 0 \le  x_1 \le \frac 14,\\
% 4\delta & \text{if } \frac 38 \le x_1 \le \frac 58, \\
% 4(1-\delta)w & \text{if } \frac 34 \le x_1 \le 1\\
% 0 & \text{elsewhere}.
% \end{cases} \] Let $ \sigma \in \{-1, 1\}. $ We shall choose $ \delta  $ later. We specify the class probabilities in the following way:
% \[ \pi_P = \frac12 , \ \pi_Q^\sigma = \frac 12 (1+\sigma m) \]  where, $  m = \frac 1 {16\sqrt{n_Q}}. $ Then \[ \eta_Q^\sigma (x) = \frac{\pi_Q^\sigma g_1(x)}{\pi_Q^\sigma g_1(x) + (1-\pi_Q^\sigma)g_0(x)} = \begin{cases}
% \frac{w(1+\sigma m)}{w(1+\sigma m) + (1-w) (1-\sigma m)} & \text{if }  0 \le  x_1 \le \frac 14,\\
% \frac{1+\sigma m}{2} & \text{if } \frac 38 \le x_1 \le \frac 58, \\
% \frac{(1-w)(1+\sigma m)}{(1-w)(1+\sigma m) + w (1-\sigma m)} & \text{if } \frac 34 \le x_1 \le 1.
% \end{cases} \]

% Given the class conditional densities and the class probabilities the population distributions can be constructed in the following way: for a Borel set $ A \subset [0,1]^d $ and for index $ y \in \{0,1\} $ \[ P(X\in A, Y = y) = y \pi_P \int_A g_1(x) + (1-y) (1-\pi_P) \int_A g_0(x) \] and 

% \[ Q^\sigma (X\in A, Y = y) = y \pi_Q^\sigma \int_A g_1(x) + (1-y) (1-\pi_Q^\sigma) \int_A g_0(x). \]

% It is easy to see that the densities $ g_0 $ and $ g_1 $ are locally $ \alpha $-H\"older smooth with constant $ C_\alpha. $ We need to check the margin  condition. 

% \textbf{Checking margin condition \ref{def:margin-condition}:} 


% Note that \begin{align*}
% \left|\frac{w(1+\sigma m)}{w(1+\sigma m) + (1-w) (1-\sigma m)} - \frac 12\right| & = \frac 12  \frac{|w(1+\sigma m) - (1-w) (1-\sigma m)|}{w(1+\sigma m) + (1-w) (1-\sigma m)}\\ 
% & = \frac 12 \frac {|2w +\sigma m -1|}{1-\sigma m + 2\omega\sigma m	}\\
% & = \frac 12 \frac {1-2w -\sigma m }{1-\sigma m + 2\omega\sigma m	} \ge \frac 12 \frac {1-3/16}{1+3/16} = \frac {13}{38}
% \end{align*}

% and \begin{align*}
% \left| \frac{(1-w)(1+\sigma m)}{(1-w)(1+\sigma m) + w (1-\sigma m)} - \frac 12 \right| & = \frac12 \frac{(1-w)(1+\sigma m)- w (1-\sigma m) }{(1-w)(1+\sigma m) + w (1-\sigma m)} \\
% & = \frac 12 \frac{1+\sigma m-2w}{1 +\sigma m- 2w\sigma m} \ge \frac 12 \frac {1-3/16}{1+3/16} = \frac {13}{38}
% \end{align*}


% Hence  for $ t < m $ we have \[ Q\left( \left| \eta_Q^\sigma(X) - \frac 12 \right| \le t  \right) = 0 \]. For $ m \le t < \frac{13}{38} $ we have 
% \begin{align*}
% Q\left( \left| \eta_Q^\sigma(X) - \frac 12 \right| \le t  \right) &= Q \left( \frac 38 \le X_1 \le \frac 58  \right) = \delta. 
% \end{align*}
% We choose $ \delta = C_\beta m^\beta . $ Then \[ Q\left( \left| \eta_Q^\sigma(X) - \frac 12 \right| \le t  \right) \le C_\beta m^\beta \le C_\beta t^\beta. \]
% and for $ t \ge \frac{13}{38} $ we have \[ Q\left( \left| \eta_Q^\sigma(X) - \frac 12 \right| \le t  \right) \le 1 \le C_\beta t^\beta. \]


% We define our distribution class $ \cH = \{ \Pi_\sigma : \sigma \in \{-1, 1\} \}, $ where $ \Pi_\sigma  $ is defined as \[  \Pi^\sigma = P^{\otimes n_P} \otimes \left(Q^\sigma \right)^{\otimes n_Q}. \] Then the Kullback-Leibler divergence between $ \Pi_{-1} $ and $ \Pi_1 $ is \begin{align*}
% D\left(  \Pi_1 | \Pi_{-1}  \right)  = & n_Q D\left(Q^{(-1)}| Q^{(1)}\right)\\
%  = & n_Q \Bigg[ \log\left( \frac{1+\frac{1}{16\sqrt{n_Q}}}{1-\frac{1}{16\sqrt{n_Q}} } \right) \left( 1+\frac{1}{16\sqrt{n_Q}}  \right)\\
%  & + \log\left( \frac{1-\frac{1}{16\sqrt{n_Q}}}{1+\frac{1}{16\sqrt{n_Q}} } \right) \left( 1-\frac{1}{16\sqrt{n_Q}}  \right)  \bigg] \\
%  = & \frac {2n_Q}{16\sqrt{n_Q}} \log\left( \frac{1+\frac{1}{16\sqrt{n_Q}}}{1-\frac{1}{16\sqrt{n_Q}} } \right)\\
%  \le & \frac{6n_Q}{256 n_Q } \ \text{using } \log\left( \frac{1+x}{1-x} \right) \le 3x \text{ for } 0 \le x\le \frac 12,\\
%  = & \frac 3{128}.
% \end{align*}

% Here $ M = |\cH| = 2 $ , $ \Pi_{1} \ll \Pi_{-1} $ and\\ $ \frac1M \sum_{\sigma\in \{-1,1\}} D(\Pi^\sigma | \Pi^{-1}) = \frac12 D(\Pi^1 | \Pi^{-1}) = \frac 3 {256} < \frac{\log 2}{8}.  $


% Also, let $ f_\sigma  $ is the Bayes decision rule for distribution $ Q^\sigma,  $ \ie, \ \[ f_\sigma (x) = \indicator\left\{ \eta_Q^\sigma (x)  \ge \frac 12  \right\}. \] Then  \begin{align*}
% \cE_{Q^{1}}\left(f_{-1}\right) & = \Ex_{Q^{1}} \left[ \left| \eta_Q^1(X) - \frac 12 \right|\indicator\left\{ f_1(X) \neq f_{-1}(X)  \right\}  \right]\\
% & = \delta m \\
% & = \frac{C_\beta}{16^{\beta+1}} n_Q^{-\frac{\beta+1}{2}} \triangleq 2s.
% \end{align*}

% Using proposition \ref{prop:tsybakov} \begin{align*}
% \sup_{(P,Q)\in \Pi} \Ex \cE_Q (\hat f)& \ge \sup_{(P,Q)\in \Pi} s \Pr_\Pi \left ( \cE_Q (\hat f)\ge s \right)\\
% & \ge s \sup_{\sigma\in \{-1,1\}} \Pi_\sigma \left(\cE_{Q^\sigma} (\hat f)\ge s \right) \\
% & \ge s \frac {3-2\sqrt{2}}{8}\\
% & \ge C'n_Q^{-\frac{1+\beta}{2}}
% \end{align*}


	
% Combining these two lower bounds, we get the result.
% \end{proof}





\begin{proof}[\bf{Proof of theorem \ref{th:upper-bound}}]
	\label{pr:upper-bound}
The proof is broken into several steps to prove the final result.

	\noindent \textbf{Step I: Concentration of $\hat \pi_Q $ and $ n_1 $}
	
	Consider the following notations: $ N = n_P+n_Q $, $ \zeta(x) = \left|\eta_Q(x)-\frac12 \right|,$ $ n_k^P = \# \{Y_i^{(P)}=k\},$ $ n_k^Q = \# \{Y_i^{(Q)}=k\}  $,  $n_k = \# \{y_i = k\} $ for $k=0,1.$
	Then by lemma \ref{lemma:bernoulli} \begin{equation}
	\Pr \left(|\hat\pi_Q - \pi_Q|  > t \right) \le \exp\left(  - \frac{n_Qt^2}{4 \pi_Q (1- \pi_Q)}  \right),
	\label{eq:y-target}
	\end{equation}
	
		and \begin{equation}
	\Pr \left( |n_1 - n_P\pi_P - n_Q\pi_Q | >t   \right)\le 2\exp \left(  - \frac{t^2}{n_P + n_Q}  \right).
	\label{eq:y-total}
	\end{equation}
	
	
	Letting $ t^2 = 4\eta^2 \pi_Q (1-\pi_Q), $ in inequality \ref{eq:y-target} we get \[ |\hat\pi_Q - \pi_Q| \le 2\eta\sqrt{\pi_Q (1-\pi_Q)} \] with probability at least $ 1-\exp \left( - \eta^2 n_Q  \right). $
Also, 	letting $ t = \delta N^{\frac{2\alpha + d/2}{2\alpha + d}},  $ in \ref{eq:y-total} we get \[ \Pr \left( |n_1 - n_P\pi_P - n_Q\pi_Q | >\delta N^{\frac{2\alpha + d/2}{2\alpha + d}}   \right)\le 2\exp \left(  - \delta^2 N^{\frac{2\alpha}{2\alpha + d}}  \right). \]
	
	Hence, with probability $ \ge 1- 2\exp \left(  - \delta^2 N^{\frac{2\alpha}{2\alpha + d}}  \right) $ we have \[ |n_1 - n_P\pi_P - n_Q\pi_Q | \le \delta N^{\frac{2\alpha + d/2}{2\alpha + d}}. \]
	
	 Since, $\epsilon \le \pi_P, \pi_Q \le 1- \epsilon$  we see that $\eps (n_P+n_Q) \le n_P \pi_P+ n_Q\pi_Q \le (1-\eps)(n_P+n_Q)$ and  $n_P\pi_P + n_Q\pi_Q \gg (n_P+n_Q)^{\frac{2\alpha+d/2}{2\alpha+d}}.$ Hence, for $ k \in \{0,1\}, $ $ c_kN \le n_k  \le C_k N, $ for some $0<c_k \le C_K \le 1$ for all sufficiently large $n_P$ and $n_Q.$
	
	
	
	
	
	
	
	
	
	
	
%	Consider the following notations: $ \phi = \frac{p_0}{p_1}, \  m = n_0 \wedge n_1,  $ $ \varepsilon_\phi (x,r) = \sup_{x' \in B(x,r)} |\phi(x)-\phi(x')|,  $ $ c_n = v\log (2n) + \log (8/\delta) $ and $ e_{n,r}(x) = \sqrt{\frac{24c_{n}}{nP_1 (B(x,r))}}. $
%	
%	Using Lemma 1 and 2 in \citet{kpotufe2017lipschitz} we get that with probability at least $ 1-2\delta $, the following holds for all $ x \in \Omega $ satisfying $ \cE_r(x): $
%	\[ \left| \hat \phi (x) - \phi(x) \right| \le e_{n_1,r}(x) \phi(x) + 2 \left(  e_{n_0,r}(x) \sqrt{\phi (x) + \varepsilon_\phi(x,r)} + e^2_{n_0,r}(x) + \varepsilon_\phi(x,r)  \right) \]
%	
%	Here, $ \varepsilon_\phi(x,r) \le C_\alpha r^\alpha $  and $ e_{n,r} (x) \le \sqrt{\frac{24 (v\log (2n)+ \log(8/\delta))}{n\mu a(d) r^d}} ,$ where $ a(d) = \lambda(B(0,1)). $ Hence, the above inequality can be simplified as: \[ \left| \hat \phi (x) - \phi(x) \right| \le   C_1\sqrt{\frac{24 (v\log (2m)+ \log(8/\delta))}{m\mu a(d) r^d}} + C_2 r^\alpha  \]
%	Letting $ \delta = 8\times (2m)^{d+1} \exp\left(-\eta^2 \mu a(d) m^{\frac{2\alpha}{2\alpha+d}} \right)  $ we get \[ \left| \hat \phi (x) - \phi(x) \right| \le   C_1\eta + C_2 r^\alpha. \]
%	Now, \begin{align*}
%	\left|  \frac{1- \hat \pi_Q}{\hat\pi_Q} \hat \phi (x) - \frac{1- \pi_Q}{\pi_Q} \phi(x) \right| \le & \left|  \frac{1- \hat \pi_Q}{\hat\pi_Q}  - \frac{1- \pi_Q}{\pi_Q}  \right|\hat \phi (x) + \frac{1- \pi_Q}{\pi_Q}  \left| \hat \phi (x) - \phi(x) \right| \\
%	\le & \left|  \frac{1- \hat \pi_Q}{\hat\pi_Q}  - \frac{1- \pi_Q}{\pi_Q}  \right| \left(\phi (x) + C_1 \eta + C_2 r^\alpha\right)+ \frac{1- \pi_Q}{\pi_Q}   \left( C_1 \eta +C_2 r^{\alpha}\right) \\
%	\le & \frac{|\hat \pi_Q - \pi_Q|}{\hat \pi_Q \pi_Q} \left(\phi (x) + C_1 \eta + C_2 r^\alpha\right)+ \frac{1- \pi_Q}{\pi_Q}   \left( C_1 \eta +C_2 r^{\alpha}\right)
%	\end{align*}
%	
%	
%	
%	Using $ \left| \frac{1}{1+x'} - \frac1{1+x} \right| = \frac{|x'-x|}{(1+x)(1+x')} ,$ for sufficiently large $ n_P $ and $ n_Q, $ we get \begin{align*}
%	\left| \frac1{1+\frac{1- \hat \pi_Q}{\hat\pi_Q} \hat \phi (x)}  - \frac1{1+\frac{1- \pi_Q}{\pi_Q} \phi(x)} \right| & \le \frac{\frac{|\hat \pi_Q - \pi_Q|}{\hat \pi_Q \pi_Q} \left(\phi (x) + C_1 \eta + C_2 r^\alpha\right)+ \frac{1- \pi_Q}{\pi_Q}   \left( C_1 \eta +C_2 r^{\alpha}\right)}{\left(1+\frac{1- \hat \pi_Q}{\hat\pi_Q} \hat \phi (x)\right)\left(1+\frac{1- \pi_Q}{\pi_Q} \phi(x)\right)} \\
%	& \le \frac{\left(\phi (x) + C_1 \eta + C_2 r^\alpha\right)|\hat \pi_Q - \pi_Q|}{\left(\hat \pi_Q+ (1-\hat\pi_Q)\hat\phi(x)\right)\left( \pi_Q+ (1-\pi_Q)\phi(x)\right)} + \frac{C_1\eta + C_2 r^\alpha}{\lambda_-} \\
%	& \le \frac{\left(\lambda_+ + C_1 \eta + C_2 r^\alpha\right)\eta}{\left(\lambda_- -C_1 \eta - C_2 r^\alpha \right)\lambda_-} + \frac{C_1\eta + C_2 r^\alpha}{\lambda_-} \\
%	& \le C_5 \eta + C_6 r^\alpha\le \xi
%	\end{align*} with probability at least $ 1 - \exp\left(-C_6\xi^2N^{\frac{2\alpha}{2\alpha + d}} \right) - \exp\left(-C_7\xi^2 n_Q\right)\ge 1 - \exp\left(-\xi^2\left(C_6N^{\frac{2\alpha}{2\alpha + d}} \wedge C_7 n_Q\right)\right), $ where $ \xi $ is chosen such that $ \xi \ge  2C_5\eta, $ and $ \xi \ge 2C_6r^\alpha. $
%	
%	
%	Hence, \[ \sup_{\Pr \in \cP}\Pr\left( \left| \hat \eta_Q(X) - \eta_Q(X) \right| > \xi   \right) \le  \exp\left(-\xi^2C_8\left(N^{\frac{2\alpha}{2\alpha + d}} \wedge n_Q\right)\right), \] where, $ C_8 = 2(C_6 \vee C_7). $
%	
%	To get a bound for the generalization error we define the following events: $$ A_0 = \left\{ x\in \reals^d: 0< \left| \eta_Q(x) - \frac12\right| < \xi        \right\}  \text{ and for }j \ge 1, \ A_j = \left\{ x\in \reals^d: 2^{j-1}< \left| \eta_Q(x) - \frac12\right| < 2^j\xi        \right\}  $$ Now, \begin{align*}
%	\cE_Q(\hat f)  = & 2 \Ex_X \left(\left| \eta_Q(X) -\frac12 \right|\indicator_{\{\hat f(X)\neq f^*(X)\}}  \right) \\
%	= & 2\sum_{j=0}^\infty \Ex_X\left(\left| \eta_Q(X) -\frac12 \right|\indicator_{\{\hat f(X)\neq f^*(X)\}} \indicator_{\{X\in A_j\}} \right) \\
%	\le & 2 \xi \Ex_X\left( 0< \left| \eta_Q(X) -\frac12 \right|< \xi  \right) \\
%	& + 2\sum_{j=1}^\infty \Pr_X\left(\left| \eta_Q(X) -\frac12 \right|\indicator_{\{\hat f(X)\neq f^*(X)\}} \indicator_{\{X\in A_j\}} \right)
%	\end{align*}
%	On the event $ \{ \hat f\neq f^*  \} $ we have $ \left| \eta_Q - \frac12 \right| \le \left| \hat \eta - \eta \right|. $ So, for any $ j \ge 1 $ we get \begin{align*}
%	\Ex_X&\Ex \left(\left| \eta_Q(X) -\frac12 \right|\indicator_{\{\hat f(X)\neq f^*(X)\}} \indicator_{\{X\in A_j\}} \right) \\
%	& \le 2^{j+1}\xi \Ex_X\Ex \left(\indicator_{\{|\hat \eta_Q(X)- \eta_Q(X)| \ge2^{j-1}\xi \}} \indicator_{\{0< |\eta_Q(X)-1/2|<2^{j}\xi\}} \right) \\
%	& = 2^{j+1}\xi \Ex_X \left[\Pr\left(\indicator_{\{|\hat \eta_Q(X)- \eta_Q(X)| \ge2^{j-1}\xi \}}\right) \indicator_{\{0< |\eta_Q(X)-1/2|<2^{j}\xi\}} \right] n\\
%	& \le 2^{j+1}\xi \exp\left(-a(2^{j-1}\xi)^2\right)\Pr_X (0< |\eta_Q(X)-1/2|<2^{j}\xi)\\
%	& \le 2C_\beta 2^{j(1+\beta)}\xi ^{1+\beta} \exp\left(-a(2^{j-1}\xi)^2\right).
%	\end{align*} where $ a = C_8\left(N^{\frac{2\alpha}{2\alpha + d}} \wedge  n_Q\right). $
%	Letting $ \xi = a^{-\frac12}  $ we get \begin{align*}
%	\sup_{\Pr \in \cP}\cE(\hat f) & \le 2C_\beta \left( \xi^{1+\beta} + \sum_{j\ge 1}  2^{j(1+\beta)} \xi^{1+\beta}\exp\left(-a(2^{j-1}\xi)^2\right)   \right) \\
%	& \le C \left(N^{\frac{2\alpha}{2\alpha + d}} \wedge n_Q\right)^{-\frac{1+\beta}{2}}.
%	\end{align*}






\noindent \textbf{Step II: Concentration of $\hat \eta_Q(x) $}

We consider the following result:


Let $ K :\reals^d \to [0,\infty) $ be a kernel with $ \int_{\reals^d} K(x) dx = 1. $ For some  $ h >0 $ let $ \cF_h = \left\{  K\left( \frac{\cdot - x}{h} \right): x \in \reals^d  \right\}. $ Then $ d_{\cF_h} \le d+1. $ According to Corollary \ref{cor:empirical-convergence}, with probability at least $ 1-\delta  $  for any $ f \in \cF_h $


\begin{align*}
	|\nu_n(f) - \nu(f)| & \le \begin{cases}
	\sqrt{6\nu(f)\alpha_n} + \alpha_n & \text{if } 3\nu(f) \ge 2 \alpha_n,\\
	3\alpha_n & \text{if } 3\nu(f) < 2\alpha_n
	\end{cases} \\
	& \le  \sqrt{6\nu(f)\alpha_n} + 3\alpha_n. 
\end{align*}


Note that the regression function  $ \eta_Q(x) $ has the following form \[ \eta_Q(x) = \frac{\pi_Q g_1(x)}{\pi_Qg_1(x)+(1-\pi_Q)g_1(x)}. \] Let us remind some notations: $ \cZ $ is the set of all $ n_P+n_Q $ sample points of feature-outcome pairs $ (X,Y) $. For $  i = 0,1, \  \cX_i = \{x: (x,y)\in\cZ, y = i \},  $ $ \widehat G_i  $ is empirical measure on $ \cX_i. $ For a fixed $ x \in [0,1]^d $ define $ u = \pi_Qg_1(x) $ and $ v = (1-\pi_Q)g_0(x), $ $ \hat u = \hat \pi_Q \widehat G_1 \left( \frac{1}{h^d} K\left( \frac{\cdot - x}{h} \right)  \right) $ and $ \hat v = (1-\hat \pi_Q) \widehat G_0 \left( \frac{1}{h^d} K\left( \frac{\cdot - x}{h} \right)  \right). $ Then \begin{align*}
	\left|\hat \eta_Q(x) -  \eta_Q(x) \right| & \le \left|  \frac{\hat u }{\hat u + \hat v}- \frac{u}{u+v}  \right|\\
	& \le \frac{|\hat u v - u \hat v|}{(u+v)(\hat u + \hat v)}\\
	& \le \frac{|\hat u (v- \hat v) +  \hat v(\hat u - u)|}{(u+v)(\hat u + \hat v)}\\
	& \le \frac{|\hat u - u|+ |\hat v - v|}{u+v}
\end{align*}

We shall get a high probability bound for $ |\hat u - u|+ |\hat v - v|. $

Note that  \[ |\hat u - u| \le \hat \pi_Q \left|  \deone  - g_1(x)  \right| + g_1(x)|\hat \pi_Q - \pi_Q|.  \] Now, to bound $ \left|  \deone  - g_1(x)  \right| $ we notice that 

\begin{align*}
\Bigg| &  \deone  - g_1(x)  \Bigg|\\ \le &   \left| \deone - \popone \right|\\ & + \left| \popone - g_1(x) \right|
\end{align*}
 A high probability upper bound for $ \left| \deone - \popone \right| $ is obtained using Corollary \ref{cor:empirical-convergence}. We shall use smoothness of $ g_1 $ to bound $ \left| \popone - g_1(x) \right|. $ From the definition of locally $ \alpha $-H\"older smoothness of $ g_0 $ and $ g_1 $ (definition \ref{def:holder-smooth}) there is some $ \delta_0 >0 $ such that for any $ \delta \in (0, \delta_0] $ and for any $x, x' \in \Omega$ with $ \|x-x'\|_2 \le \delta  $ we have  \[  \max\{ |g_0(x)-g_0(x')|, |g_1(x) - g_1(x')| \} \le (C_\alpha+1) \|x-x'\|_2^\alpha.   \]

Let $ a>\alpha $ be such that $ C_a \triangleq \int_{\reals^d} \|x\|_2^a K(x) dx <\infty   $ (such an $ a $ exists because $ K \in \cK(\alpha) $). Using Markov's inequality, for any $ R>0 $ \[ \int_{\|x\| > R} K(x)dx \le \frac1{R^a} \int_{\reals^d} \|x\|^a K(x) dx = h^\alpha  \] if $ R = C_a^{\frac1 a} h^{- \frac  \alpha a }. $ Let $ h_0 \triangleq \left(\frac{\delta_0}{C_a^{\frac1 a}}  \right)^{\frac a{a-\alpha}} . $ Then for any $ h \in (0, h_0) $ if we let $ R(h) = C_a^{\frac1 a} h^{- \frac \alpha a } $ we have the followings:
\begin{enumerate}
	\item  $ \int_{\|x\| > R(h)} K(x)dx \le h^\alpha, $ and 
	\item $ h R(h) = C_a^{\frac1 a} h^{1-\frac \alpha a } \le C_a^{\frac1 a} h_0^{\frac {a-\alpha} a } = \delta_0. $
\end{enumerate}
Note that 
\begin{align*}
	\popone - g_1(x)  = &  \int \frac{1}{h^d} K\left( \frac{y - x}{h} \right)(g_1 (y)- g_1(x))dy\\
	 = & \int_{\reals^d} K(z) (g_1(x+ zh)- g_1(x)) dz \\
	  = & \underbrace{\int_{\|z\|\le R(h)} K(z) (g_1(x+ zh)- g_1(x)) dz}_{(I)} \\
	  & + \underbrace{\int_{\|z\|> R(h)} K(z) (g_1(x+ zh)- g_1(x)) dz}_{(II)}.
\end{align*}

Now, for $ \|z\|\le R(h) $ we have $\|zh\| \le  h R(h) \le \delta_0.$ For such $ z $ we have $ |g_1(x+zh) - g_1(x)| \le \|zh\|^\alpha = h^\alpha \|z\|^\alpha. $ Hence,  \begin{align*}
	|(I)|  \le &  \int_{\|z\|\le R(h)} K(z) |g_1(x+ zh)- g_1(x)| dz\\
	\le & \int_{\|z\|\le R(h)} K(z) h^\alpha \|z\|^\alpha dz \\
	 \le & h^\alpha \int_{\reals^d} \|z\|^\alpha K(z) dz \\
	 \le &  h^\alpha \int_{\reals^d} \left( 1+ \|z\|^a \right) K(z) dz\\
	 = & (1+C_a) h^\alpha.
\end{align*}

Since the densities are bounded by $ \mu_+, $ we have \begin{align*}
	|(II)| \le & \int_{\|z\|> R(h)} K(z) |g_1(x+ zh)- g_1(x)| dz\\
	\le &  \mu_+ \int_{\|z\|> R(h)} K(z)dz \le \mu_+ h^\alpha.
\end{align*}
Combining $ (I) $ and $ (II) $ we get,  \[ \text{for } h \le h_0, \  \left|\popone - g_1(x) \right| \le (1+C_a + \mu_+) h^\alpha = c_1(\alpha)h^\alpha. \] Similarly we can get the bound \[\text{for } h \le h_0, \ \left|\popzero - g_0(x) \right| \le  c_1(\alpha)h^\alpha.  \]



By Corollary \ref{cor:empirical-convergence}, with probability at least $ 1- 2\delta $ for any $ x $ and $ k \in  \{0,1\}, $ 
\begin{align}
\label{eq:concentration-kde}
\left| \widehat G_k \left( \frac{1}{h^d} K\left( \frac{\cdot - x}{h} \right)  \right) -  G_k \left( \frac{1}{h^d} K\left( \frac{\cdot - x}{h} \right)  \right) \right| & \le \sqrt{6\frac{\alpha_m}{h^d} G_k \left( \frac{1}{h^d} K\left( \frac{\cdot - x}{h} \right)  \right) } + \frac{\alpha_m}{h^d} \nonumber\\
&\le \sqrt{6\frac{\alpha_m}{h^d} (g_k(x)+ c_1(\alpha)h^\alpha) } + \frac{\alpha_m}{h^d}
\end{align}

\begin{align}
	|\hat u - u| + |\hat v - v|  \le &\underbrace{\hat \pi_Q \left|  \deone  - g_1(x)  \right|}_{(I)}\\ &  + \underbrace{(1-\hat \pi_Q) \left|  \dezero  - g_0(x)  \right|}_{(II)} \nonumber \\
	& + \underbrace{g_1(x)|\hat \pi_Q - \pi_Q| + g_0(x)|\hat \pi_Q - \pi_Q|}_{(III)}
\end{align}

By repeated usage of $ (\sqrt{x}+\sqrt{y})^2 \le 2(x+y) $ we get:

\begin{align}
	(I) + (II) \le & \hat \pi_Q\left( \sqrt{6\frac{\alpha_m}{h^d} (g_1(x)+ c_1(\alpha)h^\alpha) } + \frac{\alpha_m}{h^d} + c_1(\alpha)h^\alpha \right)\nonumber \\
	& + (1- \hat \pi_Q) \left( \sqrt{6\frac{\alpha_m}{h^d} (g_0(x)+ c_1(\alpha)h^\alpha) } + \frac{\alpha_m}{h^d} + c_1(\alpha)h^\alpha \right) \nonumber\\
	\le &  2\sqrt{6\frac{\alpha_m}{h^d} (\hat \pi_Q^2 g_1(x)+ (1-\hat \pi_Q)^2g_0(x))} + \sqrt{6\frac{\alpha_m}{h^d} c_1(\alpha)h^\alpha} + \frac{\alpha_m}{h^d} + c_1(\alpha)h^\alpha  \nonumber\\
%	\le & 2\sqrt{6\frac{\alpha_m}{h^d} \left(\left(\pi_Q + \sqrt{\pi_Q(1-\pi_Q)/n_Q}\right)^2 g_1(x)+ \left(1-\pi_Q + \sqrt{\pi_Q(1-\pi_Q)/n_Q}\right)^2g_0(x)\right)} + 4 \frac{\alpha_m}{h^d} + 2c_1(\alpha)h^\alpha (*)\nonumber\\
%	\le & C_1 \sqrt{\frac{\alpha_m}{h^d} (\pi_Q g_1(x)+(1-\pi_Q)g_0(x))} + 4 \frac{\alpha_m}{h^d} + 2c_1(\alpha)h^\alpha (*)\nonumber\\
	\le & C_2 \sqrt{\frac{\alpha_m}{h^d} } + 4 \frac{\alpha_m}{h^d} + 2c_1(\alpha)h^\alpha
\end{align}

Letting $ h = C m^{-\frac1{2\alpha + d}} $ for some $C>0$ (note that $ h\le h_0 $ for sufficiently large $ m $) and $ \delta = 8(2m)^{d+1} \exp \left( -c_3(\alpha) \eta^2 m^{\frac{2\alpha}{2\alpha+d}}\right) $ for some $ \eta<1, $
  in Corollary \ref{cor:empirical-convergence} we get \[ (I) + (II) \le C_2 \eta \sqrt{c_3(\alpha)} + 4c_3(\alpha)\eta^2 + 2c_1(\alpha)h^\alpha\le \mu_-\eta/2 + 2c_1(\alpha) m^{-\frac\alpha{2\alpha + d}} .\] Here, $ c_3(\alpha) $ is appropriately chosen such that the above inequality holds. 

Turning our attention to $ (III) $ we see that, with probability at least $ 1- \exp(-t^2 n_Q) $ 
\[  (II)  \le 2 \sqrt{\pi_Q (1-\pi_Q)} (g_1(x) + g_0(x)) t \le C_3 t. \]  Since, $ q_X(x) \ge \mu_-  $ for any $ x \in \Omega, $ with probability at least $ 1- \exp(-t^2 n_Q) - 8(2m)^{d+1} \exp \left( -c_3(\alpha) \eta^2 m^{\frac{2\alpha}{2\alpha+d}}\right) $ we get \[ |\hat \eta_Q(x) - \eta_Q(x)| \le \frac\eta 2 +\frac{2c_1(\alpha)}{\mu_-} m^{-\frac\alpha{2\alpha + d}}+ \frac{C_3 t}{\mu_-}  \text{ for any }x \in \Omega. \] 
For appropriate $ c_4 $ with probability \begin{align*}
    &  1- \exp(-c_4\eta^2 n_Q) - 8(2m)^{d+1} \exp \left( -c_3(\alpha) \eta^2 m^{\frac{2\alpha}{2\alpha+d}}\right)\\ \ge &   1- \exp\left(-c_5 \eta^2 \left( n_Q \wedge m^{\frac{2\alpha}{2\alpha+d}}\right)   \right)
\end{align*}  we get \[|\hat \eta_Q(x) - \eta_Q(x)| \le\eta + \frac{2c_1(\alpha)}{\mu_-} m^{-\frac\alpha{2\alpha + d}} \text{ for any }x \in \Omega  \] This implies \begin{align*}
& 	\Pr \left( |\hat \eta_Q(x) - \eta_Q(x)| > \eta  \text{ for any }x \in \Omega   \right)\\  \le & \ \exp\Bigg[-c_5 \left(\eta -\frac{2c_1(\alpha)}{\mu_-} m^{-\frac\alpha{2\alpha + d}} \right)^2   \left( n_Q \wedge m^{\frac{2\alpha}{2\alpha+d}}\right)\Bigg]\\
	 \le & \ \exp\Bigg[-c_5 \left(\frac{\eta^2} 2  -\frac{4c_1^2(\alpha)}{\mu_-^2} m^{-\frac{2\alpha}{2\alpha + d}} \right)\left( n_Q \wedge m^{\frac{2\alpha}{2\alpha+d}}\right)\Bigg] \\
	& \hspace{0.3in} \big( \text{using } (a-b)^2 \ge a^2 /2 - b^2\big) \\
	 \le & \ \exp \left(- c_6\left( n_Q \wedge m^{\frac{2\alpha}{2\alpha+d}}\right) \right)\\
	\le & \ \exp \left(- c_6\left( n_Q \wedge N^{\frac{2\alpha}{2\alpha+d}}\right) \right)
\end{align*}

\noindent \textbf{Step III: Upper bound of $\Ex \cE_Q(\hat f) $}

	To get a bound for $ \Ex \cE_Q(\hat f) $ we define the following events: $$ A_0 = \left\{ x\in \reals^d: 0< \left| \eta_Q(x) - \frac12\right| < \xi        \right\}$$  and for $j \ge 1,$ $$\ A_j = \left\{ x\in \reals^d: 2^{j-1}< \left| \eta_Q(x) - \frac12\right| < 2^j\xi        \right\} . $$ Now, \begin{align*}
	\cE_Q(\hat f)  = & 2 \Ex_X \left(\left| \eta_Q(X) -\frac12 \right|\indicator_{\{\hat f(X)\neq f^*(X)\}}  \right) \\
	= & 2\sum_{j=0}^\infty \Ex_X\left(\left| \eta_Q(X) -\frac12 \right|\indicator_{\{\hat f(X)\neq f^*(X)\}} \indicator_{\{X\in A_j\}} \right) \\
	\le & 2 \xi \Ex_X\left( 0< \left| \eta_Q(X) -\frac12 \right|< \xi  \right) \\
	& + 2\sum_{j=1}^\infty \Pr_X\left(\left| \eta_Q(X) -\frac12 \right|\indicator_{\{\hat f(X)\neq f^*(X)\}} \indicator_{\{X\in A_j\}} \right)
	\end{align*}
	On the event $ \{ \hat f\neq f^*  \} $ we have $ \left| \eta_Q - \frac12 \right| \le \left| \hat \eta - \eta \right|. $ So, for any $ j \ge 1 $ we get \begin{align*}
	\Ex_X&\Ex \left(\left| \eta_Q(X) -\frac12 \right|\indicator_{\{\hat f(X)\neq f^*(X)\}} \indicator_{\{X\in A_j\}} \right) \\
	& \le 2^{j+1}\xi \Ex_X\Ex \left(\indicator_{\{|\hat \eta_Q(X)- \eta_Q(X)| \ge2^{j-1}\xi \}} \indicator_{\{0< |\eta_Q(X)-1/2|<2^{j}\xi\}} \right) \\
	& = 2^{j+1}\xi \Ex_X \left[\Pr\left(\indicator_{\{|\hat \eta_Q(X)- \eta_Q(X)| \ge2^{j-1}\xi \}}\right) \indicator_{\{0< |\eta_Q(X)-1/2|<2^{j}\xi\}} \right] n\\
	& \le 2^{j+1}\xi \exp\left(-a(2^{j-1}\xi)^2\right)\Pr_X (0< |\eta_Q(X)-1/2|<2^{j}\xi)\\
	& \le 2C_\beta 2^{j(1+\beta)}\xi ^{1+\beta} \exp\left(-a(2^{j-1}\xi)^2\right).
	\end{align*} where $ a = c_5\left(N^{\frac{2\alpha}{2\alpha + d}} \wedge  n_Q\right). $
	Letting $ \xi = a^{-\frac12}  $ we get \begin{align*}
	\sup_{\Pr \in \cP}\Ex\cE(\hat f) & \le 2C_\beta \left( \xi^{1+\beta} + \sum_{j\ge 1}  2^{j(1+\beta)} \xi^{1+\beta}\exp\left(-a(2^{j-1}\xi)^2\right)   \right) \\
	& \le C \left(N^{\frac{2\alpha}{2\alpha + d}} \wedge n_Q\right)^{-\frac{1+\beta}{2}}.
	\end{align*}


\end{proof}



\subsection{Proof of results in section \ref{sec:unlabeled-target-data}}


% \begin{proof}[\bf{Proof of Theorem \ref{th:lower-bound-unlabeled}}]
% 	The proof is very similar to the proof of Theorem \ref{th:lower-bound}. We break the proof in two parts. The first part deals with $ n_P^{-\frac{\alpha(1+\beta)}{2\alpha + d}} $ rate, whereas the second part deals with $ n_Q^{- \frac{1+\beta}{2}} $ rate.
	
% 	\noindent \textbf{Part I:}
	
% 	Let $  d_0 = 2 + \frac d \alpha,  $ $ r = c_r n_P^{-\frac1{\alpha d_0}} ,\ m = \lfloor c_m r^{\alpha\beta -d} \rfloor,\ w = c_w r^d ,$ where, $ c_r = \frac19, \ c_m = 8\times 9^{\alpha\beta - d},\ 0<c_w \le 1 $ to be chosen later. 
	
% 	For such a choice we have $ 8\le m < \lfloor r^{-1} \rfloor ^d. $ As, $ \alpha\beta \le d, $ we have $ r \le \frac19. $ This implies $ c_m r^{\alpha\beta -d} \ge 8. $  Since $ r^{-1} \ge 8 $ which gives us $ r^{-1} \le \frac{9\lfloor r^{-1}\rfloor}{8}. $ Therefore, $ c_mr^{\alpha\beta -d} = 8 (9r)^{\alpha\beta}\left( \frac{r^{-1}}{9}\right) < 8^{1-d } \lfloor r^{-1} \rfloor ^d  \le \lfloor r^{-1} \rfloor ^d.$ 
	
% 	$ mw = mc_w r^d <1. $
	
% 	\textbf{Construction of $ g_0 $ and $ g_1: $}
% 	Divide $ \cX = [0,1]^d $ into $ \lfloor r^{-1} \rfloor ^d $ hypercubes of length $ r. $ Let $ \cZ $ be the set of their centers. Let $ \cZ_1 \subset \cZ $ such that $ \left|\cZ_1 \right| = m. $ Let $ \cZ_0 = \cZ \backslash \cZ_1,\ \cX_1 = \cup_{z\in\cZ_1} B\left( z,\frac r6  \right), \text{and } \cX_0 = \cup_{z\in\cZ_0} B\left( z,\frac r2  \right). $ Let $ q_1 = \frac w{\text{Vol}\left( B\left(z,\frac r6\right)  \right)}, \text{ and } q_0 = \frac{1-mw}{\text{Vol}\left(\cX_0\right)}.$  For $ \sigma \in \{-1,1\}^m, $ define \[ g_1^\sigma (x) = \begin{cases}
% 	a^\sigma q_1 \left(1+\sigma(z)C_\alpha'r^\alpha \right) & x \in B\left(z,\frac r6  \right), \ z \in \cZ_1,\\
% 	a^\sigma q_0 & x \in B\left(z,\frac r2  \right), \ z \in \cZ_0,\\
% 	0 & \text{otherwise},
% 	\end{cases} \] and, \[ g_0^\sigma (x) = \begin{cases}
% 	b^\sigma q_1 \left(1-\sigma(z)C_\alpha'r^\alpha \right) & x \in B\left(z,\frac r6  \right), \ z \in \cZ_1,\\
% 	b^\sigma q_0 & x \in B\left(z,\frac r2  \right), \ z \in \cZ_0,\\
% 	0 & \text{otherwise},
% 	\end{cases} \] where, $ C_\alpha'r^\alpha = C_\alpha' r^\alpha u^\alpha \left( \frac{\|x-z\|_2}{r}  \right) ,$ \[ u(x) = \begin{cases}
% 	1 & \text{if } x \le \frac16,\\
% 	1 - 6\left(x -\frac16  \right) & \text{if } \frac16 < x \le \frac13,\\
% 	0 & \text{if } x> \frac13,
	
% 	\end{cases} \] and $ C_\alpha' = \min \left\{ C_\alpha 6^{-\alpha}, \frac12, 1-2\epsilon  \right\}. $
	
% 	We want $ \int g_1^\sigma (x) dx = a^\sigma \left[ mw + (1-mw) + w\sum_{z\in\cZ_1} \sigma(z) C_\alpha'r^\alpha \right] = 1. $ Hence, $ a^\sigma = \frac1 {1+ w\sum_{z\in\cZ_1} \sigma(z)C_\alpha'r^\alpha}. $ Also, $ b^\sigma = \frac1 {1- w\sum_{z\in\cZ_1} \sigma(z)C_\alpha'r^\alpha}. $ Also, we want $ \frac{a^\sigma q_0 \pi_Q ^\sigma   }{b^\sigma q_0 \left(1-\pi_Q ^\sigma  \right)} = 1, $ which implies $ \pi_Q ^\sigma = \frac{1/a^\sigma}{1/a^\sigma + 1/b^\sigma} = \frac 12 \left( 1+ w  \sum_{z\in\cZ_1} \sigma(z) \right)  . $ We have freedom to choose $ \pi_P^\sigma>0. $ Set $ \pi_P^\sigma = \frac 12 \left( 1+ w  \sum_{z\in\cZ_1} \sigma(z) \right)  . $
	
% 	Then \[ \frac{1-\pi_Q^\sigma}{\pi_Q^\sigma} \frac{g_0^\sigma(x)}{g_1^\sigma(x)} = \begin{cases}
% 	\frac{1- \sigma(z)C_\alpha'r^\alpha}{1+ \sigma(z)C_\alpha'r^\alpha} & \text{if } x\in \cX_1,\\
% 	1 & \text{if } x\in \cX_0.
% 	\end{cases} \] 
% 	Then $ \eta_Q^\sigma(x) = \begin{cases}
% 	\frac{1+ \sigma(z)C_\alpha'r^\alpha}{2} & \text{if } x\in \cX_1,\\
% 	\frac12 & \text{if } x\in \cX_0.
% 	\end{cases} $ 
	
% 	So, $ \eta_Q^\sigma $ simplifies to \[ \eta_Q^\sigma(x) = \begin{cases}
% 	\frac{1+ \sigma(z)C_\alpha'r^\alpha}{2} & \text{if } x\in B\left( z,\frac r6 \right),\ z\in\cZ_1\\
% 	\frac12 & \text{if } x\in\cX_0.
% 	\end{cases}. \] 
% 	Extend it to \[ \eta_Q^\sigma(x) = \begin{cases}
% 	\frac{1+ \sigma(z)C_\alpha'r^\alpha}{2} & \text{if } x\in B\left( z,\frac r6 \right),\ z\in\cZ_1\\
% 	\frac12 & \text{otherwise.}
% 	\end{cases}. \] 
% 	The marginal density of $ X $ under the distribution $ Q $ is \[q_X = \pi_Q^\sigma g_1^\sigma + (1-\pi_Q^\sigma) g_0^\sigma= \begin{cases}
% 	q_1 & \text{for } x\in \cX_1,\\
% 	q_0 & \text{for } x \in \cX_0.
% 	\end{cases}\] 
	
	
% 	For $ x\in B\left(z,\frac r6 \right), \ z\in \cZ_1, $ \begin{align*}
% 	q_X(x) & = \pi_Q^\sigma g_1^\sigma(x) + (1-\pi_Q^\sigma) g_0^\sigma(x)\\
% 	& = a^\sigma q_1 \left(1+\sigma(z)C_\alpha'r^\alpha \right) \frac1{2a^\sigma}  + b^\sigma q_1 \left(1-\sigma(z)C_\alpha'r^\alpha \right) \frac1{2b^\sigma}\\
% 	& = q_1.
% 	\end{align*}
	
% 	For $ x\in B\left(z,\frac r2 \right), \ z\in \cZ_0, $ \begin{align*}
% 	q_X(x) & = \pi_Q^\sigma g_1^\sigma(x) + (1-\pi_Q^\sigma) g_0^\sigma(x)\\
% 	& = a^\sigma q_0  \frac1{2a^\sigma}  + b^\sigma q_0  \frac1{2b^\sigma}\\
% 	& = q_0.
% 	\end{align*}
	
% 	Hence the marginal density \[q_X(x) = \begin{cases}
% 	q_1 & \text{for } x\in \cX_1,\\
% 	q_0 & \text{for } x \in \cX_0.
% 	\end{cases}\] is independent of $ \sigma. $
	
	
% 	\textbf{Checking for $ \epsilon \le \pi_P^\sigma \le 1- \epsilon  $:} In the expression $ \pi_P^\sigma = \frac 12 \left( 1+ w  \sum_{z\in\cZ_1} \sigma(z) C_\alpha' r^\alpha \right)  $ first we try to get a bound for $ w  \sum_{z\in\cZ_1} \sigma(z) C_\alpha' r^\alpha.  $ Note that \begin{align*}
% 		\left| w  \sum_{z\in\cZ_1} \sigma(z) C_\alpha' r^\alpha  \right|  & \le  w  \sum_{z\in\cZ_1}  C_\alpha' r^\alpha\\& \le mw C_\alpha' r^\alpha \\
% 		 & \le C_\alpha'r^{\alpha} \le 1-2\epsilon.
% 	\end{align*} Hence, $ \pi_P^\sigma \ge \frac12 (1 - (1-2\epsilon)) = \epsilon $ and  $ \pi_P^\sigma \le \frac12 (1 + (1-2\epsilon)) = 1- \epsilon. $
	
% 	\textbf{Checking local $ \alpha $-H\"older condition for  $ g_0 $ and $ g_1 $:} Note that 
% 	We shall verify the local smoothness condition for  $ g_1. $ Exact same steps can be followed  to verify smoothness for $ g_0. $ 
	
% 	Since we are interested in limiting smoothness (see definition \ref{def:holder-smooth}) we set our biggest radius of interest to be $ \frac r6. $ We shall show that for any $ x, x' \in \Omega $ with $ \|x-x'\| \le \frac r6 $ \[ \frac{|g_1(x)-g_1(x')|}{\|x-x'\|^\alpha} \le C_\alpha. \] Note that, $ x, x' \in \Omega $ with $ \|x-x'\| \le \frac r6 $ implies the following possible cases:
% 	\begin{enumerate}
% 		\item $ x, x' \in B(z, r/2) $ for some $ z \in \cZ_0. $ In that case, \[ |g_1(x) - g_1(x')| = |a^\sigma q_0 - a^\sigma q_0| = 0 \] and the inequality  holds trivially. 
% 		 \item $ x, x' \in B(z, r/6) $ for some $ z \in \cZ_1. $ In that case,  \[ |g_1(x) - g_1(x')| = |a^\sigma q_1 (1+ \sigma(z) C_\alpha' r^\alpha ) - a^\sigma q_1(1+ \sigma(z) C_\alpha' r^\alpha )| = 0 \] and the inequality  holds trivially again.
% 		 \item $ x \in B(z, r/2) $ and $ x' \in B(z', r/2) $ for some $ z, z' \in \cZ. $ In that case  \[ \|x-x'\| \ge \|z-z'\| - \|x-z\|-\|x'-z'\| \ge r > \frac r 6. \] So, this an invalid case.
% 	\end{enumerate}
	
	
% 	\textbf{Checking Tsybakov's noise condition:}\\ For $ t < C_\alpha' r^\alpha/2, \ Q_X^\sigma \left( 0< \left| \eta_Q^\sigma(X) -\frac12 \right| \le t \right) =0. $ 
% 	For $ t\ge C_\alpha' r^\alpha/2, $ \begin{align*}
% 	Q_X \left( 0< \left| \eta_Q(X) -\frac12 \right| \le t \right) &  = mw\\
% 	& \le c_mc_w r^{\alpha \beta}\\
% 	& \le C_\beta \left( \frac{C_\alpha' r^\alpha}{2}  \right)^\beta.
% 	\end{align*}
	
% 	\begin{align*}
% 	\cE_{Q^\sigma}(h) & = 2\Ex _{Q_X} \left[\left | \eta_Q^\sigma(X) - \frac12 \right | \mathbf{1}\left( h(X) \neq h^*_\sigma(X)  \right)\right]\\
% 	& = C_\alpha' r^\alpha Q_X\left( \{h(X) \ne h_\sigma^*(X)  \} \cap \cX_1 \right).
% 	\end{align*}
% 	We set $ \pi_Q^\sigma = \pi_P^\sigma. $  
	
% 	Let $ \cF $ be the set of all classifier relevant to this classification problem. For $ h,h'\in\cF $ define $ \bar\rho (h,h') \coloneqq C_\alpha' r^\alpha Q_X \left( \{h(X)\neq h'(X)\} \cap \cX_1 \right). $ For $ \sigma\in\{-1,1\}^m, $ let $ h_\sigma^* $ be the Bayes classifier defined as $ h_\sigma^* (x) = \mathbf{1}\{\eta_Q^\sigma(x) \ge 1/2\}. $ Then, for $ \sigma, \sigma'\in\{-1,1\}^m, $  $ \bar\rho (h_\sigma^*, h_{\sigma'}^*) = C_\alpha' r^\alpha w \rho_H(\sigma, \sigma'), $ where, $ \rho_H(\sigma,\sigma') $ is the Hamming distance defined as $ \rho_H(\sigma,\sigma') \coloneqq \text{card} \{z\in\cZ_1 :\sigma(z) \neq \sigma'(z) \}. $
	
	
	
	
% 	Let $\{ \sigma_0,\ldots , \sigma_M \} \subset \{-1,1\}^m  $ be the choice obtained from the  lemma \ref{lemma:varshamov-gilbert}. For each $ i \in \{0,\ldots,M\} $ let us set the distributions of two populations to be $ (P^i, Q^i) = (P^{\sigma_i}, Q^{\sigma_i}). $ For the distribution pair $(P^i,Q^i) $ joint distribution of the dataset $\left\{  \{(X_i^P,Y_i^P)\}_{1\le i\le n_P} , \{X_i^Q\}_{1\le i\le n_Q} \right\} $ $ (\bX,\bY) $ is $ \Pi_i = {P^i}^{\otimes n_p} \otimes {Q_X}^{\otimes n_Q} .$ Note that the distribution $ Q_X $ doesn't depend on $ i. $
	
% 	Denote $ h_{\sigma_i}^* $ by $ h_i^* .$ For $ 0\le i<j\le M, $ \begin{align*}
% 	\bar\rho (h_i^*,h_j^*) &\ge C_\alpha' \frac{wmr^\alpha }{8}\\ 
% 	&\ge \frac12 C_\alpha' c_r^\alpha n_P^{-\frac1{d_0}} c_mr^{\alpha\beta -d} c_w r^d \\
% 	& \ge C n_P^{-\left(\frac{1}{d_0} +\frac{\alpha\beta}{\alpha d_0} \right)}\\
% 	& = C n_p^{-\frac{1+\beta}{d_0}}\\
% 	& =: s.
% 	\end{align*}
	
% 	Let $ D(P|Q) $ be the KL-Divergence between the distributions $ P $ and $ Q. $ Then $ D(\Pi_i| \Pi_0) = n_P D(P^i|P^0) + n_Q D(Q_X|Q_X) = n_P D(P^i|P^0) = n_P D(Q^i|Q^0). $ Now, \begin{align*}
% 	D(Q^i|Q^0)  =&  \int \log\left( \frac{dQ^i}{dQ^0}  \right) dQ^i\\
% 	 =& \int \left[ \log \left( \frac{\eta_Q^i (x)}{\eta_Q^0(x)}  \right) \eta_Q^i(x) + \log \left( \frac{1-\eta_Q^i (x)}{1-\eta_Q^0(x)}  \right) (1-\eta_Q^i(x))  \right] dQ_X\\
% 	 =& \sum_{z: \sigma_i(z) \neq \sigma_0(z)} Q_X \left(B\left( z,\frac r6  \right)  \right) \Bigg[ \log \left( \frac{1+ C_\alpha'r^\alpha}{1- C_\alpha'r^\alpha}  \right) \frac{1+ C_\alpha'r^\alpha}{2}\\
% 	 & +  \log\left( \frac{1- C_\alpha'r^\alpha}{1+ C_\alpha'r^\alpha}  \right) \frac{1- C_\alpha'r^\alpha}{2} \Bigg] \\
% 	 =& w \rho_H(\sigma_i , \sigma_0) \log \left( \frac{1+ C_\alpha'r^\alpha}{1- C_\alpha'r^\alpha}  \right) C_\alpha'r^\alpha\\
% 	 \le & 2mw\frac{C_\alpha'^2 r^{2\alpha}}{1-C_\alpha'r^\alpha}\\
% 	 \le & 4mw C_\alpha'^2 r^{2\alpha}.
% 	\end{align*}  Hence, 
% 	\begin{align*}
% 	D(\Pi_i|\Pi_0) &\le  4mw C_\alpha'^2 r^{2\alpha} n_P\\
% 	&= 4m c_w r^d C_\alpha'^2 r^{2\alpha} n_P\\
% 	& = 4m c_w C_\alpha'^2 r^{2\alpha+d} n_P\\
% 	& = 4m c_w C_\alpha'^2 c_r^{2\alpha+d} n_P^{-\frac{2\alpha +d}{\alpha d_0}} n_P\\
% 	& = 4m c_w C_\alpha'^2 c_r^{2\alpha+d} \text{ since } \alpha d_0 = 2\alpha + d\\
% 	& = 2^5 (\log 2)^{-1} c_w C_\alpha'^2 c_r^{2\alpha+d} \log (M)\\
% 	&\le \frac 18\log (M),  
% 	\end{align*} for $ c_w $ small enough. 
	
	
% 	Hence, by proposition \ref{prop:tsybakov} \begin{align*}
% 	\sup_{(P,Q)\in \Pi} \Ex \cE_Q (\hat f)& \ge \sup_{(P,Q)\in \Pi} s \Pr_\Pi \left ( \cE_Q (\hat f)\ge s \right)\\
% 	& \ge s \sup_{\sigma\in \{-1,1\}^m} \Pi_\sigma \left(\cE_{Q^\sigma} (\hat f)\ge s \right) \\
% 	& \ge s \frac {3-2\sqrt{2}}{8}\\
% 	& \ge C'n_P^{-\frac{1+\beta}{d_0}}
% 	\end{align*}
	
% \noindent \textbf{Part II:}	

% 	Now we  deal with the error of estimation for the parameter $ \pi_Q. $ We shall see that, it is enough to construct two distributions for this purpose.
	

% 	For some $ w = \frac 1{16} $ (to be chosen later) let us define the following class conditional densities: 
	
% 	\[ g_1(x) = \begin{cases}
% 	4w (1-\delta) & \text{if } 0 \le  x_1 \le \frac 14,\\
% 	4\delta & \text{if } \frac 38 \le x_1 \le \frac 58, \\
% 	4(1-\delta)(1-w) & \text{if } \frac 34 \le x_1 \le 1.
% 	\end{cases} \] and \[ g_0(x) = \begin{cases}
% 	4(1-w) (1-\delta) & \text{if } 0 \le  x_1 \le \frac 14,\\
% 	4\delta & \text{if } \frac 38 \le x_1 \le \frac 58, \\
% 	4(1-\delta)w & \text{if } \frac 34 \le x_1 \le 1.
% 	\end{cases} \] Let $ \sigma \in \{-1, 1\}. $ We shall choose $ \delta  $ later. We specify the class probabilities in the following way:
% 	\[ \pi_P = \frac12 , \ \pi_Q^\sigma = \frac 12 (1+\sigma m) \]  where, $  m = \frac 1 {16\sqrt{n_Q}}. $ Then \[ \eta_Q^\sigma (x) = \frac{\pi_Q^\sigma g_1(x)}{\pi_Q^\sigma g_1(x) + (1-\pi_Q^\sigma)g_0(x)} = \begin{cases}
% 	\frac{w(1+\sigma m)}{w(1+\sigma m) + (1-w) (1-\sigma m)} & \text{if }  0 \le  x_1 \le \frac 14,\\
% 	\frac{1+\sigma m}{2} & \text{if } \frac 38 \le x_1 \le \frac 58, \\
% 	\frac{(1-w)(1+\sigma m)}{(1-w)(1+\sigma m) + w (1-\sigma m)} & \text{if } \frac 34 \le x_1 \le 1.
% 	\end{cases} \]
	
% 	Given the class conditional densities and the class probabilities the population distributions can be constructed in the following way: for a Borel set $ A \subset [0,1]^d $ and for index $ y \in \{0,1\} $ \[ P(X\in A, Y = y) = y \pi_P \int_A g_1(x) + (1-y) (1-\pi_P) \int_A g_0(x) \] and 
	
% 	\[ Q^\sigma (X\in A, Y = y) = y \pi_Q^\sigma \int_A g_1(x) + (1-y) (1-\pi_Q^\sigma) \int_A g_0(x). \]
	
% 	It is easy to see that the densities $ g_0 $ and $ g_1 $ are locally $ \alpha $-H\"older smooth with constant $ C_\alpha. $ We need to check the margin  condition. 
	
% 	\textbf{Checking margin condition \ref{def:margin-condition}:} 
	
	
% 	Note that \begin{align*}
% 		\left|\frac{w(1+\sigma m)}{w(1+\sigma m) + (1-w) (1-\sigma m)} - \frac 12\right| & = \frac 12  \frac{|w(1+\sigma m) - (1-w) (1-\sigma m)|}{w(1+\sigma m) + (1-w) (1-\sigma m)}\\ 
% 		& = \frac 12 \frac {|2w +\sigma m -1|}{1-\sigma m + 2\omega\sigma m	}\\
% 		& = \frac 12 \frac {1-2w -\sigma m }{1-\sigma m + 2\omega\sigma m	} \ge \frac 12 \frac {1-3/16}{1+3/16} = \frac {13}{38}
% 	\end{align*}
	
% 	and \begin{align*}
% 		\left| \frac{(1-w)(1+\sigma m)}{(1-w)(1+\sigma m) + w (1-\sigma m)} - \frac 12 \right| & = \frac12 \frac{(1-w)(1+\sigma m)- w (1-\sigma m) }{(1-w)(1+\sigma m) + w (1-\sigma m)} \\
% 		& = \frac 12 \frac{1+\sigma m-2w}{1 +\sigma m- 2w\sigma m} \ge \frac 12 \frac {1-3/16}{1+3/16} = \frac {13}{38}
% 	\end{align*}
	
	
% 	Hence  for $ t < m $ we have \[ Q\left( \left| \eta_Q^\sigma(X) - \frac 12 \right| \le t  \right) = 0 \]. For $ m \le t < \frac{13}{38} $ we have 
% 	\begin{align*}
% 		 Q\left( \left| \eta_Q^\sigma(X) - \frac 12 \right| \le t  \right) &= Q \left( \frac 38 \le X_1 \le \frac 58  \right) = \delta. 
% 	\end{align*}
% 	We choose $ \delta = C_\beta m^\beta . $ Then \[ Q\left( \left| \eta_Q^\sigma(X) - \frac 12 \right| \le t  \right) \le C_\beta m^\beta \le C_\beta t^\beta. \]
% 	and for $ t \ge \frac{13}{38} $ we have \[ Q\left( \left| \eta_Q^\sigma(X) - \frac 12 \right| \le t  \right) \le 1 \le C_\beta t^\beta. \]
	
	
% 	We define our distribution class $ \cH = \{ \Pi_\sigma : \sigma \in \{-1, 1\} \}, $ where $ \Pi_\sigma  $ is defined as \[  \Pi^\sigma = P^{\otimes n_P} \otimes \left(Q_X^\sigma \right)^{\otimes n_Q}. \] Then the Kullback-Leibler divergence between $ \Pi_{-1} $ and $ \Pi_1 $ is \begin{align*}
% 		D\left(  \Pi_1 | \Pi_{-1}  \right)  = & n_Q D\left(Q_X^{(-1)}| Q_X^{(1)}\right)\\
% 		 \le &  n_Q D\left(Q^{(-1)}| Q^{(1)}\right) \ \text{using lemma \ref{lemma:kl-ineq}}, \\
% 		 = &  n_Q \Bigg[ \log\left( \frac{1+\frac{1}{16\sqrt{n_Q}}}{1-\frac{1}{16\sqrt{n_Q}} } \right) \left( 1+\frac{1}{16\sqrt{n_Q}}  \right)\\
% 		 & + \log\left( \frac{1-\frac{1}{16\sqrt{n_Q}}}{1+\frac{1}{16\sqrt{n_Q}} } \right) \left( 1-\frac{1}{16\sqrt{n_Q}}  \right)  \Bigg] \\
% 		  = & \frac {2n_Q}{16\sqrt{n_Q}} \log\left( \frac{1+\frac{1}{16\sqrt{n_Q}}}{1-\frac{1}{16\sqrt{n_Q}} } \right)\\
% 		  \le & \frac{6n_Q}{256 n_Q } \ \text{using } \log\left( \frac{1+x}{1-x} \right) \le 3x \text{ for } 0 \le x\le \frac 12,\\
% 		  = & \frac 3{128}.
% 	\end{align*}
	
% 	Here $ M = |\cH| = 2 $ , $ \Pi_{1} \ll \Pi_{-1} $\\ and $ \frac1M \sum_{\sigma\in \{-1,1\}} D(\Pi^\sigma | \Pi^{-1}) = \frac12 D(\Pi^1 | \Pi^{-1}) = \frac 3 {256} < \frac{\log 2}{8}.  $
	
	
% 	Also, let $ f_\sigma  $ is the Bayes decision rule for distribution $ Q^\sigma,  $ \ie, \ \[ f_\sigma (x) = \indicator\left\{ \eta_Q^\sigma (x)  \ge \frac 12  \right\}. \] Then  \begin{align*}
% 	\cE_{Q^{1}}\left(f_{-1}\right) & = \Ex_{Q^{1}} \left[ \left| \eta_Q^1(X) - \frac 12 \right|\indicator\left\{ f_1(X) \neq f_{-1}(X)  \right\}  \right]\\
% 	& = \delta m \\
% 	& = \frac{C_\beta}{16^{\beta+1}} n_Q^{-\frac{\beta+1}{2}} \triangleq s.
% 	\end{align*}
	
% 		By proposition \ref{prop:tsybakov} \begin{align*}
% 	\sup_{(P,Q)\in \Pi} \Ex \cE_Q (\hat f)& \ge \sup_{(P,Q)\in \Pi} s \Pr_\Pi \left ( \cE_Q (\hat f)\ge s \right)\\
% 	& \ge s \sup_{\sigma\in \{-1,1\}} \Pi_\sigma \left(\cE_{Q^\sigma} (\hat f)\ge s \right) \\
% 	& \ge s \frac {3-2\sqrt{2}}{8}\\
% 	& \ge C'n_Q^{-\frac{1+\beta}{2}}
% 	\end{align*}
	
	
	 
	
% 	Combining these two lower bounds, we get the result.
% \end{proof}





\begin{proof}[\bf{Proof of Theorem \ref{th:upper-bound-unlabeled}}]
	
	\label{proof:th-lower-bnd-unlabeled}
	
	Throughout our study we assume $ \Pr $ to be the probability measure generating the  data.
	
	
	\noindent	\textbf{Step I: Concentration of $ \widehat C(g) $ and $ \widehat \Xi_Q(g) $} 
	
	
	Let $ g $ be a classifier such that the matrix $ C_P(g) $ is invertible.
	Fix $ 0\le i,j\le 1. $ Note that  $\left\{\indicator\left(g(X_l^P) = i, Y_l^P = j \right)\right\}_{l=1}^{n_P} $ are \iid \ Bernoulli random variables with success probability $ P\left( g(X) = i, Y= j  \right) =  C_{i,j} (g) .$ By Lemma \ref{lemma:bernoulli} \[ \text{for any }t>0,\  \Pr\left(\left|\widehat{C}_{i,j}(g) - C_{i,j}(g)\right| > t \right) \le 2\exp\left( - \frac{n_Pt^2}{4} \right). \]
	Hence, we get the element-wise convergence of the matrix $\widehat C(g): $ \[ \text{for any } t>0, \ \Pr \left(\text{for some }0\le i,j\le1, \left|\widehat{C}_{i,j}(g) - C_{i,j}(g)\right| > t  \right)\le 8\exp\left( - \frac{n_Pt^2}{4} \right). \] 
	
	Fix $ i = 0,1. $ We see that $ \left\{\indicator \left\{ g(X_l^Q) =i \right\}  \right\}_{l=1}^{n_Q} $ are \iid \ Bernoulli random variables with success probability $ Q(g(X_l^Q)=i) = \begin{cases}
	\xi_Q(g) & \text{if }i = 1\\
	1- \xi_Q(g) & \text{if } i = 0
	\end{cases}. $ Hence, similarly as before we get: \[ \text{for any } t>0, \ \Pr\left(    \left|\hat \xi_Q(g) - \xi_Q(g) \right|>t  \right) \le 2\exp\left(-\frac{n_Qt^2}{4}\right). \]
	
	By union bound, for any $ t>0 $ with probability at least $  1-8\exp\left( - \frac{n_Pt^2}{4} \right) - 2\exp\left(-\frac{n_Qt^2}{4}\right)  $ we have \[ \text{for } 0\le i, j\le 1, \ \left|\widehat{C}_{i,j}(g) - C_{i,j}(g)\right| \le  t\ \text{and } \left|\hat \xi_Q(g) - \xi_Q(g) \right|\le t . \]
	
	\noindent \textbf{Step II: Concentration of $ \widehat{w} $}
	
	For an invertible  matrix $ A = \left(\begin{matrix}
	a & b \\
	c & d
	\end{matrix}\right) $ and a vector $ v =  \left(\begin{matrix}
	e \\ f
	\end{matrix}   \right) $ we see that \[ A^{-1}v = \frac{1}{ad-bc} \left(\begin{matrix}
	a & -c \\ -b & d
	\end{matrix}\right)\left(\begin{matrix}
	e \\ f
	\end{matrix}   \right) = \frac1{ad-bc} \left(\begin{matrix}
	ae-cf \\ df - be
	\end{matrix}\right). \] Here, $ a = C_{0,0} (g), \ b = C_{0,1}(g), \ c = C_{1,0}(g) $, $ d = C_{1,1}(g ) $ and $ e = Q(f(X) = 0), \ f = Q(f(X)=1). $ We also define $ \hat a = \widehat C_{0,0} (g), \ \hat b = \widehat  C_{0,1}(g), \ \hat c = \widehat  C_{1,0}(g) $, $ \hat d =  \widehat  C_{1,1}(g ) $ and $ \hat e = \widehat  Q(f(X) = 0), \ \hat f = \widehat  Q(f(X)=1). $
	Note that, $0 \le  a,b,c,d,e,f,\hat a, \hat b, \hat c, \hat d, \hat e, \hat f \le 1.$ Then \[ |\hat a\hat d - ad| \le |\hat a -a|+|\hat d - d| \le 2t. \] Using similar inequalities , with probability at least  $  1-8\exp\left( - \frac{n_Pt^2}{4} \right) - 2\exp\left(-\frac{n_Qt^2}{4}\right)  $ we have \begin{enumerate}
		\item $  |\hat a\hat d-\hat b\hat c -ad+bc| \le |\hat a\hat d - ad| + |\hat b\hat c -bc| \le 4t, $
		\item $ |\hat a\hat e-\hat c\hat f -ae+cf| \le |\hat a\hat e -ae| + |\hat c\hat f -cf|\le 4t, $
		\item $ |\hat d\hat f-\hat b\hat e -df+be| \le|\hat d\hat f -df| + |\hat b\hat e -be|  \le 4t, $
	\end{enumerate}
	
	\begin{lemma}
		\label{lemma:ineq-ratio}
		Let  $x \ge 0, \  y >0 $ and $ |\hat x -x |, |\hat y - y| \le \delta < y. $ Then \[ \left| \frac{\hat x}{\hat y} - \frac x y  \right| \le \frac \delta {y - \delta} \left(1+ \frac x y  \right). \]
	\end{lemma}
	\begin{proof}
		\begin{align*}
		\left| \frac{\hat x}{\hat y} - \frac x y  \right| & \le \frac{|\hat x y - \hat y x|}{y \hat y}\\
		& \le  \frac{y |\hat x - x| + x |\hat y - y|}{y \hat y}\\
		& \le \frac{\delta}{\hat y} + \frac{x \delta}{y \hat y }	\\
		& \le \frac{\delta}{ y - \delta} + \frac{x \delta}{y (y - \delta) }
		\end{align*}
	\end{proof}
	Let $ t < \frac14 (ad-bc). $
	Using lemma \ref{lemma:ineq-ratio}, we see that with probability at least $  1-8\exp\left( - \frac{n_Pt^2}{4} \right) - 2\exp\left(-\frac{n_Qt^2}{4}\right) \ge 1- 10 \exp\left( - (n_P\vee n_Q)\frac{t^2}{4} \right)  $ we have
	\begin{align*}
	\left| \widehat{w}_0 - w_0  \right|  =  & \left| \frac{\hat a\hat e-\hat c\hat f}{\hat a\hat d -\hat b\hat c} -\frac{ae - cf}{ad - bc} \right|\\ &  \le \frac{4t}{ad - bc - 4t} \left( 1+ \frac{ae - cf}{ad - bc}   \right)\\ & = \frac{4t}{ad - bc - 4t} (1+w_0)
	\end{align*} and 
	\begin{align*}
	    \left| \widehat{w}_1 - w_1  \right| & = \left| \frac{\hat d\hat f-\hat b\hat e}{\hat a\hat d -\hat b\hat c} -\frac{df - be}{ad - bc} \right| \\&  \le \frac{4t}{ad - bc - 4t} \left( 1+ \frac{df - be}{ad - bc}\right)\\ &  =  \frac{4t}{ad - bc - 4t} (1+w_1).
	\end{align*}
	
	
	
	\noindent \textbf{Step III: Concentration of $ \frac1{n_P}\sum_{ l =1}^{n_P} Y_l^P\widehat w_1K_h (x-X_l^P) $ and $ \frac1{n_P}\sum_{ l =1}^{n_P} (1-Y_l^P)\widehat w_0K_h (x-X_l^P) $}
	
	Let us consider the following notations: Let $  \widehat G_1^{P} = \frac1{\sum_{ l =1}Y_l^P} \sum_{ l : Y_l^P =1 } \delta_{X_l^P} $ be the empirical measure on the set $ \left\{  X_l^P: 0 \le l \le n_P,\  Y_l^P = 1  \right\} .$ Here $ \delta_x  $ denotes the degenerate probability measure on $ x . $
	Similarly, we define  $ \widehat G_0^{P} = \frac1{n_P - \sum_{ l =1}Y_l^P} \sum_{ l : Y_l^P =0 } \delta_{X_l^P} $ as the empirical measure on $ \left\{  X_l^P: 0 \le l \le n_P, \  Y_l^P = 0  \right\} . $ Let $  \hat u = \frac1{n_P}\sum_{ l =1}^{n_P} Y_l^P\widehat w_1K_h (x-X_l^P)  $,  $ \hat v = \frac1{n_P}\sum_{ l =1}^{n_P} (1-Y_l^P)\widehat w_1K_h (x-X_l^P) $, $ u = w_1 \pi_P g_1(x) $ and $  w_0 (1-\pi_P) g_0(x). $ We shall determine the concentration of $ |\hat u - u| + |\hat v - v|. $
	
	\vspace{0.2in}
	
	Let $ K :\reals^d \to [0,\infty) $ be a kernel with $ \int_{\reals^d} K(x) dx = 1. $ For some  $ h >0 $ let $ \cF_h = \left\{  K\left( \frac{\cdot - x}{h} \right): x \in \reals^d  \right\}. $ Then $ d_{\cF_h} \le d+1. $ According to Corollary \ref{cor:empirical-convergence}, with probability at least $ 1-\delta  $  for any $ f \in \cF_h $
	
	
	\begin{align*}
	|\nu_n(f) - \nu(f)| & \le \begin{cases}
	\sqrt{6\nu(f)\alpha_n} + \alpha_n & \text{if } 3\nu(f) \ge 2 \alpha_n,\\
	3\alpha_n & \text{if } 3\nu(f) < 2\alpha_n
	\end{cases} \\
	& \le  \sqrt{6\nu(f)\alpha_n} + 3\alpha_n. 
	\end{align*}
	
	Note that \begin{align*}
	|\hat u - u| \le & \hat \pi_P \widehat w_1 \left| \widehat{G}^P_1 \left(\frac1{h^d} K_h \left(  \frac{x-\cdot}{h}  \right)  \right) -g_1(x)\right|\\ & + \hat \pi_P g_1(x) \left|\widehat w_1 - w_1 \right| +  w_1 g_1(x) |\hat \pi_P - \pi_P| 
	\end{align*} and 
	\begin{align*}
	    |\hat v - v| \le &  (1- \hat \pi_P )\widehat w_0 \left| \widehat{G}^P_0 \left(\frac1{h^d} K_h \left(  \frac{x-\cdot}{h}  \right)  \right) -g_0(x)\right|\\ &  + (1-\hat \pi_P) g_0(x) \left|\widehat w_0 - w_0 \right| +   w_0 g_0(x) |\hat \pi_P - \pi_P|  
	\end{align*}
	To bound $ \left|  \widehat{G}^P_1 \left(\frac1{h^d} K_h \left(  \frac{x-\cdot}{h}  \right)  \right)  - g_1(x)  \right| $ we notice that 

	\begin{align*}
		& \left|  \widehat{G}^P_1 \left(\frac1{h^d} K_h \left(  \frac{x-\cdot}{h}  \right)  \right)  - g_1(x)  \right|\\   & \hspace{0.1in}\le   \left| \widehat{G}^P_1 \left(\frac1{h^d} K_h \left(  \frac{x-\cdot}{h}  \right)  \right) - \popone \right| \\ & \hspace{0.15in}+ \left| \popone - g_1(x) \right|
	\end{align*}
	
	 A high probability upper bound for $ \left| \widehat{G}^P_1 \left(\frac1{h^d} K_h \left(  \frac{x-\cdot}{h}  \right)  \right) - \popone \right| $ is obtained using Corollary \ref{cor:empirical-convergence}. We shall use smoothness of $ g_1 $ to bound $ \left| \popone - g_1(x) \right|. $
	
	
	From the definition of locally $ \alpha $-H\"older smoothness of $ g_0 $ and $ g_1 $ (definition \ref{def:holder-smooth}) there is some $ \delta_0 >0 $ such that for any $ \delta \in (0, \delta_0] $ and for any $x, x' \in \Omega$ with $\|x-x'\|_2 \le \delta $ we have  \[  \max\{ |g_0(x)-g_0(x')|, |g_1(x) - g_1(x')| \} \le (C_\alpha+1) \|x-x'\|_2^\alpha.   \]
	
	Let $ a>\alpha $ be such that $ C_a \triangleq \int_{\reals^d} \|x\|_2^a K(x) dx <\infty   $ (such an $ a $ exists because $ K \in \cK(\alpha) $). Using Markov's inequality, for any $ R>0 $ \[ \int_{\|x\| > R} K(x)dx \le \frac1{R^a} \int_{\reals^d} \|x\|^a K(x) dx = h^\alpha  \] if $ R = C_a^{\frac1 a} h^{- \frac  \alpha a }. $ Let $ h_0 \triangleq \left(\frac{\delta_0}{C_a^{\frac1 a}}  \right)^{\frac a{a-\alpha}} . $ Then for any $ h \in (0, h_0) $ if we let $ R(h) = C_a^{\frac1 a} h^{- \frac \alpha a } $ we have the followings:
	\begin{enumerate}
		\item  $ \int_{\|x\| > R(h)} K(x)dx \le h^\alpha, $ and 
		\item $ h R(h) = C_a^{\frac1 a} h^{1-\frac \alpha a } \le C_a^{\frac1 a} h_0^{\frac {a-\alpha} a } = \delta_0. $
	\end{enumerate}
	Note that 
	\begin{align*}
	\popone - g_1(x)  = &  \int \frac{1}{h^d} K\left( \frac{y - x}{h} \right)(g_1 (y)- g_1(x))dy\\
 =& \int_{\reals^d} K(z) (g_1(x+ zh)- g_1(x)) dz \\
	 = & \underbrace{\int_{\|z\|\le R(h)} K(z) (g_1(x+ zh)- g_1(x)) dz}_{(I)}\\ &  + \underbrace{\int_{\|z\|> R(h)} K(z) (g_1(x+ zh)- g_1(x)) dz}_{(II)}.
	\end{align*}
	
	Now, for $ \|z\|\le R(h) $ we have $\|zh\| \le  h R(h) \le \delta_0.$ For such $ z $ we have $ |g_1(x+zh) - g_1(x)| \le \|zh\|^\alpha = h^\alpha \|z\|^\alpha. $ Hence,  \begin{align*}
	|(I)|  \le &  \int_{\|z\|\le R(h)} K(z) |g_1(x+ zh)- g_1(x)| dz\\
	\le & \int_{\|z\|\le R(h)} K(z) h^\alpha \|z\|^\alpha dz \\
	\le & h^\alpha \int_{\reals^d} \|z\|^\alpha K(z) dz \\
	\le &  h^\alpha \int_{\reals^d} \left( 1+ \|z\|^a \right) K(z) dz\\
	= & (1+C_a) h^\alpha.
	\end{align*}
	
	Since the densities are bounded by $ \mu_+, $ we have \begin{align*}
	|(II)| \le & \int_{\|z\|> R(h)} K(z) |g_1(x+ zh)- g_1(x)| dz\\
	\le &  \mu_+ \int_{\|z\|> R(h)} K(z)dz \le \mu_+ h^\alpha.
	\end{align*}
	Combining $ (I) $ and $ (II) $ we get,  \[ \text{for } h \le h_0, \  \left|\popone - g_1(x) \right| \le (1+C_a + \mu_+) h^\alpha = c_1(\alpha)h^\alpha. \] Similarly we can get the bound \[\text{for } h \le h_0, \ \left|\popzero - g_0(x) \right| \le  c_1(\alpha)h^\alpha.  \]
	
	
	
	By Corollary \ref{cor:empirical-convergence}, with probability at least $ 1- 2\delta $ for any $ x $ and $ k \in  \{0,1\}, $ 
	\begin{align}
	\label{eq:concentration-kde-no-label-1}
	& \left| \widehat G_k^P \left( \frac{1}{h^d} K\left( \frac{\cdot - x}{h} \right)  \right) -  G_k \left( \frac{1}{h^d} K\left( \frac{\cdot - x}{h} \right)  \right) \right| \nonumber \\ \le &  \sqrt{6\frac{\alpha_m}{h^d} G_k \left( \frac{1}{h^d} K\left( \frac{\cdot - x}{h} \right)  \right) } + \frac{\alpha_m}{h^d} \nonumber\\
	\le & \sqrt{6\frac{\alpha_m}{h^d} (g_k(x)+ c_1(\alpha)h^\alpha) } + \frac{\alpha_m}{h^d} 
	\end{align} where $ \alpha_m = \frac{d_{\cF}\log(2n)+\log (1/\delta) }{m}. $
	Here, $ m $ is the minimum sample size for label $ 0 $ and $ 1 $ in $ P $-data. Since for some $ \epsilon > 0, \ \epsilon \le \pi_P \le 1- \epsilon$, letting $ t < \frac \epsilon 2 $ we see that with probability at least $ 1- 2\exp\left(- \frac{n_Pt^2}{4}  \right) $ we have \[ |\hat \pi_P - \pi_P | \le t \text{ or } m \ge \frac{n_P \epsilon}2. \]
	
	Let $ A $ be the event under which the following holds: \begin{enumerate}
		\item $ 	\left| \widehat G_k^P \left( \frac{1}{h^d} K\left( \frac{\cdot - x}{h} \right)  \right) -  G_k \left( \frac{1}{h^d} K\left( \frac{\cdot - x}{h} \right)  \right) \right| \le \sqrt{6\frac{\alpha_m}{h^d} (g_k(x)+ c_1(\alpha)h^\alpha) } + \frac{\alpha_m}{h^d} $
		\item For $k = 0,1, \  |\widehat w_k-w_k| \le \frac{4t}{\text{det}(C(g))-4t} (1+w_k) $
		\item $ |\hat \pi_P - \pi_P| \le t $
	\end{enumerate}
	Note that $ \Pr(A) \ge 1-\delta - 2\exp\left(- \frac{n_Pt^2}{4}  \right) - 10 \exp\left( - (n_P\vee n_Q)\frac{t^2}{4} \right). $
	Under the event $ A $ \begin{align*}
	|\hat u - u| + |\hat v - v| \le  & \  \hat \pi_P \widehat w_1 \left(  \sqrt{6\frac{\alpha_m}{h^d} (g_1(x)+ c_1(\alpha)h^\alpha) } + \frac{\alpha_m}{h^d} +c_1(\alpha) h^\alpha \right) \\
	& +(1- \hat \pi_P) \widehat w_0 \left(  \sqrt{6\frac{\alpha_m}{h^d} (g_0(x)+ c_1(\alpha)h^\alpha) } + \frac{\alpha_m}{h^d} +c_1(\alpha) h^\alpha \right) \\
	& + \hat \pi_P g_1(x) \frac{4t}{\text{det}(C(g))-4t} (1+w_1) \\ & + (1- \hat \pi_P) g_0 (x)  \frac{4t}{\text{det}(C(g))-4t}(1+w_0) \\
	& + w_1 g_1(x) t + w_0 g_0(x) t
	\end{align*}
	
	
	Let us denote $ \text{det}(C(g)) $ as $ \Delta. $
	In the above bound we shall use the following inequalities to simplify it farther:
	\begin{enumerate}
		\item $ t \le \frac1 {32} \Delta \le  \frac18 \Delta, $
		\item  $ w_1 \le \frac{\pi_Q}\delta $ and $ w_0 \le \frac{1-\pi_Q}{\delta}, $
		\item For $ k = 0,1, $ $ \frac{4t}{\Delta - 4t} (1+w_k) \le \frac{16t}{\delta \Delta}  $
		
		\item \begin{align*}
		\hat \pi_P \widehat w_1 \le \widehat w_1 \le w_1 +  \frac{4t}{\Delta-4t} (1+w_1) \le \frac{16t}{\delta \Delta} + \frac{ \pi_Q} {\delta},
		\end{align*}
		\item Similarly, $ (1-\hat \pi_P) \widehat w_0 \le \frac{16t}{\delta \Delta} + \frac{1-\pi_Q} {\delta}. $
	\end{enumerate}
	
	
	
	
	
	The above bound for $ |\hat u - u| + |\hat v - v| $ simplifies to \begin{align*}
	|\hat u - u| + |\hat v - v| \le & \left( \frac{16t}{\delta \Delta} + \frac{ \pi_Q} {\delta}  \right) \left(  \sqrt{6\frac{\alpha_m}{h^d} (g_1(x)+ c_1(\alpha)h^\alpha) } + \frac{\alpha_m}{h^d} +c_1(\alpha) h^\alpha \right) \\
	& + \left( \frac{16t}{\delta \Delta} + \frac{ 1-\pi_Q} {\delta}  \right)\left(  \sqrt{6\frac{\alpha_m}{h^d} (g_0(x)+ c_1(\alpha)h^\alpha) } + \frac{\alpha_m}{h^d} +c_1(\alpha) h^\alpha \right)\\
	& + \frac{16t}{\delta \Delta}  (g_1(x) + g_0(x) ) + \frac t \delta \left(  \pi_Q g_1(x) + (1-\pi_Q) g_0(x
	)  \right) \\
	\le & \left( \frac{32t}{\delta \Delta} + \frac{ 1} {\delta}  \right) \left(  \sqrt{6\frac{\alpha_m}{h^d} (\mu_+ + c_1(\alpha)h^\alpha) } + \frac{\alpha_m}{h^d} +c_1(\alpha) h^\alpha \right) \\
	& + \frac{32t}{\delta \Delta} \mu_+ + \frac t \delta \mu_+ \\
	\le & \left( \frac{32t}{\delta \Delta} + \frac{ 1} {\delta}  \right) \left(  \sqrt{6\frac{\alpha_m}{h^d} 2\mu_+ } + \frac{\alpha_m}{h^d} +c_1(\alpha) h^\alpha \right) + \frac{32t}{\delta \Delta} \mu_+ + \frac t \delta \mu_+, \\ & \hspace{2.5in} \text{for } h^\alpha \le \frac{\mu_+}{c_1(\alpha)},\\
	\le & \frac2 \delta \left(  \sqrt{12\mu_+\frac{\alpha_m}{h^d}  } + \frac{\alpha_m}{h^d} +c_1(\alpha) h^\alpha \right) + \frac{32t}{\delta \Delta} \mu_+ + \frac t \delta \mu_+, \ \text{since } t \le \frac \Delta {32}.\\
	\end{align*}
	Letting $ h = C n_P^{- \frac{1}{2\alpha + d}} $ for some $C>0$ and $ \delta = (2n_P)^{d+1} \exp \left( -c_3(\alpha) t^2 m^{\frac{2\alpha}{2\alpha+d}}\right) $ we see that  \[ \frac{\alpha_m}{h^\alpha} = \frac{c_3(\alpha)t^2 n_P^{-\frac d{2\alpha + d}}}{n_P^{-\frac{d}{2\alpha + d}}} = c_4(\alpha) t^2. \]
	Since, $ t < 1, $ we have \[ |\hat u - u| + |\hat v - v| \le c_5(\alpha) t + c_6(\alpha) n_P^{-\frac \alpha{2\alpha + d}} \]
	
	For  $ m \ge \frac{n_P\epsilon}{2} $ and an appropriate choice of $ c_7(\alpha) $ which is independent of sample sizes, \[ \delta = (2m)^{d+1} \exp \left( -c_3(\alpha) t^2 m^{\frac{2\alpha}{2\alpha+d}}\right) \le  \exp \left( -c_7(\alpha) t^2 n_P^{\frac{2\alpha}{2\alpha+d}}\right). \]
	
	Finally, with probability at least $ 1- 12 \exp \left( - (n_P\wedge n_Q) \frac{t^2}{4} \right) - \exp \left( -c_7(\alpha) t^2 n_P^{\frac{2\alpha}{2\alpha+d}}\right)$ we have \[ |\hat u - u| + |\hat v - v| \le c_5(\alpha) t + c_6(\alpha) n_P^{-\frac \alpha{2\alpha + d}}. \]
	
	
	\noindent \textbf{Step IV: Concentration of $ \hat\eta_Q $}
	
	Note that, according to the above notation $ \hat \eta_Q(x) = \frac{\hat u}{\hat u + \hat v} $ and $ \eta_Q(x) = \frac{u}{u + v}. $ Then \begin{align*}
	|\hat \eta_Q(x) - \eta_Q(x)| & = \left| \frac{\hat u }{\hat u + \hat v} - \frac u {u+v}\right|\\
	& = \frac{|\hat u v - u \hat v|}{(\hat u + \hat v)(u + v)} \\
	& \le \frac{|\hat u - u| \hat v + \hat u |\hat v - v|}{(\hat u + \hat v)(u + v)} \\
	& \le \frac{(|\hat u - u|+ |\hat v-v| )(\hat v + \hat u)}{(\hat u + \hat v)(u + v)} \\
	& = \frac{|\hat u - u|+ |\hat v-v| }{u + v}
	\end{align*}
	
	Here, $ u + v = \pi_P w_1 g_1(x) + (1-\pi_Q)w_0 g_0(x) = \pi_Q g_1(x) + (1-\pi_Q)g_0(x) \ge \mu_-. $ Hence, \[ 	|\hat \eta_Q(x) - \eta_Q(x)| \le \frac{|\hat u - u|+ |\hat v-v| }{\mu_-} \le\frac{c_5(\alpha) t + c_6(\alpha) n_P^{-\frac \alpha{2\alpha + d}} }{\mu_-}  \] with probability at least 
	
	\begin{align*}
	  &   1- 12 \exp \left( - (n_P\vee n_Q) \frac{t^2}{4} \right) - \exp \left( -c_7(\alpha) t^2 n_P^{\frac{2\alpha}{2\alpha+d}}\right)\\ & \ge  1- 13\exp \left( -c_7(\alpha) t^2 \left(n_P^{\frac{2\alpha}{2\alpha+d}}\wedge n_Q \right)\right)   .
	\end{align*}
	
	Letting $ \frac{c_5(\alpha) t + c_6(\alpha) n_P^{-\frac \alpha{2\alpha + d}} }{\mu_-} = \eta  $ we see that \[ 	|\hat \eta_Q(x) - \eta_Q(x)| \le  \eta   \] with probability at least \begin{align*}
& 	1- 13\exp \left( -c_7(\alpha) t^2 \left(n_P^{\frac{2\alpha}{2\alpha+d}}\wedge n_Q \right)\right) \\ & =   1- 13 \exp \left( -c_7(\alpha) \left( \frac{\mu_- \eta - c_6(\alpha) n_P^{-\frac\alpha {2\alpha+d}} }{c_5(\alpha)} \right)^2 \left(n_P^{\frac{2\alpha}{2\alpha+d}}\wedge n_Q \right)\right)
	\end{align*}
	For $ a, b\ge 0 $ note that \[ 2(a-b)^2 + 2b^2 \ge a^2 \text{ or } (a-b)^2 \ge \frac {a^2} 2 - b^2.  \] Using the above inequality we get 
	\begin{align*}
	& 13 \exp \left( -c_7(\alpha) \left( \frac{\mu_- \eta - c_6(\alpha) n_P^{-\frac\alpha {2\alpha+d}} }{c_5(\alpha)} \right)^2 \left(n_P^{\frac{2\alpha}{2\alpha+d}}\wedge n_Q \right)\right)\\
	 \le &  13  \exp \left( -c_7(\alpha) \left( \frac{\mu_-^2 \eta^2  }{2c_5^2(\alpha)} - \frac{c_6^2(\alpha)n_P^{-\frac{2\alpha}{2\alpha+d}} }{c_5^2(\alpha)} \right) \left(n_P^{\frac{2\alpha}{2\alpha+d}}\wedge n_Q \right)\right)\\
	 = &  13  \exp \left( c_7(\alpha)  \frac{c_6^2(\alpha)n_P^{-\frac{2\alpha}{2\alpha+d}} }{c_5^2(\alpha)}  \left(n_P^{\frac{2\alpha}{2\alpha+d}}\wedge n_Q \right)\right)\\ & \exp \left( -c_7(\alpha) \frac{\mu_-^2 \eta^2  }{2c_5^2(\alpha)} \left(n_P^{\frac{2\alpha}{2\alpha+d}}\wedge n_Q \right)\right) \\
	 = & c_8(\alpha) \exp \left(  - c_9(\alpha) \eta^2 \left(n_P^{\frac{2\alpha}{2\alpha+d}}\wedge n_Q \right)  \right).
	\end{align*}
	
	Finally we get the concentration bound 
	\begin{align*}
	    & \Pr\Big( |\hat\eta_Q(x) - \eta_Q(x)| \le \eta \text{ for any } x \in \Omega \Big) \\ &  \ge 1-c_8(\alpha) \exp \left(  - c_9(\alpha) \eta^2 \left(n_P^{\frac{2\alpha}{2\alpha+d}}\wedge n_Q \right)  \right).
	\end{align*}
	
	\noindent \textbf{Step V: Bound for $ \Ex \cE_Q(\hat f ) $}
	
	To get a bound for $ \Ex \cE_Q(\hat f) $ we define the following events: $$ A_0 = \left\{ x\in \reals^d: 0< \left| \eta_Q(x) - \frac12\right| < \xi        \right\} $$ and for $j \ge 1, $ $$   A_j = \left\{ x\in \reals^d: 2^{j-1}< \left| \eta_Q(x) - \frac12\right| < 2^j\xi        \right\}  $$ Now, \begin{align*}
	\cE_Q(\hat f)  = & 2 \Ex_X \left(\left| \eta_Q(X) -\frac12 \right|\indicator_{\{\hat f(X)\neq f^*(X)\}}  \right) \\
	= & 2\sum_{j=0}^\infty \Ex_X\left(\left| \eta_Q(X) -\frac12 \right|\indicator_{\{\hat f(X)\neq f^*(X)\}} \indicator_{\{X\in A_j\}} \right) \\
	\le & 2 \xi \Ex_X\left( 0< \left| \eta_Q(X) -\frac12 \right|< \xi  \right) \\
	& + 2\sum_{j=1}^\infty \Pr_X\left(\left| \eta_Q(X) -\frac12 \right|\indicator_{\{\hat f(X)\neq f^*(X)\}} \indicator_{\{X\in A_j\}} \right)
	\end{align*}
	On the event $ \{ \hat f\neq f^*  \} $ we have $ \left| \eta_Q - \frac12 \right| \le \left| \hat \eta - \eta \right|. $ So, for any $ j \ge 1 $ we get \begin{align*}
	\Ex_X&\Ex \left(\left| \eta_Q(X) -\frac12 \right|\indicator_{\{\hat f(X)\neq f^*(X)\}} \indicator_{\{X\in A_j\}} \right) \\
	& \le 2^{j+1}\xi \Ex_X\Ex \left(\indicator_{\{|\hat \eta_Q(X)- \eta_Q(X)| \ge2^{j-1}\xi \}} \indicator_{\{0< |\eta_Q(X)-1/2|<2^{j}\xi\}} \right) \\
	& = 2^{j+1}\xi \Ex_X \left[\Pr\left(\indicator_{\{|\hat \eta_Q(X)- \eta_Q(X)| \ge2^{j-1}\xi \}}\right) \indicator_{\{0< |\eta_Q(X)-1/2|<2^{j}\xi\}} \right] n\\
	& \le 2^{j+1}\xi \exp\left(-a(2^{j-1}\xi)^2\right)\Pr_X (0< |\eta_Q(X)-1/2|<2^{j}\xi)\\
	& \le 2C_\beta 2^{j(1+\beta)}\xi ^{1+\beta} \exp\left(-a(2^{j-1}\xi)^2\right).
	\end{align*} where $ a = c_9\left(n_P^{\frac{2\alpha}{2\alpha + d}} \wedge  n_Q\right). $
	Letting $ \xi = a^{-\frac12}  $ we get \begin{align*}
	\sup_{\Pr \in \cP}\Ex\cE(\hat f) & \le 2C_\beta \left( \xi^{1+\beta} + \sum_{j\ge 1}  2^{j(1+\beta)} \xi^{1+\beta}\exp\left(-a(2^{j-1}\xi)^2\right)   \right) \\
	& \le C \left(n_P^{\frac{2\alpha}{2\alpha + d}} \wedge n_Q\right)^{-\frac{1+\beta}{2}}\\
	& \le C \left(n_P^{-\frac{2\alpha}{2\alpha + d}} \vee n_Q^{-1}\right)^{\frac{1+\beta}{2}}.
	\end{align*}
	
	
\end{proof}



\section{Choice of pilot classifier}
\label{appendix:choice-of-g}
\begin{theorem}[\citet{vapnik16ja}]
Let $  P  $ be a probability defined on $ \cX. $ Let $ X_1 , \dots, X_n \sim \iid\ P. $ Define $ P_n = \frac 1n \sum_{i=1}^n \delta_{X_i}. $	Let $ \cF $ be a class of binary functions defined on the space $ \cX $ and $ s(\cF,n) $ is the shattering number of $ \cF $.  For any $ t > \sqrt{\frac{2}{n}}, $ \[ \Pr \left( \sup_{f \in \cF} |P_nf - Pf| > t \right) \le 4s(\cF, 2n) e^{-nt^2/8}. \]
\end{theorem}
\begin{corollary}
	\label{lemma:g-1}
	Let $ (P,Q)\in \Pi $ and let $ (X_1^P, Y_1^P), \dots , (X_{n_P}^P, Y_{n_P}^P)\sim \iid \ P  $ and $ X_1^Q, \dots, X_{n_Q}^Q   \sim\iid \ Q_X $ For $ w = (w_0,  w_1^T)^T \in \reals \times \reals^d $  let us define the following classifier:
	\[ h_w (x) \triangleq \indicator\{  w_1^Tx  + w_0  > 0 \}. \] For $ i,j \in \{0,1\} $ let us define \[ Z_{i,j} (n_P) = \sup_{w \in \reals^{d+1}} \left| \frac 1{n_P} \sum_{ l =1}^{n_P} \indicator\left\{ h_w(X_l^P) = i, Y_l^P = j  \right\} - P\left( h_w(X) = i, Y = j  \right)   \right| \] and for $  i \in \{0,1\} $ let us define  \[ W_i(n_Q) = \sup_{w \in \reals^{d+1}} \left| \frac 1{n_Q} \sum_{ l =1}^{n_Q} \indicator\left\{ h_w(X_l^Q) = i \right\} - P\left( h_w(X) = i  \right)   \right|   \] Then for any $ t > \max\left\{ \sqrt{\frac 2 {n_P}}, \sqrt{\frac 2{n_Q}} \right\} $ \[ \Pr\left( Z_{i,j}(n_P) >  t \right) \le 4\left(\frac{2en_P}{d+1}  \right)^{d+1}e^{-n_Pt^2/8}  \] and \[ \Pr\left( W_i(n_Q) >  t \right) \le 4\left(\frac{2en_Q}{d+1}  \right)^{d+1}e^{-n_Qt^2/8}. \]
\end{corollary}
\begin{proof}
	Since VC dimension of $ \cF = \{ h_w : w\in \reals^d \} $ is $ d+1,  $ for $ n \ge d+1 $  we get $ s(\cF, n) = \left(\frac{en}{d+1} \right)^{d+1}. $\end{proof}

%\begin{corollary}
%	Let $ (P,Q)\in \Pi $ and let $ (X_1, Y_1), \dots , (X_n, Y_n)\sim \iid \ P . $ For $ w = (w_0, \tilde w^T)^T \in \cS^{d}\triangleq \{ x \in\reals^{d+1} : \|x\|_2 = 1 \} $ with $ w_0 \in \reals, $ and $ \tilde w \in \reals^d $ let us define the following classifier:
%	\[ h_w (x) \triangleq \indicator\{ \tilde w^Tx  + w_0  > 0 \}. \] Let us also define $ \widehat C_n(w) $ and $ C(w) $ to be the determinant of the sample and population  version of confusion matrix of $ h_w $ and  \[ \cZ(n)  = \sup_{w \in \cS^{d}} \left| \widehat C_n(w) - C(w)  \right|. \] Then for any $ t > 0 $ \[ \Pr\left( \cZ(n) >  t \right) \le 8\left(\frac{en}{d+1}  \right)^{d+1}e^{-\frac{nt^2}{128}} . \]
%\end{corollary}
%
%\begin{proof}
%	Let us define the empirical probability measure as $  \widehat P_n \triangleq \frac1 n \sum_{l=1}^n \indicator_{(X_l, Y_l)}. $ Then \begin{align*}
%	&	|\widehat P_n (h_w(X) = 1, Y = 1) \widehat P_n (h_w(X) = 0, Y = 0)  -  P (h_w(X) = 1, Y = 1)  P (h_w(X) = 0, Y = 0) | \\
%	\le &    \widehat P_n (h_w(X) = 1, Y = 1) |\widehat P_n (h_w(X) = 0, Y = 0)  -    P (h_w(X) = 0, Y = 0) |\\
%	& +  \widehat P_n (h_w(X) = 0, Y = 0) |\widehat P_n (h_w(X) = 1, Y = 1)  -    P (h_w(X) = 1, Y = 1) |\\
%	& \le  |\widehat P_n (h_w(X) = 0, Y = 0)  -    P (h_w(X) = 0, Y = 0) | +   |\widehat P_n (h_w(X) = 1, Y = 1)  -    P (h_w(X) = 1, Y = 1) |.
%	\end{align*}
%	Similarly, \begin{align*}
%		& |\widehat P_n (h_w(X) = 1, Y = 0) \widehat P_n (h_w(X) = 0, Y = 1)  -  P (h_w(X) = 1, Y = 0)  P (h_w(X) = 0, Y = 1) | \\
%		& \le  |\widehat P_n (h_w(X) = 1, Y = 0)  -    P (h_w(X) = 1, Y = 0) | +   |\widehat P_n (h_w(X) = 0, Y = 1)  -    P (h_w(X) = 0, Y = 1) |.
%	\end{align*}
%	Hence, \[ \sup_{w \in \cS^{d}}\left| \widehat C_n(w) -  C(w)  \right| \le \sum_{i,j\in \{0,1\}}\sup_{w \in \cS^{d}} |\widehat P_n (h_w(X) = i, Y = j)  -    P (h_w(X) = i, Y = j) |.  \] This follows 
%	\begin{align*}
%		\Pr \left( \cZ(n) > 4t \right) \le & \Pr\left( \exists i,j \in \{0,1\} \text{ such that } Z_{i,j}(n) > t  \right) \\ 
%		\le & \sum_{i,j\in \{i,j\}} \Pr \left( Z_{i,j}(n) > t \right)\\
%		\le & 8\left(\frac{en}{d+1}  \right)^{d+1}e^{-nt^2/8}.
%	\end{align*}
%	Substituting $ t $ by $ t/4 $ we get the result.
%\end{proof}


\begin{lemma}
	\label{lemma:g-2}
	Let $ R>0, $ $ (P,Q)\in \Pi $ and let $ (X_1^P, Y_1^P), \dots , (X_{n_P}^P, Y_{n_P}^P)\sim \iid \ P . $ Consider the loss function $ \ell : \{0,1\}\times \reals^{d} \times \reals^{d+1} \to \reals $ defined as $ \ell(y, x, (b_0,  b_1^T)^T) = y(x^Tb_1 + b_0) - \log \left( 1+ e^{x^T b_1 + b_0}  \right) . $ Let us define \[ b^* = (b_0^*, ( b_1^*)^T)^T = \argmin_{(b_0,  b_1^T)^T \in \reals^{d+1}} E_P\left[\ell(Y, X, (b_0,  b_1^T)^T)\right]  \] and \[ \hat b = (\hat b_0,  \hat b_1^T)^T = \argmin_{\substack{b = (b_0,  b_1^T)^T \in \reals^{d+1}\\ \|b- b^*\|_2 \le R}} \left[\frac 1{n_P} \sum_{ l =1}^{n_P}\ell(Y_i^P, X_i^P, (b_0,  b_1^T)^T)\right]. \] Then, for any $ t >0 $ \[ \Pr \left( \|\hat b - b^* \|_2^2 > t  \right) \le 2R^{d+1}\left( 1+ \frac{12\sqrt{d}}{t} \right)^{d+1}e^{-cn_Pt^2}  \] for some $ c>0. $
\end{lemma}

\begin{proof}
	
\noindent \textbf{Step I:}	
Let $ B(b^*, R) = \{ b \in \reals^{d+1}: \|b-b^*\|_2 \le R \} $ and \\$ \cF = \left\{ f_b(x, y) = yx^Tb - \log\left(1+e^{x^Tb} \right) \Big| b \in B(b^*, R) \right\} \subset \reals^{\reals^d\times \{0,1\}} $ be the class of all loss functions. Then for any $ b \in B(b^*, R) $ we have \[  |x^Tb| \le \|x\|_2\|b\|_2 \le \sqrt{d}(R+ \|b^*\|_2).   \] This implies \[ |f_b(x,y)| \le |x^Tb| + \log \left( 1+ e^{x^Tb} \right) \le 3|x^Tb| \le 3\sqrt{d} (R+\|b^*\|_2) \triangleq L  \] or \[  \|f_b\|_\infty \le L \text{ for any } b \in B(b^*, R). \] 

\noindent \textbf{Step II:} Let $ b, b' \in B(b^*, R). $ Then \begin{align*}
   f_b(x,y) - f_{b'}(x,y) &= yx^T(b-b') + \log \left( 1+ e^{x^Tb'} \right) - \log \left( 1+ e^{x^Tb} \right) \\
   &= yx^T(b-b')  - x^T(b-b') \frac{e^{a}}{1+e^a}\\
   & = x^T(b-b')\left[ y -\frac{e^{a}}{1+e^a}  \right]
\end{align*} for some $ a  $ in between $ x^Tb $ and $ x^Tb'. $ Hence, \[ |f_b(x,y) - f_{b'}(x,y)| \le 2\|x\|_2 \|b-b'\|_2\le 2\sqrt{d}\|b-b'\|_2.  \] This implies \[ \|f_b-f_{b'}\|_\infty \le 2\sqrt{d} \|b-b'\|_2 \text{ for }b,b' \in B(b^*, R). \]

\noindent \textbf{Step III:} Let $ \epsilon > 0 $ and $ B' $ be the $ \frac\epsilon{2\sqrt d} $-covering set of $ B(b^*, R), $ \ie \    $ B' \subset B(b^*, R) $ be a minimal set such that for any $ b \in B(b^*, R) $ there is a $ b'\in B' $ such that $ \|b-b'\|_2 \le \frac \epsilon {2\sqrt d}. $ Then \[ |B'| \le R^{d+1} \left( 1+ \frac{4\sqrt{d}}{\epsilon} \right)^{d+1}. \] Let's define  $ \cF' = \{f_b: b \in B'\}.  $ Then for any $ b \in B(b^*, R) $ we choose $ b' \in B' $ such that $ \|b-b'\|_2 \le \frac \epsilon {2\sqrt d}. $ Then \[ \|f_b - f_{b'}\|_\infty \le \epsilon. \] This implies $ \cF' $ is an $ \epsilon $-covering set for $ \cF.  $ Hence, \[ N(\epsilon , \cF, \|\cdot\|_\infty ) \le R^{d+1} \left( 1+ \frac{4\sqrt{d}}{\epsilon} \right)^{d+1}.  \]

\noindent \textbf{Step IV:} Let $ t > 0. $ Letting $  \epsilon = \frac t3 $ we get $ \cF' $ as an  $ \epsilon $-cover for $ \cF. $ Let $ \widehat P_{n_P} = \frac{ 1}{n_P} \sum_{l=1}^{n_P} \delta_{(X_l^P, Y_l^P)}. $ For $ f \cF $ let $ f' \in \cF' $ such that $ \|f-f'\|_\infty \le \epsilon. $ Then \begin{align*}
	\left| \widehat P_{n_P} f - Pf \right| & \le \left| \widehat P_{n_P} f - \widehat P_{n_P}f' \right| + \left| \widehat P_{n_P} f' - Pf' \right| + \left|  P f - Pf' \right| \\
	& \le \left| \widehat P_{n_P} f' - Pf' \right| + 2\epsilon.
\end{align*}
Hence, \begin{align*}
 \Pr \left( \sup_{f \in \cF} \left|  \widehat P_{n_P} f - Pf  \right| > 3\epsilon  \right) & \le \Pr \left( \sup_{f' \in \cF'} \left|  \widehat P_{n_P} f' - Pf'  \right| + 2\epsilon > 3\epsilon  \right)\\
 & \le \sum_{f' \in \cF'} \Pr \left( \sup_{f' \in \cF'} \left|  \widehat P_{n_P} f' - Pf'  \right|  > \epsilon  \right)\\
 & \le 2 N(\epsilon ,\cF, \|\cdot\|_\infty  ) e^{-\frac{n_P\epsilon^2}{2L^2}}.
\end{align*}
Here, in the last step is obtained using the following Hoeffding's inequality: Since $ \|f\|_\infty \le L $ for any $ f \in \cF, $ we have \[ \Pr \left(  \left|  \widehat P_{n_P} f - Pf  \right|  > \epsilon  \right) \le 2e^{-\frac{n_P\epsilon^2}{2L^2}}.  \]
From Step III we get \[ \Pr \left( \sup_{f \in \cF} \left|  \widehat P_{n_P} f - Pf  \right| > t \right) \le 2 R^{d+1} \left( 1+ \frac{12\sqrt{d}}{t} \right)^{d+1} e^{-\frac{n_Pt^2}{18L^2}}. \]

\noindent \textbf{Step V:} Since, $ \delta \le \pi_P \le 1-\delta $ for some $ \delta > 0 $ independent of $ (P,Q), $ note that $  P_X \gg Q_X. $ Hence, $ P_X $ also satisfies the strong density assumption \ref{def:strong-density} with same parameter values. Then for any $ \|a\|_2 = 1, $ \begin{align*}
a^T \int_{\Omega} xx^T dP_X(x) a & \ge \mu_-\int_{\Omega\cap B(x_0, r_\mu)} (a^Tx)^2 dx ,
\end{align*} where $ x_0 $ and $ r_\mu  $ is chosen in such a way that $ B(x_0, r_\mu ) \subset \Omega.  $
Then \begin{align*}
\int_{ B(x_0, r_\mu)} (a^Tx)^2 dx & = \int_{ B(0, r_\mu)} \left[(a^Tx)^2 + 2(a^Tx)(a^Tx_0) + (a^Tx_0)^2\right] dx \\
& = \int_{ B(0, r_\mu)}x_1^2 dx + (a^Tx)^2 \lambda[B(0,r_\mu)] > c,
\end{align*} for some $ c>0. $ Hence, the minimum eigen-value of $ \Sigma = E_P(XX^T) $ is $ \ge c. $

\noindent \textbf{Step VI:} Let $ b \in B(b^*, R). $ Then \begin{align*}
f_b(x, y)  & = f_{b^*}(x, y) + (b-b^*)^T\nabla_b f_{b^*}(x,y) + (b-b^*)^T\nabla^2_b f_{b'}(x,y)(b-b^*),
\end{align*}
where  $ b' = \lambda b + (1-\lambda )b^* $ for some $ \lambda \in [0,1]. $ Here, $ b'\in B(b^*, R) $ and  $ |x^Tb'| \le \|x\|_2 \|b'\|_2 \le \sqrt d(R+\|b^*\|_2).  $ Hence, \begin{align*}
\frac{1}{1+ e^{\sqrt d(R+\|b^*\|_2)}} 	\le \frac{e^{x^Tb'}}{ 1+ e^{x^Tb'}  } \le \frac{e^{\sqrt d(R+\|b^*\|_2)}}{1+ e^{\sqrt d(R+\|b^*\|_2)}} .
\end{align*} Since, $ \frac{e^t}{\left(1+e^t \right)^2} $ is a concave function of $ \frac{e^t}{1+e^t} $ and symmetric around $ \frac12,  $ we get \[ \inf_{|x^Tb'| \le \sqrt d (R+\|b^*\|_2)} \frac{e^{x^Tb'}}{\left( 1+ e^{x^Tb'} \right)^2 } = \frac{e^{\sqrt d(R+\|b^*\|_2)}}{\left(1+ e^{\sqrt d(R+\|b^*\|_2)}\right)^2}.  \] This implies \begin{align*}
Pf_b - Pf_{b^*} &= P (b-b^*)^T\nabla_b f_{b^*}(x,y) + P(b-b^*)^T\nabla^2_b f_{b'}(x,y)(b-b^*)\\
& = P(b-b^*)^T\nabla^2_b f_{b'}(x,y)(b-b^*), \text{ since } P \nabla_b f_{b^*}(x,y) = 0,\\
& \ge \|b-b^*\|_2^2 c\frac{e^{\sqrt d(R+\|b^*\|_2)}}{\left(1+ e^{\sqrt d(R+\|b^*\|_2)}\right)^2} \triangleq c'\|b-b^*\|_2^2.
\end{align*}
\noindent \textbf{Step VII:} Let $ t >0. $ Under the event $ \sup_{\|b-b^*\|_2  \le R} \left|  \widehat P_{n_P} f_b - Pf_b  \right| \le t $ we have \[\widehat P_{n_P} f_{\hat b} \le \widehat P_{n_P} f_{ b^*}  - Pf_{b^*} + Pf_{b^*} \le t + Pf_{b^*} , \] and \[ \widehat P_{n_P} f_{\hat b} = \widehat P_{n_P} f_{\hat b} - Pf_{\hat b} + Pf_{\hat b} \ge -t + Pf_{\hat b}. \] Hence, \[ 2t \ge Pf_{\hat b} - Pf_{b^*} \ge c'\|\hat b-b^*\|_2^2. \]
Putting all together  
\begin{align*}
    &  P\left( c'\|\hat b - b^* \|_2^2 > 2t  \right)\\ \le &  \Pr \left( \sup_{f \in \cF} \left|  \widehat P_{n_P} f - Pf  \right| > t \right)\\  \le  & 2 R^{d+1} \left( 1+ \frac{12\sqrt{d}}{t} \right)^{d+1} e^{-\frac{n_Pt^2}{18L^2}}. 
\end{align*}
Hence, we have the result. 
\end{proof}


%\begin{lemma}
%	Let $ (P,Q)\in \Pi $ and let $ (X_1, Y_1), \dots , (X_n, Y_n)\sim \iid \ P . $ Consider the loss function $ \ell : \{0,1\}\times \reals^{d} \times \reals^{d+1} \to [0,\infty) $ defined as $ \ell(y, x, (w_0,  w_1^T)^T) = y(x^Tw_1 + w_0) - \log \left( 1+ e^{x^T w_1 + w_0}  \right) . $ Then for any $ R>0 $ there exists a $ K>0 $ such that for any $ t > 0 $ we have \[ \Pr \left( \sup_{\|w\|_2 \le R} \left| \frac 1n \sum_{ i =1}^n\ell(Y_i, X_i, w) -E_P\left[\ell(Y, X, w)\right]  \right| > t \right) \le 8\left( \frac{en}{d+1} \right)^{d+1} e^{-\frac{nt^2}{K^2}}. \]
%\end{lemma}

\begin{theorem}
	\label{th:upper-bound-no-label-g}
	Let $ (P,Q)\in \Pi $ and let $ (X_1^P, Y_1^P), \dots , (X_{n_P}^P, Y_{n_P}^P)\sim \iid \ P  $ and $ X_1^Q, \dots, X_{n_Q}^Q  \sim\iid \  Q_X $ For $ b = (b_0,  b_1^T)^T \in \reals \times \reals^d $ let $ h_b $ be the classifier defined as in lemma \ref{lemma:g-1} and $ b^* $ and $ \hat b $ are as in lemma \ref{lemma:g-2}. In algorithm \ref{alg:distributional-matching} let $ g = h_{\hat b}. $ Assume that there exists a $ \delta >0  $ and $ \phi>0 $ in dependent of $ (P,Q) \in \Pi $ such that  \[ \inf_{\|b-b^*\|_2 \le \delta } |\text{det}(C_P(h_b))| \ge \phi. \] Let $ K\in \cK (\alpha)$, $ h = n_P^{-\frac{1}{2\alpha+d}}, $  and $ \hat f (x) \triangleq \indicator \{\hat \eta_Q(x) \ge 1/2 \}. $        There exists a constant $ C>0 $ independent of the sample sizes $ n_P $ and $ n_Q, $ such that \[ \sup_{(P,Q)\in \Pi} \Ex_{\dataunlabeled} \left[\cE_Q \left( \hat f  \right)\right] \le C\left( n_P^{-\frac{2\alpha}{2\alpha+d}} \vee n_Q^{-1} \right)^{\frac{1+\beta}{2}}. \]
\end{theorem}
\begin{proof}
	Let $  t \ge\max\left\{ \sqrt{\frac 2 {n_P}}, \sqrt{\frac 2{n_Q}} \right\}.  $ By lemma \ref{lemma:g-2} with probability $ 1- 2R^{d+1}\left( 1+ \frac{12\sqrt{d}}{\delta^2} \right)^{d+1}e^{-cn_P\delta^4}  $ we have \[ \|\hat b - b^*\|_2 \le \delta. \] This implies with probability $ 1- 2R^{d+1}\left( 1+ \frac{12\sqrt{d}}{c'\delta^2} \right)^{d+1}e^{-c{c'}^2n_P\delta^4} $ we have \[ |\text{det}(C_P(g))| > \phi. \] Hence  using lemma \ref{lemma:g-1} with probability at least $ 1 -2R^{d+1}\left( 1+ \frac{12\sqrt{d}}{\delta^2} \right)^{d+1}e^{-cn_P\delta^4}   -16\left(\frac{2en_P}{d+1} \right)^{d+1} e^{-\frac{n_Pt^2}{8}} - 8\left(\frac{2en_Q}{d+1} \right)^{d+1} e^{-\frac{n_Qt^2}{8}} $ we have the concentration of $ \widehat w  $ as in step II of proof of theorem \ref{th:upper-bound-unlabeled}. Step III stays same. In step IV we get 
	\begin{align*}
	&	\Pr\Big( |\hat\eta_Q(x) - \eta_Q(x)| \le \eta \text{ for any } x \in \Omega \Big)\\  \ge & 1-2R^{d+1}\left( 1+ \frac{12\sqrt{d}}{\delta^2} \right)^{d+1}e^{-cn_P\delta^4}   -  16\left(\frac{en_P}{d+1} \right)^{d+1} e^{\frac{n_P\eta^2}{8}}  \\
		 & - 8\left(\frac{en_Q}{d+1} \right)^{d+1}  e^{\frac{n_Q\eta^2}{8}}  -  \exp \left(  - c_7(\alpha) \eta^2 \left(n_P^{\frac{2\alpha}{2\alpha+d}} \right)  \right) \\
		 \ge & 1 - c_8\exp \left(  - c_9(\alpha) \eta^2 \left(n_P^{\frac{2\alpha}{2\alpha+d}} \wedge n_Q \right)  \right)
	\end{align*} with $ c_9(\alpha) < \frac 12. $
	Rest of the proof follows same as in proof of Theorem \ref{th:upper-bound-unlabeled}. 
\end{proof}

==> proofs.tex <==
\section{Proof of Theorem \ref{th:lower-bound-unlabeled}}

In this section, we prove Theorem \ref{th:lower-bound-unlabeled}. The proof of Theorem \ref{th:lower-bound} is similar, and we defer the details to the supplementary materials. At a high-level, the proof has two parts. The first part shows that the minimax rate is at least $(\eps_P n_P)^{-\frac{\beta(1+\alpha)}{2\beta + d}}$. This is due to the difficulty arising from  the non-parametric part of the label shift problem: estimating the class conditional densities $g_0$ and $g_1$. The second part shows that the minimax rate is at least $n_Q^{- \frac{1+\alpha}{2}} $. This stems from  the difficulty of the parametric part of the label shift problem: estimating the class probabilities in target domain $\pi_Q$. 

\subsection{Difficulty of the non-parametric part} To study the difficulty of the non-parametric part of the label shift problem, we appeal to the following proposition  to obtain lower bounds in the non-parametric regression problems. 

\begin{proposition}[Theorem 2.5 in Tsybakov (2009) \cite{tsybakov2009Introduction}] 
\label{prop:tsybakov}
Let $ \{ \Pi_h\}_{h\in \cH} $ be a family of distributions indexed over a subset $ \cH $ of a semi-metric $ (\cF,\bar \rho). $ Suppose there are $h_0, \ldots h_M\in \cH , $ $ M\ge 2, $ such that:
\begin{enumerate}
\item $ \bar\rho (h_i , h_j) \ge 2s>0$ for all $0 \le i<j \le M, $
\item $ \Pi_{h_i} \ll \Pi_{h_0} $ for all $ i\in [M] $, and the average KL-divergence to $ \Pi_{h_0} $ satisfies \[ \frac1M \sum_{i=1}^M\KL(\Pi_{h_i}\mid\Pi_{h_0}) \le \kappa \log M\text{ for some }0<\kappa < \frac18. \]
\end{enumerate}
Let $ Z\sim \Pi_h$ and $ \hat f : Z \to \cF $ be any improper learner of $ h \in \cH. $ We have for any $ \hat f : $ \[ \sup_{h\in\cH}  \Pi_h\left( \bar\rho (\hat f (Z),h)  \ge s \right)  \ge \frac {3-2\sqrt{2}}{8}.  \]
\end{proposition}

The crux of this part  is  construction of a family of distributions on the source and target domains $\{\Pi_i\}_{i=1}^M$ that satisfies the assumptions of proposition \ref{prop:tsybakov}. Before delving into the technical details, we describe the intuition behind the construction. 

We devote most of our efforts in this part to constructing the class conditional densities because we wish to study (the difficulty of) the non-parametric part of the problem. We partition the sample space $[0,1]^d$ into small (hyper-)rectangles and divide the rectangles into three groups. The class conditional densities differ on the second and third groups, but they are identical on the first group. The sizes of the two groups are carefully adjusted to satisfy the margin condition in definition \ref{def:distribution-class} and minimize the KL divergence between the $\Pi_i$'s. Within each rectangle, the class conditional densities are smooth  functions with a rise/fall near center of the rectangle and half near the boundaries. 



% This construction has two main benefits:
% \begin{enumerate}
% \item the class conditional densities are constant on its connected components, so they trivially satisfy the smoothness conditions of definition \ref{def:distribution-class}.
% \item the regression functions are piece-wise constant, so it is easy to relate the excess risk to the number of rectangles on which the class conditional densities differ.
% \end{enumerate}
% Although the piece-wise constant regression functions are similar to the regression functions in the minimax construction of \citet{kpotufe2018Marginal}, the construction of the class conditional densities is novel. 



In the proof, we associate the rectangles with the vertices of a hypercube and judiciously pick a subset of rectangles on which the class conditional densities differ, so that the Hamming distance between the associated verticies of the hypercube is maximized. The lower bound on the minimax rate then follows directly from proposition \ref{prop:tsybakov}. 




We assume $\eps_Pn_P \ge 1. $
Let  $r = c_r (\eps_Pn_P)^{-1/(2\beta + d)}, m = \lfloor c_m r ^{\alpha\beta - d}\rfloor,$ where $\alpha\ge 0 $ is the noise condition exponent and $\beta>0 $ is the H\"older smoothness exponent.
Also, define $w = c_w r^d$ where $c_r = (1/17) ,\  c_m = 8 \times 17^{\alpha\beta - d}$ and $c_w \in (0, 1)$ is a constant to be picked later. 
The preceding constants satisfy \[ 8 \le m <\frac12 \left\lfloor \frac 1r \right\rfloor^d. \]  
To see the first inequality, we observe that $r \le 1/17$ and recall $\alpha\beta \le 1 \le  d.$ 
Thus \[ m = 8 \times (17r)^{\alpha\beta - d} \ge 8. \] 
To see the second inequality, we observe that $r^{-1} \ge 16,$ which implies $r^{-1}\le 17\lfloor r^{-1}\rfloor/16.$ 
Thus \[ m = 8 (17r)^{\alpha\beta} \left(\frac 1{17r}\right)^d \le 8\cdot  16^{-d} \lfloor r^{-1} \rfloor ^d \le\frac1 2 \lfloor r^{-1} \rfloor ^d. \] We also have $2mw = 2mc_w r^d\le 2c_m c_w<1 $ for a suitable $c_w.$
    
    \textit{Construction of $\{\Pi_i\}_{i=1}^M$.}
    Let $r_1 = 1/\lfloor 1/r\rfloor.$ Let us consider the grid of points \begin{equation}
        \cZ = \{ (1/2+i)r_1 : i = 0, 1, \dots , \lfloor 1/r\rfloor -1 \}^d.
    \end{equation} 
    We see that $\cZ$ is a grid of equally spaced points of size $\lfloor 1/r \rfloor^d.$ For a $z \in \cZ$ we consider the hyper-cube \[ C(z) = \{x \in [0,1]^d: \|x-z\|_\infty\le r_1/2 \}. \] Note that, volume of each of these hyper-cubes is $r_1^d.$ Let $\cZ_1, \cZ_2 \subset \cZ $ be subsets of size $m$. Moreover, we let $\cZ_1 $ and $\cZ_2$ are disjoint. We define a bijection $u : \cZ_1 \to \cZ_2 $ which shall be used to construct the conditional densities. We define $\cZ_0 = \cZ \backslash (\cZ_1 \cup \cZ_2).$ On this grid, we define a set of distributions parametrized by $\sigma\in \{ -1, 1 \}^{\cZ_1}.$ 
    % Let $C_\beta' =  (C_\beta6^{\beta}) \wedge (1/3).$ 
    % Then \[C_\beta'r_1^\beta \le 1/3r_1^\beta \le 1/3. \]
    
    
    
    
    

    
    \noindent\textit{Conditional densities.}  For $\beta >0$ we define a function $u_\beta$ supported on on $[0, \infty)$ which will be used heavily for the construction of conditional densities. 
    
    \begin{equation}
    \label{eq:u-function}
    u_{\beta}(x)=     \begin{cases}   \begin{cases} 
    \big( 1-x \big)^{\beta} & \text{if}\  x \le 1\\
    0 & \text{otherwise,}
    \end{cases} & \quad \text{for }\beta < 1,\\
    \begin{cases} 
    \big( 2^{1-\beta}-x^\beta \big) & \text{if}\  x \le 1/2\\
    \big( 1 -x \big)^\beta & \text{if}\  1/2 < x \le 1\\
    0 & \text{otherwise,}
    \end{cases} & \quad \text{for }\beta \le 1.
        \end{cases}
    \end{equation}
    
    
    
    It can be shown that $u$ is $\beta$-smooth with constant $L$ for some $L>0$.  Let  $C_\beta' = (C_\beta L^{-1})\wedge (1/3).$
    Therefore, the following functions are $(C_\beta, \beta)$-H\"older: 
    \[ z \in \cZ_1, \hspace{0.3cm} \eta_z(x) = C_\beta' r_1^\beta u_\beta \left(\frac{2\|x-z\|_2 }{c_wr_1}\right). \]
    
    For a parameter $\sigma$ the  construction of  conditional densities are given below. 
    
    
    \begin{gather}
        \left\{    
        \begin{aligned}
         g_1^{\sigma}(x) & = \begin{cases}
    1+  \sigma(z) \sqrt{\eps_P} \eta_z(x) & \hspace{0.3cm} x \in C(z),\ z \in \cZ_1,\\
    1-  \sigma(z) \sqrt{\eps_P} \eta_{f(z)}(x) & \hspace{0.3cm} x \in C(f(z)),\  z \in \cZ_1,\\
    1 & \hspace{0.3cm} x \in C(z),\  z \in \cZ_0,
    \end{cases} \\
    g_0^{\sigma}(x)&  = \begin{cases}
     1-  \sigma(z) \sqrt{\eps_P}  \eta_z(x) & \hspace{0.3cm} x \in C(z),\ z \in \cZ_1,\\
    1+  \sigma(z) \sqrt{\eps_P}  \eta_{f(z)}(x) & \hspace{0.3cm} x \in C(f(z)),\  z \in \cZ_1,\\
    1 & \hspace{0.3cm} x \in C(z),\  z \in \cZ_0.\end{cases}
        \end{aligned}
        \right.
        \label{eq:density-class-unsupervised-density}
    \end{gather}
    
    % \begin{equation}
    % \label{eq:density-class-1}
    %     g_1^{\sigma}(x) = \begin{cases}
    % 1+  \sigma(z) \sqrt{\eps_P} \eta_z(x) & \hspace{0.3cm} x \in C(z),\ z \in \cZ_1,\\
    % 1-  \sigma(z) \sqrt{\eps_P} \eta_{f(z)}(x) & \hspace{0.3cm} x \in C(f(z)),\  z \in \cZ_1,\\
    % 1 & \hspace{0.3cm} x \in C(z),\  z \in \cZ_0.
    % \end{cases} 
    % \end{equation}
    
    
    % \begin{equation}
    % \label{eq:density-class-1}
    %     g_1^{\sigma}(x) = \begin{cases}
    %  c_w\big(1+  \sigma(z) \sqrt{\eps_P} \eta_z(x)\big) & \hspace{0.3cm} x \in C(z),\ z \in \cZ_1,\\
    % c_w\big(1-  \sigma(z) \sqrt{\eps_P} \eta_{f(z)}(x)\big) & \hspace{0.3cm} x \in C(f(z)),\  z \in \cZ_1,\\
    % c_w + v(\|x-z\|_2/r_1) & \hspace{0.3cm} x \in C(z),\  z \in \cZ_0.
    % \end{cases} 
    % \end{equation}
    
    %  \begin{equation}
    %     g_0^{\sigma}(x) = \begin{cases}
    % q_1 (1- \frac12\sigma(z) C_\beta' r^\beta) & \hspace{0.3cm} x \in B(z, r/6), z \in \cZ_1,\\
    % q_1 (1+\frac12 \sigma(z)  C_\beta' r^\beta) & \hspace{0.3cm} x \in B(f(z), r/6), z \in \cZ_1,\\
    % q_0 & \hspace{0.3cm} x \in B(z, r/6), z \in \cZ_0.
    % \end{cases} 
    % \end{equation}
    
    
    % \begin{equation}
    % \label{eq:density-class-0}
    %     g_0^{\sigma}(x) = \begin{cases}
    %  1-  \sigma(z)  \eta_z(x) & \hspace{0.3cm} x \in C(z),\ z \in \cZ_1,\\
    % 1+  \sigma(z)  \eta_{f(z)}(x) & \hspace{0.3cm} x \in C(f(z)),\  z \in \cZ_1,\\
    % 1 & \hspace{0.3cm} x \in C(z),\  z \in \cZ_0.
    % \end{cases} 
    % \end{equation}
    
    % \begin{equation}
    % \label{eq:density-class-0}
    %     g_0^{\sigma}(x) = \begin{cases}
    %  c_w\big(1-  \sigma(z)  \eta_z(x)\big) & \hspace{0.3cm} x \in C(z),\ z \in \cZ_1,\\
    % c_w\big(1+  \sigma(z)  \eta_{f(z)}(x)\big) & \hspace{0.3cm} x \in C(f(z)),\  z \in \cZ_1,\\
    % c_w + v(\|x-z\|_2/r_1) & \hspace{0.3cm} x \in C(z),\  z \in \cZ_0.
    % \end{cases} 
    % \end{equation}
    
    
    
    
    We also define $\pi_Q^{\sigma} = 1/2$ and $\pi_P^\sigma = 1/2.$ We then define the probabilities \[P_{\sigma}(X \in A, Y= y) = \int_A [\pi_P^{\sigma} g^{\sigma}_1(x)\indicator(y = 1) + (1-\pi_P^{\sigma}) g^{\sigma}_0(x) \indicator (y = 0) ] dx\] and
    \begin{equation}
        Q_{\sigma}( X \in A, Y = y) = \int_A [\pi_Q^
    {\sigma}g^{\sigma}_1(x)\indicator(y = 1) + (1-\pi^{\sigma}_Q) g^{\sigma}_0(x) \indicator (y = 0) ] dx.
    \label{eq:dist-Q-unlabeled-density}
    \end{equation}
    Given the source and target distributions we define the joint distribution of $\dataunlabeled$ as \begin{equation}
        \label{eq:dist-unlabeled-joint-density}
        \Pi_\sigma = P_\sigma^{\otimes n_P} \otimes Q_{\sigma, X} ^{\otimes n_Q}
    \end{equation}
    
    Here, $\eps_P \le \pi_P^\sigma \le 1-\eps_P.$ Also, $\mu_- \le g_1^\sigma(x), g_0^\sigma(x)   \le \mu'\le \mu_+ $ for any $x \in \Omega.$ Hence, $\mu_- \le q^{\sigma}_X(x) \le  \mu _+ .$ Furthermore, $\Omega = [0,1]^d$ is a regular set. Hence, $q^\sigma _X$ satisfies strong density assumption. 
    
    
    For such a construction, the marginals are \begin{equation}
        \label{eq:marginals-unlabeled-density}
        p_X^\sigma(x) = q_X^\sigma(x) = \frac 12 g_1^\sigma(x)+ \frac 12 g_0^\sigma(x) = 1
    \end{equation}
    
    Furthermore, the regression function $\eta_Q^\sigma$ is \begin{equation}
        \label{eq:reg-fn-unlabeled-density}
        \eta_Q^\sigma(x) = \frac{\pi_Q^\sigma g_1^\sigma(x)}{q_X^\sigma(x)} = \frac 12 g_1^\sigma(x)
    \end{equation}
   
    
   We refer to lemma \ref{lemma:margin-unlabeled-density}, where it is shown $Q_\sigma$ satisfies $\alpha$-margin condition with constant $C_\alpha.$
   
        
  
        
        
      
        
        
    Let $ \cF $ be the set of all classifier relevant to this classification problem. For $\sigma \in \{-1, 1\}^{\cZ_1}$ let  $f_\sigma$ be the Bayes classifier corresponding to the probability distribution $Q_\sigma$ defined as $ f_\sigma (x) = \indicator\{\eta_{ Q_\sigma }(x) \ge 1/2\}.$  For $ \sigma,\sigma'\in\{-1, 1\}^{\cZ_1} $ define $ \bar\rho (\sigma,\sigma') \coloneqq \cE_{\sigma} (f_{\sigma'})   $ and  $\rho(\sigma,\sigma') = \text{card} \{z\in\cZ_1 :\sigma(z) \neq \sigma'(z) \} $ as the Hamming distance. Then \begin{align*}
        \bar\rho (\sigma,\sigma') & = 2\Ex _{Q_{\sigma, X}} \left[\left | \eta_Q^\sigma(X) - \frac12 \right | \mathbf{1}\left( f_\sigma(X) \neq f_{\sigma'}(X)  \right)\right]\\
         & \ge c   r_1^d r_1^\beta  \rho(\sigma, \sigma').
    \end{align*}
	
We recall Varshamov-Gilbert bound, which shall be used to construct the probability class. 	
	\begin{lemma}[Varshamov-Gilbert bound]
	\label{lemma:varshamov-gilbert}
	Let $ m\ge 8. $ Then there exists a subset $ \{ \sigma_0,\ldots , \sigma_M \} \subset \{-1,1\}^m $ such that $ \sigma_0 = (1 ,\ldots, 1), $ \[ \rho_H(\sigma_i , \sigma_j ) \ge \frac m 8, \ \text{for all } 0\le i<j\le M,\ \text{and } M \ge 2^{m/8}, \] where, $ \rho_H $ is the hamming distance. 
\end{lemma}



	Let $\{ \sigma_0,\ldots , \sigma_M \} \subset \{-1,1\}^m  $ be the choice obtained from the  lemma \ref{lemma:varshamov-gilbert}.  Note that for such a choice $\rho(\sigma_i, \sigma_j) \ge m/8$ whenever $i\neq j.$
	
	Then  \begin{align*}
	\bar\rho (\sigma_i, \sigma_j) &\ge c  r_1^{\beta+d}  \frac m8\\ 
	&\ge c'  r_1^{\beta+d}   r_1^{\alpha\beta -d}  \\
	& \ge c' r_1^{\beta (1+\alpha)}\\
	& = c' (\eps_P n_P)^{-\frac{\beta(1+\alpha)}{2\beta + d}}\\
	& \triangleq 2s
	\end{align*}

	
	
	
	Now we bound the Kulback-Leibler divergence between the joint distributions $\Pi_{\sigma_i}.$ Using lemma \ref{lemma:kl-unlabeled-density} we get 
	\begin{align*}
	KL(\Pi_{\sigma_i}|| \Pi_{\sigma_j}) & \le c_w^dK(d, \alpha, \beta)\rho(\sigma_i, \sigma_j) \\
	& \le  c_w^dK(d, \alpha, \beta)m \\
	& \le \frac 19 \log_2(M) \\
	\end{align*}
	for suitable $c_w < 1.$
	

	
	
	
	
	Finally we appeal to proposition \ref{prop:tsybakov} (and Markov's inequality) to obtain the minimax rate \begin{align*}
\sup_{(P,Q)\in \Pi} \Ex \cE_Q (\hat f)& \ge \sup_{(P,Q)\in \Pi} s \Pr_\Pi \left ( \cE_Q (\hat f)\ge s \right)\\
& \ge s \sup_{\sigma\in \{-1,1\}^{\cZ_1}} \Pi_\sigma \left(\cE_{Q^\sigma} (\hat f)\ge s \right) \\
& \ge s \frac {3-2\sqrt{2}}{8}\\
& \ge C(\eps_Pn_P)^{-\frac{\beta(1+\alpha)}{2\beta + d}}.
\end{align*}


\subsection{Difficulty of the parametric part} To study the difficulty of the parametric part, it is enough to construct two well-separated hypotheses (versus the family of well-separated hypotheses required in our study of the non-parametric part). We refer to the following theorem to establish  lower bound.


\textcolor{blue}{There is some mistake in the bound}
\begin{theorem}[LeCam's bound]
\label{th:lb-lecam}

Let $\cP$ be a set of distributions. For any pair $P_0, P_1 \in \cP,$
\[ \inf_{\hat \theta }\sup_{P\in \cP} \Ex_P \big[ d(\hat \theta, \theta(P) ) \big] \ge \frac \Delta 8 e^{-KL(P_0||P_1)} \] where $\Delta = d\big(\theta(P_0), \theta (P_1)\big).$

\end{theorem}

The construction will closely follow the non-parametric part. Let $\sigma \in \{-1, 1\},\ c_w<1,\ r = n_Q^{-1/2}/8,  \ C_\beta' = C_\beta .$ For $z \in \{1/3, 2/3\}$ we set \[ \eta_z(x) = C_\beta' r^\beta u_\beta \left( \frac{2|x_1- z|}{c_wr} \right) \]

\begin{gather}
\label{eq:conditional-parametric}
  \left\{  \begin{aligned}
    g_1^\sigma(x) & = \begin{cases}
     1+    \eta_{1/3}(x) & \quad |x_1-1/3|\le c_wr/2, \\
    1-   \eta_{2/3}(x) & \quad |x_1-2/3|\le c_wr/2,\\
    1 & \quad \text{otherwise,}
    \end{cases} \\
    g_0^\sigma(x) &= \begin{cases}
     1-    \eta_{1/3}(x) & \quad |x_1-1/3|\le c_wr/2, \\
    1+   \eta_{2/3}(x) & \quad |x_1-2/3|\le c_wr/2,\\
    1 & \quad \text{otherwise,}
    \end{cases} 
    \end{aligned}\right.
\end{gather} and  $\pi_P^\sigma = 1/2,\ \pi_Q^\sigma = 1/2 + \sigma r/8.$ We construct $P_\sigma, Q_\sigma$ and define 
\begin{equation}
\label{eq:dist-labeled-joint-parametric}
    \Pi_\sigma = P_{X,\sigma} ^{\otimes n_P} \otimes Q_\sigma ^{\otimes n_Q}
\end{equation}
 in the similar way. As before, we have $\eps_P \le \pi_P^\sigma \le 1-\eps_P,\ \mu_- \le g_1^\sigma (x), g_0^\sigma (x) \le \mu_+.$ Hence, $\mu_-\le q_X\le \mu_+$ and supported on $[0, 1]^d.$ This implies $Q_X$ has strong density. Also, we refer to lemma C.9 in supplement to show $Q_\sigma$ satisfies $\alpha$ margin condition with constant $C_\alpha.$


For $\sigma \in \{-1, 1\}$ let $\eta_\sigma$ and $f_\sigma$ be the regression function and Bayes classifier for $Q_\sigma,$ respectively. Then \[
\begin{aligned}
\bar \rho (\Pi_{1}, \Pi_{-1}) &= \cE_{Q_1} (f_{-1}) \\ &= 2 \Ex_{Q_{1, X}} \Big[ \big|\eta_Q^\sigma(X)-1/2\big| \indicator\{ f_1(X) \neq f_{-1}(X) \}  \Big]\\
& \ge c r\\
& \ge c r^{1+\alpha}\\
& \ge c' n_Q^{-\frac{1+\alpha}{2}} = 2s.
\end{aligned}
\]

We refer to lemma C.10 in supplement  to get the following bound \[ KL(\Pi_1||\Pi_{-1}) \le \frac3 {16}. \]
Using theorem \ref{th:lb-lecam}   we conclude 
\[
    \sup_{(P, Q) \in \Pi} \Ex \big[ \cE_Q(\hat f) \big] \ge c n_Q^{-\frac{1+\alpha}{2}}.
\]

Finally, we combine the two bounds to get \[ 
\begin{aligned}
\sup_{(P, Q) \in \Pi} \Ex \big[ \cE_Q(\hat f) \big] & \ge c n_Q^{-\frac{1+\alpha}{2}} \vee c(\eps_Pn_P )^{-\frac{\beta(1+\alpha)}{2\beta + d}}\\
& \ge c' \Bigg( (\eps_Pn_P)^{-\frac{\beta}{2\beta + d}} + n_Q^{-1/2}  \Bigg)^{1+\alpha} .
\end{aligned}
\]





















% % Before delving into the details of $\{\Pi_{h_i}\}_{i=1}^M$, we give an overview of the design choices. Following the construction in \cite{kpotufe2018Marginal}, we start by constructing a larger family and picking out a well-separated subset of this larger family to obtain $\{\Pi_{h_i}\}_{i=1}^M$.

% Define $d_0\triangleq 2+\frac{d}{\alpha}$, where $d$ is the problem dimension and $\alpha\in(0,1]$ is the H\"{o}lder-smoothness exponent. Let $r \triangleq c_r n_P^{-\frac1{\alpha d_0}}$, $m \triangleq \lfloor c_m r^{\alpha\beta -d} \rfloor$, where $\beta > 0$ is the noise condition exponent, and $w \triangleq c_w r^d$, where $ c_r \triangleq \frac19$, $c_m \triangleq 8\cdot 9^{\alpha\beta - d}$ and $c_w\in(0,1]$ is a constant to be picked later. The preceding constants satisfy 
% \[\textstyle
% 8\le m < \lfloor \frac1r\rfloor ^d.
% \]
% To see the first inequality, we observe that $r \le \frac19$ and recall $\alpha\beta - d \le 0$. Thus
% \[
% m = 8(9r)^{\alpha\beta - d} \ge 8.
% \]
% To see the second inequality, we observe that $\frac1r \ge 9 > 8$, which implies $\frac1r \le \frac98\lfloor\frac1r\rfloor$. Thus
% \[\textstyle
% m = 8 (9r)^{\alpha\beta}(\frac{1}{9r})^d \le 8^{1-d } \lfloor \frac1r\rfloor ^d  \le \lfloor \frac1r\rfloor ^d.
% \]
% We also have $ mw = mc_w r^d <1. $

% \paragraph{Construction of $\{\Pi_{h_i}\}_{i=1}^M$} Let $\cZ$ be a grid of equally space points in the feature space $[0,1]^d$. The points are spaced $r$ apart, so there are $\lfloor\frac1r\rfloor^d$ points in the grid. Let $\cZ_1\subset\cZ$ be a subset of size $m$ and $\cX_1\triangleq\cup_{z\in\cZ_1}B(z,\frac{r}{6})$. Let $\cZ_0 \triangleq \cZ\setminus\cZ_1$ and $\cX_0 \triangleq\cup_{z\in\cZ_0}B(z,\frac{r}{2})$. On this grid, we define a set of distributions parametrized by  $\sigma\in \{-1,1\}^{\cZ_1}$. 
% Let $ C_\alpha' = \min \left\{ C_\alpha 6^{-\alpha}, \frac12, 1-2\epsilon  \right\}.$
% % Let $C_\alpha'r^\alpha = C_\alpha' r^\alpha u ( \frac{\|x-z\|_2}{r})$, where $ C_\alpha' = \min \left\{ C_\alpha 6^{-\alpha}, \frac12, 1-2\epsilon  \right\}$ and 
% % \[ u(x) = \begin{cases}
% % 1 & \text{if } x \le \frac16,\\
% % 1 - 6\left(x -\frac16  \right) & \text{if } \frac16 < x \le \frac13,\\
% % 0 & \text{if } x> \frac13.

% % \end{cases} \]
% Define
% \[ g_1^\sigma (x) = \begin{cases}
% a^\sigma q_1 \left(1+\sigma(z)C_\alpha'r^\alpha\right) & x \in B\left(z,\frac r6  \right), \ z \in \cZ_1,\\
% a^\sigma q_0 & x \in B\left(z,\frac r2  \right), \ z \in \cZ_0,\\
% 0 & \text{otherwise},
% \end{cases} \] and, \[ g_0^\sigma (x) = \begin{cases}
% b^\sigma q_1 \left(1-\sigma(z)C_\alpha'r^\alpha\right) & x \in B\left(z,\frac r6  \right), \ z \in \cZ_1,\\
% b^\sigma q_0 & x \in B\left(z,\frac r2  \right), \ z \in \cZ_0,\\
% 0 & \text{otherwise},
% \end{cases} \] 
% where the constants
% \[
% \begin{aligned}
% a^\sigma \triangleq \frac1 {1+ w\sum_{z\in\cZ_1} \sigma(z)C_\alpha'r^\alpha}, \quad b^\sigma \triangleq \frac1 {1- w\sum_{z\in\cZ_1} \sigma(z)C_\alpha'r^\alpha}, \\
% q_0 \triangleq \frac{1-mw}{\text{Vol}\left(\cX_0\right)},\quad q_1 \triangleq \frac w{\text{Vol}\left( B\left(z,\frac r6\right)  \right)}
% \end{aligned} 
% \]
% are chosen so that $g_1^\sigma$ and $g_0^\sigma$ are probability densities. In particular, we pick $\pi_Q^\sigma$ so that $\frac{a^\sigma q_0 \pi_Q ^\sigma}{b^\sigma q_0 (1-\pi_Q ^\sigma)} = 1$. This implies $\pi_Q ^\sigma = \frac{1/a^\sigma}{1/a^\sigma + 1/b^\sigma} = \frac 12 \left( 1+ w  \sum_{z\in\cZ_1} \sigma(z) \right)$. Finally, we pick $\pi_P^\sigma \triangleq \pi_Q^\sigma$. We define $P^\sigma$ and $Q^\sigma$ as 
% \[
% \begin{aligned}
% p^\sigma(x,y) = \pi_P^\sigma g_1^\sigma(x)\ones\{y=1\} + (1-\pi_P^\sigma) g_0^\sigma(x)\ones\{y=0\}, \\
% q^\sigma(x,y) = \pi_Q^\sigma g_1^\sigma(x)\ones\{y=1\} + (1-\pi_Q^\sigma) g_0^\sigma(x)\ones\{y=0\}.
% \end{aligned}
% \]
% The choices of $g_1^\sigma$, $g_0^\sigma$, and $\pi_Q$ imply
% \[ \frac{1-\pi_Q^\sigma}{\pi_Q^\sigma} \frac{g_0^\sigma(x)}{g_1^\sigma(x)} = \begin{cases}
% \frac{1- \sigma(z)C_\alpha'r^\alpha}{1+ \sigma(z)C_\alpha'r^\alpha} & x\in B\left( z,\frac r6 \right),\ z\in\cZ_1,\\
% 1 & x\in \cX_0.
% \end{cases} \] 
% Thus
% \[
% \eta_Q^\sigma(x) = \begin{cases}
% \frac12(1+ \sigma(z)C_\alpha'r^\alpha) = \frac12(1+ \sigma(z)C_\alpha'r^\alpha) & x\in B\left( z,\frac r6 \right),\ z\in\cZ_1,\\
% \frac12 & x\in \cX_0.
% \end{cases} 
% \]
% Finally, we extend $\eta_Q$ to the rest of $\cX$:\[ \eta_Q^\sigma(x) = \begin{cases}
% \frac12(1+ \sigma(z)C_\alpha'r^\alpha) & x\in \cX_1\\
% \frac12 & \text{otherwise.}
% \end{cases}\] 
% We note that the marginal density of the features in the target domain $Q_X$ does not depend on $\sigma$:\[q_X^\sigma = \pi_Q^\sigma g_1^\sigma + (1-\pi_Q^\sigma) g_0^\sigma= \begin{cases}
% q_1 & x\in \cX_1,\\
% q_0 & x \in \cX_0.
% \end{cases}\] 
% Indeed, for $ x\in\cX_1, $ \begin{align*}
% q_X^\sigma(x) & = \pi_Q^\sigma g_1^\sigma(x) + (1-\pi_Q^\sigma) g_0^\sigma(x)\\
% & = a^\sigma q_1 \left(1+\sigma(z)C_\alpha'r^\alpha \right) \frac1{2a^\sigma}  + b^\sigma q_1 \left(1-\sigma(z)C_\alpha'r^\alpha \right) \frac1{2b^\sigma}\\
% & = q_1.
% \end{align*}
% Similarly, for $ x\in\cX_0, $ \begin{align*}
% q_X^\sigma(x) & = \pi_Q^\sigma g_1^\sigma(x) + (1-\pi_Q^\sigma) g_0^\sigma(x)\\
% & = a^\sigma q_0  \frac1{2a^\sigma}  + b^\sigma q_0  \frac1{2b^\sigma}\\
% & = q_0.
% \end{align*}
% Thus it is impossible to learn $\sigma$ from unlabeled observations $X \sim Q^\sigma$. This simplifies the derivation of the minimax rate from proposition \ref{prop:tsybakov}.

% Before appealing to proposition \ref{prop:tsybakov}, we check that the preceding choices satisfy our assumptions on the unsupervised label shift problem (see definition \ref{def:distribution-class}). 

% \paragraph{Checking $ \epsilon \le \pi_P^\sigma \le 1- \epsilon  $:} We have
% \begin{align*}
% \left| w  \sum_{z\in\cZ_1} \sigma(z) C_\alpha' r^\alpha  \right|  & \le  w  \sum_{z\in\cZ_1}  C_\alpha' r^\alpha\\& \le mw C_\alpha' r^\alpha \\
% & \le C_\alpha'r^{\alpha} \le 1-2\epsilon.
% \end{align*} 
% Thus
% \[
% \textstyle
% \pi_P^\sigma = \frac 12 \left( 1+ w  \sum_{z\in\cZ_1} \sigma(z) C_\alpha' r^\alpha \right) \left\{\begin{aligned}\textstyle\ge \frac12 (1 - (1-2\epsilon)) = \epsilon \\\textstyle
% \le \frac12 (1 + (1-2\epsilon)) = 1- \epsilon
% \end{aligned}\right.
% \]

% \paragraph{Checking local $ \alpha $-H\"older smoothness of $ g_0^\sigma $ and $ g_1^\sigma $:} $g_1^\sigma$ and $g_0^\sigma$ are piece-wise constant on their support, so they are trivially locally $ \alpha $-H\"older smooth on their support.

% % We are interested in the local smoothness of $ g_0^\sigma $ and $ g_1^\sigma $ (see definition \ref{def:holder-smooth}), so we only consider the variation of $g_1^\sigma$ and $g_0^\sigma$ in balls of radii $ \frac r6. $

% % As we shall see, for any $ x, x' \in \Omega $ with $ \|x-x'\| \le \frac r6 $ \[ \frac{|g_1^\sigma(x)-g_1^\sigma(x')|}{\|x-x'\|^\alpha} \le C_\alpha. \] 
% % We check this claim case-by-case:
% % \begin{enumerate}
% % \item $g_1^\sigma$ and $g_0^\sigma$ are constant in $ x, x' \in B(z, r/2) $ for some $ z \in \cZ_0. $ 

% % In that case, \[ |g_1(x) - g_1(x')| = |a^\sigma q_0 - a^\sigma q_0| = 0 \] and the inequality  holds trivially. 
% % \item $ x, x' \in B(z, r/6) $ for some $ z \in \cZ_1. $ In that case,  \[ |g_1(x) - g_1(x')| = |a^\sigma q_1 (1+ \sigma(z) C_\alpha' r^\alpha ) - a^\sigma q_1(1+ \sigma(z) C_\alpha' r^\alpha )| = 0 \] and the inequality  holds trivially again.
% % \item $ x \in B(z, r/2) $ and $ x' \in B(z', r/2) $ for some $ z, z' \in \cZ. $ In that case  \[ \|x-x'\| \ge \|z-z'\| - \|x-z\|-\|x'-z'\| \ge r > \frac r 6. \] So, this an invalid case.
% % \end{enumerate}


% \paragraph{Checking the margin condition (definition \ref{def:margin-condition})} For $ t < C_\alpha' r^\alpha/2$, 
% \[\textstyle
% Q_X^\sigma \left( 0< \left| \eta_Q^\sigma(X) -\frac12 \right| \le t \right) =0.
% \]
% For $ t\ge C_\alpha' r^\alpha/2, $ \begin{align*}
% Q_X \left( 0< \left| \eta_Q(X) -\frac12 \right| \le t \right) &  = mw\\
% & \le c_mc_w r^{\alpha \beta}\\
% & \le C_\beta \left( \frac{C_\alpha' r^\alpha}{2}  \right)^\beta.
% \end{align*}

% We return to the task of constructing a well-separated family of distributions. 
% Let $\{ \sigma_0,\ldots , \sigma_M \} \subset \{-1,1\}^{\cZ_1}  $ be a large subset that is well-separated in Hamming distance. More precisely, $M \ge 2^{\frac{m}{8}}$ and $\rho_H(\sigma_i,\sigma_j) \ge \frac{m}{8}$ for any $i,j\in[m]$ (see lemma \ref{lemma:varshamov-gilbert}). 
% To each $\sigma_i$ in this well-separated subset, we associate the pair of distributions $(P^{\sigma_i},Q^{\sigma_i})$. In the unsupservised label shift problem, a dataset consists of $n_P$ labeled observations from the source domain and $n_Q$ unlabeled observations from the target domain, so the distribution of a dataset is $ \Pi_i = {P^{\sigma_i}}^{\otimes n_p} \otimes {Q_X}^{\otimes n_Q} .$ This is our well-separated family of distributions.
% % Note that the distribution $ Q_X $ doesn't depend on $ i. $

% Let $ \cF $ be the hypothesis class (the set of all measurable $f:[0,1]^d\to\{0,1\}$). For any $ h,h'\in\cF $, define the semi-metric 
% \[
% \bar\rho (h,h') \triangleq C_\alpha' r^\alpha Q_X \left( \{h(X)\neq h'(X)\} \cap \cX_1 \right). 
% \]
% This definition is motivated by 
% \begin{align*}
% \cE_{Q^\sigma}(h) & = 2\Ex _{Q_X} \left[\left | \eta_Q^\sigma(X) - \frac12 \right | \mathbf{1}\left( h(X) \neq h^*_\sigma(X)  \right)\right]\\
% & = C_\alpha' r^\alpha Q_X\left( \{h(X) \ne h_\sigma^*(X)  \} \cap \cX_1 \right).
% \end{align*}
% For any $ \sigma\in\{-1,1\}^{\cZ_1}, $ let $ h_\sigma^* $ be the Bayes classifier: $h_\sigma^* (x) \triangleq \mathbf{1}\{\eta_Q^\sigma(x) \ge 1/2\}$. For $ \sigma, \sigma'\in\{-1,1\}^m $ we see that $ \bar\rho (h_\sigma^*, h_{\sigma'}^*) = C_\alpha' r^\alpha w \rho_H(\sigma, \sigma'), $ where, $ \rho_H(\sigma,\sigma') $ is the Hamming distance.
% % defined as $ \rho_H(\sigma,\sigma') \coloneqq \text{card} \{z\in\cZ_1 :\sigma(z) \neq \sigma'(z) \}. $





% % Let $\{ \sigma_0,\ldots , \sigma_M \} \subset \{-1,1\}^m  $ be the choice obtained from the  lemma \ref{lemma:varshamov-gilbert}. For each $ i \in \{0,\ldots,M\} $ let us set the distributions of two populations to be $ (P^i, Q^i) = (P^{\sigma_i}, Q^{\sigma_i}). $ For the distribution pair $(P^i,Q^i) $ joint distribution of the dataset $\left\{  \{(X_i^P,Y_i^P)\}_{1\le i\le n_P} , \{X_i^Q\}_{1\le i\le n_Q} \right\} $ $ (\bX,\bY) $ is $ \Pi_i = {P^i}^{\otimes n_p} \otimes {Q_X}^{\otimes n_Q} .$ Note that the distribution $ Q_X $ doesn't depend on $ i. $

% To keep notation manageable, we drop one level of subscripts and write $ h_{\sigma_i}^* $ as $ h_i^* .$ For any $h_i,h_j$ in the well-separated family of distributions, 
% \begin{align*}
% \bar\rho (h_i^*,h_j^*) &\ge C_\alpha' \frac{wmr^\alpha }{8}\\ 
% &\ge \frac12 C_\alpha' c_r^\alpha n_P^{-\frac1{d_0}} c_mr^{\alpha\beta -d} c_w r^d \\
% & \ge C n_P^{-\left(\frac{1}{d_0} +\frac{\alpha\beta}{\alpha d_0} \right)}\\
% & = C n_p^{-\frac{1+\beta}{d_0}}\\
% & \triangleq 2s.
% \end{align*}
% Let $ \KL(P\mid Q) $ be the KL-Divergence between the distributions $ P $ and $ Q. $ Then 
% \[
% \begin{aligned}
% \KL(\Pi_i\mid\Pi_0) &= n_P \KL(P^i\mid P^0) + n_Q \KL(Q_X\mid Q_X) \\
% &= n_P \KL(P^i\mid P^0) = n_P \KL(Q^i\mid Q^0),
% \end{aligned}
% \]
% where we recalled $Q_X$ does not depend on $\sigma$ in the second step and $\pi_P^\sigma = \pi_Q^\sigma$ in the third step. We simplify $\KL(Q^i\mid Q^0)$ to obtain
% \begin{align*}
% \KL(Q^i\mid Q^0)  =&  \int \log\left( \frac{dQ^i}{dQ^0}  \right) dQ^i\\
% =& \int \left[ \log \left( \frac{\eta_Q^i (x)}{\eta_Q^0(x)}  \right) \eta_Q^i(x) + \log \left( \frac{1-\eta_Q^i (x)}{1-\eta_Q^0(x)}  \right) (1-\eta_Q^i(x))  \right] dQ_X\\
% =& \sum_{z: \sigma_i(z) \neq \sigma_0(z)} Q_X \left(B\left( z,\frac r6  \right)  \right) \Bigg[ \log \left( \frac{1+ C_\alpha'r^\alpha}{1- C_\alpha'r^\alpha}  \right) \frac{1+ C_\alpha'r^\alpha}{2}\\
% & +  \log\left( \frac{1- C_\alpha'r^\alpha}{1+ C_\alpha'r^\alpha}  \right) \frac{1- C_\alpha'r^\alpha}{2} \Bigg] \\
% =& w \rho_H(\sigma_i , \sigma_0) \log \left( \frac{1+ C_\alpha'r^\alpha}{1- C_\alpha'r^\alpha}  \right) C_\alpha'r^\alpha\\
% \le & 2mw\frac{C_\alpha'^2 r^{2\alpha}}{1-C_\alpha'r^\alpha}\\
% \le & 4mw C_\alpha'^2 r^{2\alpha}.
% \end{align*}  
% Thus, for $ c_w $ small enough, we have
% \begin{align*}
% \KL(\Pi_i\mid \Pi_0) &\le  4mw C_\alpha'^2 r^{2\alpha} n_P\\
% &= 4m c_w r^d C_\alpha'^2 r^{2\alpha} n_P\\
% & = 4m c_w C_\alpha'^2 r^{2\alpha+d} n_P\\
% & = 4m c_w C_\alpha'^2 c_r^{2\alpha+d} n_P^{-\frac{2\alpha +d}{\alpha d_0}} n_P\\
% & = 4m c_w C_\alpha'^2 c_r^{2\alpha+d} \text{ since } \alpha d_0 = 2\alpha + d\\
% & = 2^5 (\log 2)^{-1} c_w C_\alpha'^2 c_r^{2\alpha+d} \log (M)\\
% &\le \frac 18\log (M),  
% \end{align*}
% Finally, we appeal to proposition \ref{prop:tsybakov} (and Markov's inequality) to obtain the minimax rate \begin{align*}
% \sup_{(P,Q)\in \Pi} \Ex \cE_Q (\hat f)& \ge \sup_{(P,Q)\in \Pi} s \Pr_\Pi \left ( \cE_Q (\hat f)\ge s \right)\\
% & \ge s \sup_{\sigma\in \{-1,1\}^{\cZ_1}} \Pi_\sigma \left(\cE_{Q^\sigma} (\hat f)\ge s \right) \\
% & \ge s \frac {3-2\sqrt{2}}{8}\\
% & \ge C'n_P^{-\frac{1+\beta}{d_0}}
% \end{align*}

% \subsection{Difficulty of the parametric part} To study the difficulty of the parametric part, it is enough to construct two well-separated hypotheses (versus the family of well-separated hypotheses required in our study of the non-parametric part).

% Let $ w = \frac 1{16} $ and $\delta > 0$ be a constant to be chosen later. Consider the following class conditional densities:
% \[ g_1(x) = \begin{cases}
% 4w (1-\delta) & \text{if } 0 \le  x_1 \le \frac 14,\\
% 4\delta & \text{if } \frac 38 \le x_1 \le \frac 58, \\
% 4(1-\delta)(1-w) & \text{if } \frac 34 \le x_1 \le 1, \\
% 0 & \text{elsewhere}.
% \end{cases} \] and \[ g_0(x) = \begin{cases}
% 4(1-w) (1-\delta) & \text{if } 0 \le  x_1 \le \frac 14,\\
% 4\delta & \text{if } \frac 38 \le x_1 \le \frac 58, \\
% 4(1-\delta)w & \text{if } \frac 34 \le x_1 \le 1, \\
% 0 & \text{elsewhere}
% \end{cases} \] Let $ \sigma \in \{-1, 1\}. $ We specify the class probabilities in the following way:
% \[ \pi_P = \frac12 , \ \pi_Q^\sigma = \frac 12 (1+\sigma m) \]  where, $  m = \frac 1 {16\sqrt{n_Q}}. $ The regression function is piece-wise constant: \[ \eta_Q^\sigma (x) = \frac{\pi_Q^\sigma g_1(x)}{\pi_Q^\sigma g_1(x) + (1-\pi_Q^\sigma)g_0(x)} = \begin{cases}
% \frac{w(1+\sigma m)}{w(1+\sigma m) + (1-w) (1-\sigma m)} & \text{if }  0 \le  x_1 \le \frac 14,\\
% \frac{1+\sigma m}{2} & \text{if } \frac 38 \le x_1 \le \frac 58, \\
% \frac{(1-w)(1+\sigma m)}{(1-w)(1+\sigma m) + w (1-\sigma m)} & \text{if } \frac 34 \le x_1 \le 1.
% \end{cases} \] This simplifies the calculation of the excess risk.

% Armed with the class conditional densities and the class probabilities, we define the distributions $P$ and $Q^\sigma$ as: for a Borel set $ A \subset [0,1]^d $ and for index $ y \in \{0,1\} $ \[ P(X\in A, Y = y) = y \pi_P \int_A g_1(x) + (1-y) (1-\pi_P) \int_A g_0(x) \] and 

% \[ Q^\sigma (X\in A, Y = y) = y \pi_Q^\sigma \int_A g_1(x) + (1-y) (1-\pi_Q^\sigma) \int_A g_0(x). \]

% It is not hard to check that the densities $ g_0 $ and $ g_1 $ are locally $ \alpha $-H\"older smooth with constant $ C_\alpha. $ They are piece-wise constant on their support and each ``piece'' of the support is separated. We need to check the margin  condition. 

% \paragraph{Checking margin condition (definition \ref{def:margin-condition})} 
% We have \begin{align*}
% \left|\frac{w(1+\sigma m)}{w(1+\sigma m) + (1-w) (1-\sigma m)} - \frac 12\right| & = \frac 12  \frac{|w(1+\sigma m) - (1-w) (1-\sigma m)|}{w(1+\sigma m) + (1-w) (1-\sigma m)}\\ 
% & = \frac 12 \frac {|2w +\sigma m -1|}{1-\sigma m + 2\omega\sigma m	}\\
% & = \frac 12 \frac {1-2w -\sigma m }{1-\sigma m + 2\omega\sigma m	} \ge \frac 12 \frac {1-3/16}{1+3/16} = \frac {13}{38}
% \end{align*}

% and \begin{align*}
% \left| \frac{(1-w)(1+\sigma m)}{(1-w)(1+\sigma m) + w (1-\sigma m)} - \frac 12 \right| & = \frac12 \frac{(1-w)(1+\sigma m)- w (1-\sigma m) }{(1-w)(1+\sigma m) + w (1-\sigma m)} \\
% & = \frac 12 \frac{1+\sigma m-2w}{1 +\sigma m- 2w\sigma m} \ge \frac 12 \frac {1-3/16}{1+3/16} = \frac {13}{38}
% \end{align*}
% Thus $Q\left( \left| \eta_Q^\sigma(X) - \frac 12 \right| \le t  \right) = 0$ for any $ t < m $. For $ m \le t < \frac{13}{38}$, 
% \begin{align*}
% Q\left( \left| \eta_Q^\sigma(X) - \frac 12 \right| \le t  \right) &= Q \left( \frac 38 \le X_1 \le \frac 58  \right) = \delta. 
% \end{align*}
% We pick $ \delta = C_\beta m^\beta . $ Then \[ Q\left( \left| \eta_Q^\sigma(X) - \frac 12 \right| \le t  \right) \le C_\beta m^\beta \le C_\beta t^\beta. \]
% and for $ t \ge \frac{13}{38} $ we have \[ Q\left( \left| \eta_Q^\sigma(X) - \frac 12 \right| \le t  \right) \le 1 \le C_\beta t^\beta. \]

% Define the family of distributions $ \cH = \{ \Pi_\sigma : \sigma \in \{-1, 1\} \}, $ where $\Pi^\sigma = P^{\otimes n_P} \otimes \left(Q_X^\sigma \right)^{\otimes n_Q}$. For this family, $ M = |\cH| = 2 $ , $ \Pi_{1} \ll \Pi_{-1} $, and the KL divergence between $ \Pi_{-1} $ and $ \Pi_1 $ is \begin{align*}
% \KL\left(  \Pi_1 \mid \Pi_{-1}  \right)  = & n_Q \KL\left(Q_X^{(-1)}\mid Q_X^{(1)}\right)\\
% \le &  n_Q \KL\left(Q^{(-1)}\mid Q^{(1)}\right) \ \text{using lemma \ref{lemma:kl-ineq}}, \\
% = &  n_Q \Bigg[ \log\left( \frac{1+\frac{1}{16\sqrt{n_Q}}}{1-\frac{1}{16\sqrt{n_Q}} } \right) \left( 1+\frac{1}{16\sqrt{n_Q}}  \right)\\
% & + \log\left( \frac{1-\frac{1}{16\sqrt{n_Q}}}{1+\frac{1}{16\sqrt{n_Q}} } \right) \left( 1-\frac{1}{16\sqrt{n_Q}}  \right)  \Bigg] \\
% = & \frac {2n_Q}{16\sqrt{n_Q}} \log\left( \frac{1+\frac{1}{16\sqrt{n_Q}}}{1-\frac{1}{16\sqrt{n_Q}} } \right)\\
% \le & \frac{6n_Q}{256 n_Q } \ \text{using } \log\left( \frac{1+x}{1-x} \right) \le 3x \text{ for } 0 \le x\le \frac 12,\\
% = & \frac 3{128}.
% \end{align*}
% Thus
% \[
% \frac1M \sum_{\sigma\in \{-1,1\}} \KL(\Pi^\sigma \mid \Pi^{-1}) = \frac12 \KL(\Pi^1 \mid \Pi^{-1}) = \frac 3 {256} < \frac{\log 2}{8}.
% \]
% Let $h_\sigma  $ be the Bayes decision rule for the distribution $ Q^\sigma,  $ \ie, \ \[ h_\sigma (x) = \indicator\left\{ \eta_Q^\sigma (x)  \ge \frac 12  \right\}. \] Then  \begin{align*}
% \cE_{Q^{1}}\left(h_{-1}\right) & = \Ex_{Q^{1}} \left[ \left| \eta_Q^1(X) - \frac 12 \right|\indicator\left\{h_1(X) \neq h_{-1}(X)  \right\}  \right]\\
% & = \delta m \\
% & = \frac{C_\beta}{16^{\beta+1}} n_Q^{-\frac{\beta+1}{2}} \triangleq 2s.
% \end{align*}
% By proposition \ref{prop:tsybakov} \begin{align*}
% \sup_{(P,Q)\in \Pi} \Ex \cE_Q (\hat f)& \ge \sup_{(P,Q)\in \Pi} s \Pr_\Pi \left ( \cE_Q (\hat f)\ge s \right)\\
% & \ge s \sup_{\sigma\in \{-1,1\}} \Pi_\sigma \left(\cE_{Q^\sigma} (\hat f)\ge s \right) \\
% & \ge s \frac {3-2\sqrt{2}}{8}\\
% & \ge C'n_Q^{-\frac{1+\beta}{2}}
% \end{align*}
% We combine the lower bounds for the parametric and non-parametric parts to obtain the stated lower bound.































\begin{lemma}
\label{lemma:margin-unlabeled-density}
For any $\sigma \in \{-1, 1\}^{\cZ_1}$  $Q_\sigma$ as defined in  \ref{eq:dist-Q-unlabeled-density} satisfies $\alpha$-margin condition with constant $C_\alpha.$ 
\end{lemma}

\begin{proof}
We recall the marginal and regression function as in \ref{eq:marginals-unlabeled-density} and  \ref{eq:reg-fn-unlabeled-density}, respectively. For such a regression function \[ 
\big| \eta_Q^{\sigma}(x) - 1/2 \big|  = \begin{cases}
      \sqrt{\eps_P} \eta_z(x)/2 & \hspace{0.3cm} x \in C(z),\ z \in \cZ_1,\\
      \sqrt{\eps_P} \eta_{f(z)}(x)/2 & \hspace{0.3cm} x \in C(f(z)),\  z \in \cZ_1,\\
    0 & \hspace{0.3cm} x \in C(z),\  z \in \cZ_0.
    \end{cases}
\]

Let $z \in \{-1, 1\}^{\cZ_1}$ For $0 \le t \le \frac{\sqrt{\eps_P}C_\beta' r_1^\beta}{2^{1+\beta}}$ we have 
\[
\begin{aligned}
& Q_X \Big( 0 < \big| \eta_Q^{\sigma}(x) - 1/2 \big| \le t, x \in C(z) \Big)\\
& \le  Q_X \Big( \eta_z(x) \le \frac{2t}{\sqrt{\eps}C_\beta'  r_1^\beta} \Big) \\
& \le Q_X \Bigg[ \frac {c_w r_1} 2 \left( 1- \left(\frac{2t}{\sqrt{\eps_P}C_\beta'r_1^\beta}\right)^{1/\beta} \right) \le \|x-z\|_2 \le \frac {c_w r_1}2  \Bigg]
\end{aligned}
\]

Let $\bS^{d-1} = \{ x \in \real^d : \|x\|_2 = 1 \}$ let us define  $A(d-1) = \text{Leb}_{d-1} \big(\bS^{d-1}\big).$

\[
\begin{aligned}
& Q_X \Big( 0 < \big| \eta_Q^{\sigma}(x) - 1/2 \big| \le t, x \in C(z) \Big)\\
& \le A(d-1) \left(\frac{c_w r_1}{2}\right)^d \left[ 1- \left( 1- \left(\frac{2t}{\sqrt{\eps_P}C_\beta'r_1^\beta}\right)^{1/\beta} \right)^d \right]\\
& \le c \big(c_w r_1\big)^d \left(\frac{2t}{\sqrt{\eps_P}C_\beta'r_1^\beta}\right)^{1/\beta}\\
& \le c \big(c_w r_1\big)^d \left(\frac{2t}{\sqrt{\eps_P}C_\beta'r_1^\beta}\right)^{\alpha}
\end{aligned}
\]
where we get the last inequality using $\frac{2t}{\sqrt{\eps_P}C_\beta'r_1^\beta} \le  1$ and $\alpha\beta \le 1. $ Finally, \[
\begin{aligned}
Q_X \Big( 0 < \big| \eta_Q^{\sigma}(x) - 1/2 \big| \le t \Big) & \le 2m c \big(c_w r_1\big)^d \left(\frac{2t}{\sqrt{\eps_P}C_\beta'r_1^\beta}\right)^{\alpha}\\
& \le 2c_m r_1^{\alpha\beta-d} \big(c_w r_1\big)^d \left(\frac{2t}{\sqrt{\eps_P}C_\beta'r_1^\beta}\right)^{\alpha}\\
& \le c' c_w^d t^\alpha\\
& \le C_\alpha t^\alpha,
\end{aligned}
\]
for suitably chosen $c_w<1.$ For $ t \ge \frac{\sqrt{\eps_P}C_\beta' r_1^\beta}{2^{1+\beta}} $ we have \[
\begin{aligned}
Q_X \Big( 0 < \big| \eta_Q^{\sigma}(x) - 1/2 \big| \le t \Big) & \le 2m A(d-1) \big(c_w r_1/2\big)^d\\
& \le c c_w^d r_1^{\alpha\beta - d} r_1^d\\
& \le c c_w^d r_1^{\alpha\beta}\\
& \le C_\alpha \left(\frac{\sqrt{\eps_P}C_\beta' r_1^\beta}{2^{1+\beta}}\right) ^\alpha\\
& \le C_\alpha t^\alpha,
\end{aligned}
\] for suitably chosen $c_w<1.$
\end{proof}

\begin{lemma}
\label{lemma:kl-unlabeled-density}
Let $\Big\{\Pi_\sigma: \sigma \in \{-1, 1\}^{\cZ_1}\Big\}$ be the class of joint distributions defined in \ref{eq:dist-unlabeled-joint-density}. For $\sigma, \sigma' \in  \{-1, 1\}^{\cZ_1}$ we have \[ KL(\Pi_{\sigma}|| \Pi_{\sigma'})  \le c_w^dK(d, \alpha, \beta)\rho(\sigma, \sigma'). \]
\end{lemma}

\begin{proof}
We recall from \ref{eq:marginals-unlabeled-density} $Q_{X, \sigma}\sim \text{Uniform}\big([0,1]^d\big)$ doesn't depend on $\sigma.$ Hence, \[ KL\Big(Q_{X, \sigma}||Q_{X, \sigma'}\Big) = 0. \]

We refer to lemma C.4 in supplement   to show \[
\begin{aligned}
KL\Big(P_\sigma||P_{\sigma'}\Big) & = \frac 12 \Big(g_0^\sigma||g_0^{\sigma'}\Big) + \frac12 \Big(g_1^\sigma||g_1^{\sigma'}\Big)\\
& \le \eps_P c_w^d K'(d,\alpha, \beta ) r_1^{2\beta + d} \rho(\sigma, \sigma').
\end{aligned}
\]
Combining them we get \[ 
\begin{aligned}
KL\Big(\Pi_\sigma||\Pi_{\sigma'}\Big) & = n_P KL\Big(P_\sigma||P_{\sigma'}\Big) + n_Q KL\Big(Q_{X, \sigma}||Q_{X, \sigma'}\Big) \\
& \le n_P \eps_P  c_w^d K'(d,\alpha, \beta ) r_1^{2\beta + d} \rho(\sigma, \sigma')\\
& \le c_w ^d K'(d,\alpha, \beta ) c_r^{2\beta+d} (\eps_P n_P) (\eps_Pn_P)^{-1} \rho(\sigma, \sigma')\\
& \le c_w^d K(d, \alpha, \beta) \rho(\sigma, \sigma').
\end{aligned}
\]
\end{proof}
